Deciding the Closure of Inconsistent Rooted Triples is NP-Complete

Interpreting three-leaf binary trees or {\em rooted triples} as constraints yields an entailment relation, whereby binary trees satisfying some rooted triples must also thus satisfy others, and thence a closure operator, which is known to be polynomial-time computable. This is extended to inconsistent triple sets by defining that a triple is entailed by such a set if it is entailed by any consistent subset of it. Determining whether the closure of an inconsistent rooted triple set can be computed in polynomial time was posed as an open problem in the Isaac Newton Institute's "Phylogenetics" program in 2007. It appears (as NC4) in a collection of such open problems maintained by Mike Steel, and it is the last of that collection's five problems concerning computational complexity to have remained open. We resolve the complexity of computing this closure, proving that its decision version is NP-Complete. In the process, we also prove that detecting the existence of {\em any} acyclic B-hyperpath (from specified source to destination) is NP-Complete, in a significantly narrower special case than the version whose {\em minimization} problem was recently proven NP-hard by Ritz et al. This implies it is NP-hard to approximate (our special case of) their minimization problem to within {\em any} factor.

==> rt-proof-arx_copy.tex <==
% !TEX root = rootedtriples-arx.tex

\section{The Proof}

Clearly \entailprob\ is in NP: if we guess the subset $R' \subset R$, then we can verify both that $R'$ is consistent and that $R' \vdash t$ by executing Aho et al.\ \cite{aho1981inferring}'s polynomial-time BUILD algorithm on $R'$ \cite{bryant1995extension}. \minapdh\:is as well: guess the path, and check that it is acyclic.

Now we prove hardness, arguing that $R$ contains a consistent subset entailing $\alpha\beta|\gamma$ iff $H$ contains an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ iff $F$ admits a satisfying assignment $\mathbf{v}(\cdot)$, in two steps.



First we argue that acyclic paths correspond to satisfying truth assignments.
%\textbf{3SAT} reduces to \apdh\:(which is therefore NP-Complete):


\subsection{Acyclic Path $\Leftrightarrow$ Satisfying Truth Assignment}

\begin{lemma}
There is an an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ iff $F$ admits a satisfying truth assignment $\mathbf{v}(\cdot)$.
%If there is a satisfying truth assignment, then there is an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$.
\end{lemma}
\begin{proof}
($\Leftarrow$)
We construct $P$ based on the satisfying truth assignment $\mathbf{v}(\cdot)$. For each $x_i$, if $\mathbf{v}(x_i) =$ true, then we have $P$ take the $x_i$ gadget's {\em negative} side (drawn lower in Fig.\ \ref{fig:var}); otherwise, we have $P$ take its {\em positive} side (drawn higher). Then within each $C_j$, among the three possible witness paths, we choose one corresponding to the appearance of a literal that is true under $\mathbf{v}(\cdot)$ (which by assumption must exist).
%, which therefore points only to sides of variable gadgets that $P$ did {\em not} take. 
For the remainder of $P$ we have it take the required connecting arcs.

Notice that any potenial cycle contained within $P$ must necessarily involve an arc $e$ whose tail lies within some clause $C_j$'s gadget and one of whose heads lies within some variable $x_i$'s gadget. But the witness path taken within $C_j$'s gadget corresponds to an appearance $\tilde x_i^j$ of a true literal $\tilde x_i$. If it a positive literal, i.e., $\tilde x_i=x_i$, then $\mathbf{v}(x_i) =$ true, and we would have had $P$ take the $x_i$ gadget's {\em negative} side---not the side $e$ is pointing to. Similarly, if $\tilde x_i=\bar x_i$, then $\mathbf{v}(x_i) =$ false, $P$ would have taken the $x_i$ gadget's {\em positive} side, which again is then not the side $e$ is pointing to. Thus $P$ must be acyclic.

($\Rightarrow$)
We read off $\mathbf{v}(\cdot)$ from the choices the path $P$ makes when passing through the series of variable gadgets, i.e., setting $\mathbf{v}(x_i) = $ true if $P$ used the $x_i$ gadget's {\em negative} side, and setting it to false otherwise. Now, consider a clause $C_j$'s gadget, whose witness node points to a node $v'$ within some variable $x_i$'s gadget. Because $P$ is acyclic, we know that $v'$ is on the side of $x_i$'s gadget that $P$ did {\em not} use. Since we chose the truth value $\mathbf{v}(x_i)$ that makes literals within nodes on the $x_i$ gadget's {\em unused} side true, this implies that literal corresponding to $C_j$'s witness node is true, thus satisfying the clause.
\end{proof}

Thus we have proven:

\begin{theorem}\label{thm:apdh}
\minapdh\:is NP-Complete.
\end{theorem}

Since an infeasible solution is defined to have infinite cost, an algorithm with {\em any} approximation factor would allow us to distinguish between positive and negative problem instances, which immediately implies:
\begin{corollary}
Approximating \minapdh\:to within {\em any} factor is NP-hard.
\end{corollary}

Even if we restrict ourselves to problem instances admitting feasible solutions, this ``promise problem" \cite{goldreich2005promise} special case is hard to approximate within any reasonable factor.

%More formally, we obtain the following hardness of approximation.

\begin{corollary}
%In the promise problem \cite{goldreich2005promise} special case in which an acyclic B-hyperpath is assumed to exist, approximating \minapdh\:to within factor $|V|^{1-\epsilon}$ for any $\epsilon>0$ is NP-hard.
\minapdhprom\:is NP-hard to approximate to within factor $|V|^{1-\epsilon}$ for all $\epsilon>0$.
\end{corollary}
\begin{proof}
Let $\epsilon \in (0,1/4)$. Let $I = \langle H,u,v \rangle$ be an instance \minapdhprom. For this proof only, let $n=|V(H)|$.
We extend $H$ to a new hypergraph $H'$ by adding polynomially many dummy edges forming an acyclic $u{\to}v$ path of length $n^{\lceil1+1/\epsilon\rceil}$, yielding a hypergraph $H'$ with $n' = n+n^{\lceil1+1/\epsilon\rceil}-1$ nodes and a new problem instance $I' = \langle H',u,v \rangle$, which is also by construction a valid problem instance of \minapdhprom. If $H$ has a path ($I$ is a positive instance), then $H'$ (like $H$) has one of some length $OPT^+ \le n-1$; if not ($I$ is a negative instance), then $H'$'s only path has length $OPT^- = n^{\lceil1+1/\epsilon\rceil}$.

Now, suppose there were a $|V|^{1-\epsilon}$-approximation algorithm.

Running it on the $I'$ resulting from a negative $I$ will yield a path of length at least $LB^- = OPT^- = n \cdot n^{\lceil1/\epsilon\rceil}$.

Running it on the $I'$ resulting from a positive $I$ will yield a path of length of at most
\begin{align*}
UB^+ &= n'^{1-\epsilon}\cdot (n-1)\\
&= (n+n^{\lceil1+1/\epsilon\rceil}-1)^{1-\epsilon}\cdot (n-1)\\
& < (n-1) \cdot n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)} + (n-1)^{2-\epsilon}\\
&< n \cdot n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)},
\end{align*}
where the last inequality follows from the fact that $(n-1)^{2-\epsilon} < n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)}$ for $\epsilon<1/4$.

Because $\lceil1+1/\epsilon\rceil\cdot(1-\epsilon) = 1+\lceil1/\epsilon\rceil - \epsilon - \epsilon \lceil 1/\epsilon \rceil < \lceil 1/\epsilon \rceil$, it follows that $UB^+ < LB^-$.

%$\lceil1/\epsilon\rceil$ vs $\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)$
%
%$\lceil1/\epsilon\rceil$ vs $\lceil1/\epsilon\rceil\cdot(1-\epsilon) + (1-\epsilon)$
%
%$\lceil1/\epsilon\rceil$ vs $\lceil1/\epsilon\rceil - \lceil1/\epsilon\rceil\cdot\epsilon + (1-\epsilon)$
%
%0 vs $- \lceil1/\epsilon\rceil\cdot\epsilon + (1-\epsilon)$
%
%$\lceil1/\epsilon\rceil\cdot\epsilon > (1-\epsilon)$

Thus by comparing the length $ALG$ of the path in $H'$ found by the hypothetical algorithm to $UB^+$ and $LB^-$, we can decide whether $I$ was positive or negative.
%
%Then any algorithm providing an $f(|V|)$-approximation would allow us to distinguish (for $|V|$ sufficiently large) between instances $H'$ with optimal solution cost $<f(|V|)\cdot|V|$ and those with optimal solution cost $\ge f(|V|) \cdot |V|^2$, thus deciding whether $H$ had a path.
\end{proof}




Second, to extend the reduction to \entailprob, we argue that $H$ is a faithful representation of $R$ in the sense that acyclic paths from $\alpha\beta$ to $c_{m+1}\gamma$ (or acyclic supersets of such paths) correspond to consistent subsets entailing $\alpha\beta|\gamma$, and vice versa.


\subsection{Consistent Entailing Subset $\Leftarrow$ Acyclic Path}

We prove this direction via two lemmas, proving that the set of triples corresponding to an acyclic path are consistent and entail $\alpha\beta|\gamma$, respectively.



\begin{lemma}\label{lem:consistR}
If $P$ is an acyclic path $P$ in the hypergraph from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \text{triples}(P)$ is consistent.
\end{lemma}
\begin{proof}
To prove $R'$ consistent, we 
%reinterpret the procedure we carried out in the proof of Lemma \ref{lem:isentailed} as implicitly executing 
step through the execution of Aho et al.\ \cite{aho1981inferring}'s BUILD algorithm on input $R'$, picturing the state of the resulting Ahograph (see Fig.\ \ref{fig:ahograph}) and the tree being constructed (see Fig.\ \ref{fig:pathtree}) as they progress over time.
%Specifically, each application of dyadic inference rule (\ref{eq:2b}), as we step through $P$ in reverse order, can be interpreted as one iteration (or recursive call) of BUILD.
Each iteration can be interpreted one application of dyadic inference rule (\ref{eq:2b}), as we step through $P$ in reverse order.

%, of stepping through $P$ in reverse, repeatedly applying dyadic inference rule (\ref{eq:2b})
%
%again step through $P$ in reverse, implicitly executing Aho et al.\ \cite{aho1981inferring}'s BUILD algorithm on input $R'$, picturing the state of the resulting Ahograph (see Fig.\ \ref{fig:ahograph}) and the tree being constructed (see Fig.\ \ref{fig:pathtree}) along the way. 

Observe that in Ahograph $[R', L(R')]$ (see Fig.\ \ref{fig:ahograph}), $\gamma$ will be an isolated A-node, since $R$ contains no triples with $\gamma$ on their LHSs,
%Just as dyadic inference rule (\ref{eq:2b}) carried us through to $\alpha\beta | \sigma$, 
%Observe also that by definition of $R'$, the A-nodes $L(R') - \{\gamma\}$ are connected in one component of Ahograph $[R', L(R')]$, 
and that the edge $\{c_m, c_{m+1}\}$ in $[R', L(R')]$ due to $P$'s last arc (representing $c_m c_{m+1} | \gamma$) is labeled (only) with $\gamma$. Isolated A-node $\gamma$ is removed for BUILD's second iteration, in which we recurse on the remaining A-nodes. The edge $\{c_m, c_{m+1}\}$ will therefore no longer appear in that iteration's Ahograph, $[R', L(R') - \{\gamma\}]$, rendering $c_{m+1}$ an isolated A-node.

We claim that this pattern will continue to obtain the rest of the way back to the start of $P$, with a new A-node becoming isolated  by the start of each iteration, causing an edge to be removed, and hence isolating another A-node for the succeeding iteration.
%
More precisely, number the iterations in reverse, counting downward from $\ell=|P|$, where iteration $\ell$ is the first iteration executed, in which because A-node $o_\ell$ is observed to be isolated, the Ahograph's edge $\{p_\ell,q_\ell\}$ due to triple $p_\ell q_\ell | o_\ell = c_m,c_{m+1} | \gamma$ is removed. 



Let $H_P$ be the subhypergraph of $H$ induced by the nodes $\{\text{t}(e) : {e \in P}\} \cup \{c_{m+1}\gamma\}$, and recall that nodes in $H$ correspond to unordered pairs of A-nodes, and thus to potential edges in the Ahograph.

Because $P$ is a path, each node in $H_P$ except $c_{m+1}\gamma$ (which has out-degree 0) will have out-degree 1. Therefore the Ahograph will have exactly $\ell$ edges, each with one label.
%
%%of $H$ induced by $P$ has out-degree at most one. Therefore no edge in the Ahograph has more than one label. Note that $\alpha$ and $\beta$ will not be labels of any edge.
%
Because $P$ is acyclic, each node in $H_P$ except $\alpha\beta$ (which has in-degree 0) will have in-degree 1. Therefore no label will appear on multiple edges in the Ahograph.
%
Thus there is a bijection between Ahograph's $\ell$ edges and the labels appearing on them.

Node $\alpha\beta$ contains two leaves, and each arc in $P$ introduces one additional leaf, for a total of $\ell+2$ leaves in $L(R')$, and hence $\ell+2$ A-nodes in the Ahograph.

Note also that the first arc in $P$ adds label $a_1$ to edge $\{\alpha,\beta\}$ in the Ahograph, and that each subsequent arc adds a label to an edge incident to the preceding edge, and so all the Ahograph's $\ell$ edges lie within a single component. Since $\gamma$ is an isolated A-node, this means that that component has exactly $\ell+1$ A-nodes, and is therefore a tree.

%To see this, suppose $c_j \tilde x_i^j{\to}\{\tilde x_i^j \tilde y_i^j, c_j \tilde y_i^j\}$ is a back-arc in $P$.
%
%there are no other edges in the Ahograph beyond those listed here.
%%
%Note also that no label appears on more than one edge. Therefore there is a one-to-one correspondence between the Ahograph's $\ell$ edge labels and $P$'s arcs. Every A-node appears (once) as a label, except for $\alpha$ and $\beta$. Thus the Ahograph has $\ell+2$ A-nodes, and its second component is a tree.

Now, we prove by induction that at the start of each iteration $k$ from $\ell$ down to $1$, the Ahograph consists of two components: some isolated A-node $o_k$ and a tree. We have already verified the base case: $o_\ell$ is isolated at the start, in iteration $\ell$, and the $\ell+1$ remaining nodes form a tree. Assume the claim is true for each iteration from $\ell$ down through some iteration $k$.

%If this is not true for every iteration, let $k$ be the first iteration at the start of which $o_k$ is not isolated. Now, we know that at the start the previous iteration (iteration $k+1$), $o_{k+1}$ (which is the right-hand side of triple $u_{k+1}|o_{k+1}$, where $o_k \in u_{k+1}$) was found to be isolated, and therefore was removed from the iteration-$k$ Ahograph. What does it mean if we find at the start of iteration $k$ that $o_k$ is still not isolated?
%
%The deletion of $o_{k+1}$ meant the removal of label $o_{k+1}$ from from the Ahograph of edge $u_{k+1}$, which contains $o_k$. If edge $u_{k+1}$ nonetheless remains in the Ahograph, this means that it still has some label.


%\begin{align}
%\nonumber(&\gamma{:}\{c_{m+1},c_m\},\\
%&c_{m+1}{:}\{\tilde y_{i_{w_m}}^m,c_m\},~\tilde y_{i_{w_m}}^m{:}\{\tilde x_{i_{w_m}}^m,c_m\},~\tilde x_{i_{w_m}}^m{:}\{d_m,c_m\},~ d_m{:}\{c_m,c_{m-1}\},~ c_m{:}\{\tilde y_{i_{w_{m-1}}}^{m-1},c_{m-1}\},\\
%& ...,\\
%&c_2{:}\{\tilde y_{i_{w_1}}^1,c_1\},~\tilde y_{i_{w_1}}^1{:}\{\tilde x_{i_{w_1}}^1,c_1\},~\tilde x_{i_{w_1}}^1{:}\{d_1,c_1\},~ d_1{:}\{c_1,b_{n+1}\},~c_1{:}\{b_{n+1},a_{n+1}\},~b_{n+1}{:}\{a_{n+1},\tilde y_n^m\},\label{eq:clauses}\\
%&a_{n+1}{:}\{\tilde y_n^m,\tilde x_n^m\},~\tilde y_n^m{:}\{\tilde x_n^m,\tilde y_n^{m-1}\},~ ...,~\tilde x_{n}^2 {:}\{\tilde y_{n}^1,\tilde x_{n}^1\},~\tilde y_n^1{:}\{\tilde x_n^1,b_n\},~\tilde x_n^1{:}\{b_n,a_n\},~b_n{:}\{a_n,\tilde y_{n-1}^m\},\label{eq:varn}\\
%\nonumber&a_n{:}\{\tilde y_{n-1}^{m},\tilde x_{n-1}^{m}\},~\tilde y_{n-1}^m{:}\{\tilde x_{n-1}^m,\tilde y_{n-1}^{m-1}\},~ ...,~\tilde x_{n-1}^2{:}\{\tilde y_{n-1}^1,\tilde x_{n-1}^1\},~\tilde y_{n-1}^1{:}\{\tilde x_{n-1}^1,b_{n-1}\},~\tilde x_{n-1}^1{:}\{b_{n-1},a_{n-1}\},\\ 
%&b_{n-1}{:}\{a_{n-1},\tilde y_{n-2}^m\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&a_2{:}\{\tilde y_1^m,\tilde x_1^m\},~\tilde y_m^1{:}\{\tilde x_1^m,\tilde y_1^{m-1}\},~ ...,~\tilde x_1^2{:}\{\tilde y_1^1,\tilde x_1^1\},~\tilde y_1^1{:}\{\tilde x_1^1,b_1\},~\tilde x_1^1{:}\{b_1,a_1\},~
%b_1{:}\{a_1,\beta\},\label{eq:var1}\\ 
%\nonumber&a_1{:}\{\beta,\alpha\})
%\end{align}




%Given such a path $P$, we construct the corresponding $R'=f(P)$. By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths as follows:
%\begin{eqnarray*}
%P &=& (\alpha\beta,e_1,\beta a_1, e_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (a_{n+1}b_{n+1},e_3,b_{n+1}c_1,e_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (c_{m+1}\gamma)
%\end{eqnarray*}
%Given such an arc set $P$, we construct the corresponding $R'=f(P)$. 
%We choose $A' = P$, and set $R' = \text{triples}(A')$, which is consistent by Lemma \ref{lem:consistR}.
By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths:
\begin{align*}
P &~=~ (e_1,e_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (e_3,e_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m},
\end{align*}
where $P_{x_i}$ is one of the two length-$2m{+}2$ subpaths passing through $x_i$'s gadget (from $a_ib_i$ to $a_{i+1}b_{i+1}$), $P_{C_j}$ is one of the three length-4 subpaths traversing one of the $C_j$ gadget's three witness paths (from $c_jd_j$ to $c_jc_{j+1}$) {\em plus the succeeding arc with tail $c_jc_{j+1}$}, and $e_1,...,e_4$ are shorthand names for the other four connecting arcs.





For each $C_j$, let $\hat i_j$ denote the index $i$ of the variable $x_i$ appearing in the witness path of $C_j$ (through literal appearance $\tilde x_{\hat i_j}^j$) that $P$ traverses.

Now, consider the following {\em reverse linear ordering} of the A-node-labeled edges of Ahograph $[R', L(R')]$, with each subsequence of A-node-labeled edges is tagged to indicate the corresponding subpath of $P$ (compare to Figs.\ \ref{fig:ahograph} and \ref{fig:overview}, and in particular compare each ($P_{C_j}$) to Fig.\ \ref{fig:clause} and each ($P_{x_i}$) to Fig.\ \ref{fig:var}): %, for an acyclic path $P$: 
%(which takes the positive sides of variable gadgets $x_n,\tilde x_{n-1},\tilde x_1$):
\begin{alignat}{7}
(&\gamma{:}\{c_m,c_{m+1}\}, ~~&&c_{m+1}{:}\{c_m,\tilde y_{\hat i_m}^m\}, ~~&&\tilde y_{\hat i_m}^m{:}\{c_m,\tilde x_{\hat i_m}^m\}, ~~&&\tilde x_{\hat i_m}^m{:}\{c_m,d_m\},\label{eq:clausem}\tag{$P_{C_m}$}\\
&d_m{:}\{c_m,c_{m-1}\}, ~~&&c_m{:}\{c_{m-1},\tilde y_{\hat i_{m-1}}^{m-1}\}, ~~&&\tilde y_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},\tilde x_{\hat i_{m-1}}^{m-1}\}, ~~&&\tilde x_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},d_{m-1}\},\label{eq:clausemm1}\tag{$P_{C_{m-1}}$}\\
& ...,\nonumber\\
&d_2{:}\{c_2,c_2\}, ~~&&c_2{:}\{c_1,\tilde y_{\hat i_1}^1\}, ~~&&\tilde y_{\hat i_1}^1{:}\{c_1,\tilde x_{\hat i_1}^1\}, ~~&&\tilde x_{\hat i_1}^1{:}\{c_1,d_1\},\label{eq:clause1}\tag{$P_{C_1}$}\\
&d_1{:}\{c_1,b_{n+1}\}, ~~&&c_1{:}\{b_{n+1},a_{n+1}\},\label{eq:var2clause}\tag{$e_3,e_4$}\\
&b_{n+1}{:}\{a_{n+1},\tilde y_n^m\}, ~~&&a_{n+1}{:}\{\tilde y_n^m,\tilde x_n^m\}, ~~&&\tilde y_n^m{:}\{\tilde x_n^m,\tilde y_n^{m-1}\}, ~ \quad..., ~~&&\tilde x_{n}^2 {:}\{\tilde y_{n}^1,\tilde x_{n}^1\},\nonumber\\
&\quad\tilde y_n^1{:}\{\tilde x_n^1,b_n\}, ~~&&\tilde x_n^1{:}\{b_n,a_n\},\label{eq:varn}\tag{$P_{x_n}$}\\
&b_n{:}\{a_n,\tilde y_{n-1}^m\}, ~~&&a_n{:}\{\tilde y_{n-1}^{m},\tilde x_{n-1}^{m}\}, ~~&&\tilde y_{n-1}^m{:}\{\tilde x_{n-1}^m,\tilde y_{n-1}^{m-1}\},~~ ..., ~~&&\tilde x_{n-1}^2{:}\{\tilde y_{n-1}^1,\tilde x_{n-1}^1\},\nonumber\\
&\quad\tilde y_{n-1}^1{:}\{\tilde x_{n-1}^1,b_{n-1}\}, ~~&&\tilde x_{n-1}^1{:}\{b_{n-1},a_{n-1}\},\label{eq:varnm1}\tag{$P_{x_{n-1}}$}\\
&...,\nonumber\\
&b_{2}{:}\{a_{2},\tilde y_{1}^m\}, ~~&&a_{2}{:}\{\tilde y_{1}^m,\tilde x_{1}^m\}, ~~&&\tilde y_1^m{:}\{\tilde x_1^m,\tilde y_1^{m-1}\},~ \quad..., ~~&&\tilde x_1^2{:}\{\tilde y_1^1,\tilde x_1^1\},\nonumber\\
&\tilde y_1^1{:}\{\tilde x_1^1,b_1\}, ~~&&\tilde x_1^1{:}\{b_1,a_1\},\label{eq:var1}\tag{$P_{x_1}$}\\
&b_1{:}\{a_1,\beta\}, ~~&&a_1{:}\{\beta,\alpha\})\tag{$e_3,e_4$}
\end{alignat}


%\begin{alignat}{3}
%(&\gamma{:}\{c_m,c_{m+1}\}, ~~&&c_{m+1}{:}\{c_m,\tilde y_{\hat i_m}^m\}, ~~\tilde y_{\hat i_m}^m{:}\{c_m,\tilde x_{\hat i_m}^m\}, ~~\tilde x_{\hat i_m}^m{:}\{c_m,d_m\},\label{eq:clausem}\\
%&d_m{:}\{c_m,c_{m-1}\}, ~~&&c_m{:}\{c_{m-1},\tilde y_{\hat i_{m-1}}^{m-1}\}, ~~\tilde y_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},\tilde x_{\hat i_{m-1}}^{m-1}\}, ~~\tilde x_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},d_{m-1}\},\label{eq:clausemm1}\\
%& ...,\label{eq:clauses}\\
%&d_2{:}\{c_2,c_2\}, ~~c_2{:}\{c_1,\tilde y_{\hat i_1}^1\}, ~~\tilde y_{\hat i_1}^1{:}\{c_1,\tilde x_{\hat i_1}^1\}, ~~\tilde x_{\hat i_1}^1{:}\{c_1,d_1\},\label{eq:clause1}\\
%&d_1{:}\{c_1,b_{n+1}\}, ~~c_1{:}\{b_{n+1},a_{n+1}\},\label{eq:var2clause}\\
%&b_{n+1}{:}\{a_{n+1},\tilde y_n^m\}, ~~a_{n+1}{:}\{\tilde y_n^m,\tilde x_n^m\}, ~~\tilde y_n^m{:}\{\tilde x_n^m,\tilde y_n^{m-1}\}, ~~ ..., ~~\tilde x_{n}^2 {:}\{\tilde y_{n}^1,\tilde x_{n}^1\}, ~~\tilde y_n^1{:}\{\tilde x_n^1,b_n\}, ~~\tilde x_n^1{:}\{b_n,a_n\},\label{eq:varn}\\
%&b_n{:}\{a_n,\tilde y_{n-1}^m\}, ~~a_n{:}\{\tilde y_{n-1}^{m},\tilde x_{n-1}^{m}\}, ~~\tilde y_{n-1}^m{:}\{\tilde x_{n-1}^m,\tilde y_{n-1}^{m-1}\},~~ ..., ~~\tilde x_{n-1}^2{:}\{\tilde y_{n-1}^1,\tilde x_{n-1}^1\}, ~~\tilde y_{n-1}^1{:}\{\tilde x_{n-1}^1,b_{n-1}\},\\
%&\quad\tilde x_{n-1}^1{:}\{b_{n-1},a_{n-1}\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&b_{2}{:}\{a_{2},\tilde y_{1}^m\}, ~~a_{2}{:}\{\tilde y_{1}^m,\tilde x_{1}^m\}, ~~\tilde y_1^m{:}\{\tilde x_1^m,\tilde y_1^{m-1}\},~~ ..., ~~\tilde x_1^2{:}\{\tilde y_1^1,\tilde x_1^1\}, ~~\tilde y_1^1{:}\{\tilde x_1^1,b_1\}, ~~\tilde x_1^1{:}\{b_1,a_1\},\label{eq:var1}\\
%&b_1{:}\{a_1,\beta\}, ~~a_1{:}\{\beta,\alpha\})
%\end{alignat}



%\begin{align}
%\nonumber(&\gamma{:}\{c_{m+1},c_m\},~ c_{m+1}{:}\{y_m^{i_{w_m}},c_m\},~ y_m^{i_{w_m}}{:}\{x_m^{i_{w_m}},c_m\},~ x_m^{i_{w_m}}{:}\{d_m,c_m\},~ d_m{:}\{c_m,c_{m-1}\},~ c_m{:}\{y_{m-1}^{i_{w_{m-1}}},c_{m-1}\},\\
%& ...,\\
%&c_2{:}\{y_1^{i_{w_1}},c_1\},~ y_1^{i_{w_1}}{:}\{x_1^{i_{w_1}},c_1\},~x_1^{i_{w_1}}{:}\{d_1,c_1\},~ d_1{:}\{c_1,b_{n+1}\},~c_1{:}\{b_{n+1},a_{n+1}\},~b_{n+1}{:}\{a_{n+1},y_n^m\},\label{eq:clauses}\\
%&a_{n+1}{:}\{y_n^m,x_n^m\},~ y_n^m{:}\{x_n^m,y_n^{m-1}\},~ ...,~ x_{n}^2 {:}\{y_{n}^1,x_{n}^1\},~ y_n^1{:}\{x_n^1,b_n\},~x_n^1{:}\{b_n,a_n\},~b_n{:}\{a_n,y_{n-1}^m\},\label{eq:varn}\\
%\nonumber&a_n{:}\{y_{n-1}^{m},x_{n-1}^{m}\},~ y_{n-1}^m{:}\{x_{n-1}^m,y_{n-1}^{m-1}\},~ ...,~ x_{n-1}^2{:}\{y_{n-1}^1,x_{n-1}^1\},~ y_{n-1}^1{:}\{x_{n-1}^1,b_{n-1}\},~ x_{n-1}^1{:}\{b_{n-1},a_{n-1}\},\\ 
%&b_{n-1}{:}\{a_{n-1},y_{n-2}^m\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&a_2{:}\{y_1^m,x_1^m\},~ y_m^1{:}\{x_1^m,y_1^{m-1}\},~ ...,~ x_1^2{:}\{y_1^1,x_1^1\},~ y_1^1{:}\{x_1^1,b_1\},~ x_1^1{:}\{b_1,a_1\},~
%b_1{:}\{a_1,\beta\},\label{eq:var1}\\ 
%\nonumber&a_1{:}\{\beta,\alpha\})
%\end{align}

%Here (\ref{eq:clausem}) corresponds to the portion of $P$ passing through clause $C_m$'s gadget, (\ref{eq:clausemm1}) to the portion passing through $C_{m-1}$'s gadget, (\ref{eq:clauses}) to the portion passing through the gadgets for clauses $C_{m-2},...,C_2$, (\ref{eq:clause1}) through clause $C_1$, (\ref{eq:var2clause}) to the connection from clause $C_1$'s gadget back to variable $x_n$'s gadget (\ref{eq:varn}) through variable $x_n$, (\ref{eq:varnm1}) through $x_{n-1}$, (\ref{eq:othervars}) through variables $x_{n-2},...,x_2$, and (\ref{eq:var1}) through $x_1$'s gadget.

Observe that for each {\em label$:$edge} entry number $k$ after $\gamma{:}\{c_{m+1},c_m\}$ (i.e., the one for iteration $\ell$), the entry's label is one of the two A-nodes occurring in entry $k-1$'s (i.e., the next entry's) edge.

Therefore iteration $k$'s removal of the then-isolated A-node $o_k$ removes the (only) label from entry $o_k{:}\{p_k,p_k'\}$'s edge, disconnecting that component to two, in time for iteration $k-1$. Note also that one of edge $\{p_k,p_k'\}$'s two endpoints (say, $p_k$) the {\em label} of the succeeding entry $o_{k-1}{:}\{p_{k-1},p_{k-1}'\}$ (i.e., $p_k=o_{k-1}$) and does not appear as an {\em endpoint} in any subsequent edge in the ordering. That is, at the start of the iteration $k$, $p_k$ is a leaf in the Ahograph. Therefore the removal of edge $\{p_k,p_k'\}$ means that $p_k = o_{k-1}$ is an isolated A-node at the start of iteration $k-1$. The remainder of that component within the Ahograph is of course still a tree, thus proving the inductive claim.

Since the BUILD algorithm running on $R'$ never encounters a connected Ahograph, it follows \cite{bryant1995extension} that $R'$ is consistent.
%
%%Therefore each removal of the next {\em label$:$edge} entry causes the isolation of the A-node appearing as the subsequent entry's label.
%
%%The initial Ahograph consists of two components, one of which is an isolated A-node ($\gamma$). It has $\ell$ edges, corresponding to $P$'s $\ell$ arcs. Every A-node appears (once) as a label, except for $\alpha$ and $\beta$. Thus the Ahograph has $\ell+2$ A-nodes, and its second component is a tree. Therefore each deletion of an edge from that second component increases the number of components by one.
%
%Finally, observe that in each iteration, the edge deleted is incident to a leaf, thus rendering it an isolated A-node.
%
%
%\textbf{HERE}
%
%
%If $o_k$ nonetheless is still not isolated, that means that triple $p_kq_k | o_k$ was not removed in the previous iteration. 
%
%in each iteration a new A-node $u_k$ becomes isolated
%
%encountering a new isolated A-node in each iteration, 
%
%
%as the process implicitly constructs a caterpillar tree (see Fig.\ \ref{fig:caterpillar}), thus implying that $R'$ is consistent.
\end{proof}







\begin{lemma}[$\Leftarrow$]\label{lem:isentailed}
%Let $A' \subseteq A$. 
Suppose there exists an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then there exists a subset $A' \subseteq A$ for which $R' = \text{triples}(A')$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
\end{lemma}
\begin{proof}
%Given such a path $P$, we construct the corresponding $R'=f(P)$. By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths as follows:
%\begin{eqnarray*}
%P &=& (\alpha\beta,e_1,\beta a_1, e_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (a_{n+1}b_{n+1},e_3,b_{n+1}c_1,e_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (c_{m+1}\gamma)
%\end{eqnarray*}
%Given such an arc set $P$, we construct the corresponding $R'=f(P)$. 
We choose $A' = P$, and set $R' = \text{triples}(A')$, which is consistent by Lemma \ref{lem:consistR}.
%By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths:
%\begin{eqnarray*}
%P &=& (e_1,e_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (e_3,e_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (e_5)
%\end{eqnarray*}
%where $P_{x_i}$ is one of the two length-$2m{+}2$ subpaths passing through $x_i$'s gadget (from $a_ib_i$ to $a_{i+1}b_{i+1}$), $P_{C_j}$ is one of the three length-4 subpaths passing through $C_j$'s gadget (from $c_jd_j$ to $c_jc_{j+1}$) and including the succeeding connecting arc, and $e_1,...,e_5$ are placeholder names for the other five connecting arcs. 
%More precisely, the paths $P_{x_i}$ and $P_{C_j}$ are all ``half-open'' paths, meaning that they start with a node and end with an arc: $P_{x_i}$ starting with $a_ib_i$ and ending with one of the two arcs {\em preceding} $a_{i+1}b_{i+1}$, and $P_{C_j}$ starting with $c_jd_j$ and edging with the (unique) arc {\em preceding} $c_{j+1}d_{j+1}$.
%where $P_{x_i}$ is the path passing through $x_i$'s variable gadget, $P_{C_j}$ is the path passing through $C_j$'s clause gadget, and $e_1,...,e_4$ are placeholder names for the four corresponding connecting arcs. More precisely, the paths $P_{x_i}$ and $P_{C_j}$ are all ``half-open'' paths, meaning that they start with a node and end with an arc: $P_{x_i}$ starting with $a_ib_i$ and ending with one of the two arcs {\em preceding} $a_{i+1}b_{i+1}$, and $P_{C_j}$ starting with $c_jd_j$ and edging with the (unique) arc {\em preceding} $c_{j+1}d_{j+1}$.

%Recalling that each 1-2-hyperarc represents a rooted triple in $R$, we add to $R'$ the triple corresponding to each arc appearing in $P$, i.e., $R' = \{r(e) : e \in P\}$, where $r(e)$ denotes the triple represented by $e$.

Let $\ell=|P|$, and for each $k \in [\ell]$, let $e_k = u_k{\to}\{v_k,v_k'\}$ denote the $k$th arc in $P$, with $u_k = p_kq_k$ and $\{v_k,v_k'\} = \{p_ko_k, q_ko_k \}$ (for some leaves $p_k,q_k,o_k$), representing triple $p_k q_k | o_k = u_k | o_k$. The names $v_\ell,v_\ell'$ can be assigned so that $v_\ell = c_{m+1}\gamma$ (and $v_\ell'$ is $e_\ell$'s non-destination sink node $c_m \gamma$), but we can also simply represent $e_\ell$ as $u_\ell|o_\ell = c_mc_{m+1} | \gamma$.
%so hyperarc $e_\ell = u_\ell{\to}\{v_\ell, v_\ell'\}$, representing triple $u_\ell|o_\ell = p_\ellq_\ell | o_\ell = c_mc_{m+1} | \gamma$. 
Similarly, for each $k \in [2,...,\ell]$, we can assign the names $v_{k-1},v_{k-1}'$ so that $v_{k-1}=u_k$, i.e., $\text{t}(e_k) = u_k = v_{k-1} \in \text{h}(e_{k-1})$,
%and so hyperarc $e_{k-1} = u_{k-1}{\to}\{u_k, v_{k-1}'\}$, representing triple $p_{k-1}q_{k-1} | o_{k-1} = u_{k-1}|o_{k-1}$.
and we can also simply represent $e_{k-1}$ as $u_{k-1}|o_{k-1}$.

Now consider arcs $e_{\ell-1}$ and $e_\ell$, and observe that their representations as $u_{\ell-1}|o_{\ell-1}$ and $u_\ell|o_\ell$ (respectively) are 
%$e_{\ell-1} = u_{\ell-1}{\to}\{u_\ell, v_{\ell-1}'\}$ and $e_\ell = u_\ell{\to}\{v_\ell, v_\ell'\}$, representing triples $u_{\ell-1}|o_{\ell-1}$ and $u_\ell|o_\ell$, respectively, and observe that this pair of triples is 
of exactly the form that dyadic inference rule (\ref{eq:2b}) applies to: via that inference rule---{\em assuming $R'$ is consistent}---we can infer the triple $u_{\ell-1}|o_\ell$, which have the form $c_m \tilde y_i^m | \gamma$ (for some $i$). % or $c_j \bar y_i^m | \gamma$.

%, where the names $v_k,v_k'$ are assigned so that $v_k$ is $u_k$'s successor on $P$, i.e., $v_k = u_{k+1}$ (except when $k=\ell$, in which case $v_k=c_{m+1}\gamma$), and therefore, $u_k=v_{k-1}$, i.e., $u_k = \text{t}(e_k) \in \text{h}(e_{k-1}) = \{v_{k-1},v_{k-1}'\}$
%
%That is, $\text{t}(e_k) = p_kq_k$, and $o_{k-1} \in \{p_k, q_k\}$ and $|\{p_k, q_k\} \cap \{p_{k-1}, q_{k-1}\}|=1$, and so $e_k$ represents $p_k q_k | o_k$. Then observe that by applying the second dyadic inference rule (recall Def.\ \ref{def:2ord}) to the triples represented by the path's last two arcs (i.e., $p_{\ell-1} q_{\ell-1} | o_{\ell-1}$ and $p_\ell q_\ell | o_\ell$), we can infer $p_{\ell-1} q_{\ell-1} | o_\ell$. 

Similarly, by applying this inference rule to the triple represented $P$'s third-to-last arc (i.e., $u_{\ell-2} | o_{\ell-2}$) and the derived triple  $u_{\ell-1} | o_\ell$, we can infer $u_{\ell-2} | o_\ell$. Via a total of $\ell-1$ such applications of dyadic inference rule (\ref{eq:2b}) (each corresponding to one BUILD iteration), we can derive $u_1 | o_\ell = p_1 q_1 | o_\ell$ = $\alpha \beta | \gamma$.
%
%Second, by Lemma \ref{lem:consistR} proved below, $R'$ is indeed consistent.
\end{proof}





%mpj
%\newpage


%mpj
\begin{figure}%[t!]
\centering
	\begin{subfigure}{\textwidth}
\centering
%\input{triples-fig-var-leaves}
%\captionsetup{justification=centering}
%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%\input{triples-fig-tree}
\makebox[1\textwidth][c]{ %\hskip -2cm
\includegraphics[width=1.15\textwidth]{rt-fig-ahograph-arx.pdf}
}
%\vskip .05cm
%\vskip -.05cm
\caption{The initial Ahograph $[R',L(R')]$ constructed based on an underlying {\em acyclic} path $P$. Because $P$ is acyclic, the node  $\tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j$ pointed to by each $C_j$'s witness node $c_j \tilde x_{\hat i_j}^j$ is a {\em sink node in $H$}, and thus A-nodes $\tilde y_i^j$ and $\tilde x_i^j$ are {\em leaves in the Ahograph}. As a result, at each BUILD iteration, the Ahograph has two components, a tree and an isolated node.
%, distinct from the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets.% (as occurs in Fig.\ \ref{fig:ahocycle}).
%
%Because $P$ is acyclic, 
%, where $P$ is an acyclic path in the hypergraph from $\alpha\beta$ to $c_{m+1}\gamma$,
%%(specifically, the red path shown in Fig.\ \ref{fig:overview}), 
%and $R'=\text{triples}(P)$. 
%%Here $x_2$ is false and $x_1,x_3,x_4$ are true, and the witness literals for clauses $C_1,C_2,C_3,C_4$ are $\bar x_n, \bar x_1, \bar x_n, \bar x_1$, respectively. 
%%If $P$ had contained a cycle involving some clause $C_j$, then $C_j$'s $x$ and $p$ nodes in the resulting Ahograph would have 
%Let $\tilde x_i^j \tilde y_i^j$ be the variable gadget node pointed to by the $C_j$ clause's witness node. Then, because $P$ is acyclic, A-nodes $\tilde x_i^j$ and $\tilde y_i^j$ are both leaves {\em in the Ahograph}, rather than appearing in the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets (as occurs in Fig.\ \ref{fig:ahocycle}).
}
\label{fig:ahograph}
%\end{figure}
%\begin{figure}[t!]
\end{subfigure}
\vskip .5cm
\centering
	\begin{subfigure}{\textwidth}
\centering
%\captionsetup{justification=centering}
%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%\input{triples-fig-tree}
\includegraphics[width=.75\textwidth]{rt-fig-ahocycle-arx.pdf}
%\vskip .05cm
%\vskip -.05cm
\caption{A fragment of the Ahograph resulting from the cause of a cycle in $P$, viz., a back-arc in which some clause $C_j$'s witness node $c_j \bar x_i^j$ points to a {\em non-sink} node $\bar x_i^j \bar y_i^j$ that lies earlier in the path $P$ (specifically, within $x_i$'s gadget), and thus A-nodes $\tilde y_i^j$ and $\tilde x_i^j$ are {\em non-leaves} in the Ahograph. This yields the triangle $c_j-\bar y_i^j - \bar x_i^j$. After the BUILD iteration in which A-node $c_{j+1}$ and edge $c_j\bar y_i^j$ are removed, $\bar y_i^j$ will still {\em not} be isolated, and hence the Ahograph will at that point consist of a single component, indicating $R'$ is inconsistent.
%Ahograph $[R',L(R')]$, where $P$ is an acyclic path in the hypergraph from $\alpha\beta$ to $c_{m+1}\gamma$ (specifically, the red path shown in Fig.\ \ref{fig:overview}), and $R'=\text{triples}(\text{arcs}(P))$. Here $x_2$ is false and $x_1,x_3,x_4$ are true, and the witness literals are $\bar x_n, \bar x_1, \bar x_n, \bar x_1$ for clauses $C_1,C_2,C_3,C_4$, respectively. 
%%If $P$ had contained a cycle involving some clause $C_j$, then $C_j$'s $x$ and $p$ A-nodes in the resulting Ahograph would have  
%Because $P$ is acyclic, each clause $C_j$'s $x$ and $p$ A-nodes are leaves {\em in the Ahograph}, rather than being A-nodes in the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets. 
}
\label{fig:ahocycle}
\end{subfigure}
\caption{The Ahograph $[R',L(R')]$ is constructed when Aho et al.'s BUILD algorithm is executed on the triples $R' = \text{triples}(P)$ corresponding to the path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$. The existence of any cycle within $P$ involving some clause $C_j$'s witness node $c_j \tilde x_{\hat i_j}^j$ pointing to $\tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j$ (i.e., arc $c_j \tilde x_{\hat i_j}^j \to \{c_j \tilde y_{\hat i_j}^j, \tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j\}$) will be reflected in the locations in the Ahograph of A-nodes $\tilde y_{\hat i_j}^j$ and $\tilde x_{\hat i_j}^j$.}
\end{figure}







\begin{figure}[t!]
\centering
\makebox[1\textwidth][c]{ %\hskip -2cm
  \begin{subfigure}[t]{.35\linewidth}
    \centering
%    \captionsetup{width=.9\linewidth}%
    \includegraphics[height=.5\textheight]{rt-fig-pathtree-arx.pdf}
\caption{The (unique) caterpillar tree determined by the triples corresponding to $P$, which thence satisfies $\alpha\beta|\gamma$.
\label{fig:pathtree}
}
  \end{subfigure}
\hskip .35cm
  \begin{subfigure}[t]{.79\linewidth}
    \centering
    %\captionsetup{width=1.1\linewidth}%
    \includegraphics[height=.5\textheight]{rt-fig-nopathtree-arx.pdf}
\caption{A tree consistent with $A'$, i.e., displaying all of $R'=\text{triples}(A')$, but {\em not} displaying $\alpha \beta | \gamma$.
%The tree that can be constructed displaying all triples in $R'=\text{triples}(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. 
The root's left subtree contains all leaves appearing in A-nodes before the ``directed cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
\label{fig:nopathtree}
}
  \end{subfigure}
 }
%
%
%%\captionsetup{justification=centering}
%%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%%\input{triples-fig-tree}
%\includegraphics[height=.5\textheight]{triples-fig-pathtree.pdf}
%%\vskip .05cm
%\vskip -.1cm
%\caption{The caterpillar tree resulting from the triples corresponding to $P$, which thence satisfies $\alpha\beta|\gamma$.}
%\label{fig:caterpillar}
%\vskip .1cm
%\centering
%%\captionsetup{justification=centering}
%%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%%\input{triples-fig-tree}
%\includegraphics[height=.5\textheight]{triples-fig-nopathtree.pdf}
%%\vskip .05cm
%%\vskip -.05cm
\caption{Trees resulting from triples corresponding to an acyclic arc set $A' \subseteq A$ in $H$ that (a) does or (b) does not contain a path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%The tree that can be constructed displaying all triples in $R'=\text{triples}(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. The root's left subtree contains all leaves appearing in A-nodes before the ``directed cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
}
\end{figure}




























\subsection{Consistent Entailing Subset $\Rightarrow$ Acyclic Path}

We prove the contrapositive, via a proof that will depend on two subsequent lemmas proved below.

\begin{lemma}[$\Rightarrow$]\label{lem:notentailed}
%If $R'$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$, then $A' = \text{arcs}(R')$ contains the arcs of an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%
%Let $A' \subseteq A$. 
Suppose there is no acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then for every subset $A' \subseteq A$, $R' = \text{triples}(A')$ is {\em not} a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
%If $A' \subseteq A$ is {\em not} an acyclic arc set subsuming the set $P$ of arcs appearing in some path from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \text{triples}(A')$ is not a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
\end{lemma}
\begin{proof}
%Given such a subset $R'$, we construct the corresponding $P=f^{-1}(R')$.
Let $A' \subseteq A$ be an arbitrary subset of $A$, and set $R' = \text{triples}(A')$.

First, suppose there {\em is} a path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then $P$ must be cyclic, and thus $\text{triples}(P) \subseteq R'$ will be inconsistent. Intuitively, it can be seen that any (directed) cycle in $H$ corresponds to a vicious (inconsistent) cycle of rooted triples. In particular (see Fig.\ \ref{fig:ahocycle}), any clause $C_j$'s component whose witness node points to a variable gadget node already visited on the path (causing a simple cycle in $H$) will induce a triangle {\em in the Ahograph}, resulting in a single-component Ahograph in the corresponding iteration of the BUILD algorithm (if no single-component Ahograph is encountered in an earlier iteration).

Second, suppose there is no path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ having $P \subseteq A$, cyclic or otherwise. If $A'$ is cyclic then $R' = \text{triples}(A')$ will again be inconsistent, so assume $A'$ is acyclic. Now we will show constructively that in this case, $R'$ does not entail $\alpha\beta|\gamma$.

Let $S(\alpha \beta,V,R') \subseteq V$ (written $V_{\alpha\beta}$) be the set of all nodes reachable from $\alpha \beta$ via the nodes $V$ and the arcs $A'$ and let $P(c_{m+1}\gamma,V,R') \subseteq V$ (written $V_{c_{m+1}\gamma}$) be the set of all nodes that $c_{m+1}\gamma$ is reachable {\em from} via $V$ and $A'$, and set $V' = V_{\alpha\beta} \cup .V_{c_{m+1}\gamma}$ Then by assumption $V_{\alpha\beta}$ and $V_{c_{m+1}\gamma}$ are disjoint. That is, the hypergraph $(V',A')$ has two components.

Let $V_{\alpha \beta}^* \subseteq V_{\alpha\beta}$ be the maximal elements of $V_{\alpha\beta} $ in the sense that every $u \in V_{\alpha \beta}^*$ is reachable from $\alpha\beta$ but no other node $v \in V_{\alpha\beta}$'s reachability {\em depends on} $u$. That is, $S(\alpha \beta,V-\{u\},R') = S(\alpha \beta,V,R') - \{u\}$. Similarly, let $V_{c_{m+1}\gamma}^* \subseteq V_{c_{m+1}\gamma}$ be the minimal elements of $V_{c_{m+1}\gamma}$ in the sense that for any $v \in V_{c_{m+1}\gamma}^*$, there is no other node $u \in V_{c_{m+1}\gamma}$ dependent on $v$, i.e., $P(c_{m+1}\gamma,V-\{v\},R') = P(c_{m+1}\gamma,V,R')-\{v\}$.

By Lemma \ref{lem:uvpairs} proved below, we can assume wlog that there are at most 3 $u^*$s and at most 3 $v^*$s, which together yield either 1, 2, or 3 pairs $(u_h,v_h)$, with each pair connected by an arc $e_h \in  A - A'$.

Then by Lemma \ref{lem:treeexs} proved below, we can build a tree displaying $\text{triples}(A') \cup \{\alpha\gamma | \beta\}$ (see Fig.\ \ref{fig:nopathtree}). This shows that $R' \cup \{\alpha\gamma | \beta\}$ is consistent, and thus that $R'$ does not entail $\alpha\beta | \gamma$.
%
%
%
%
%
%
%%\textbf{but then there's a tree satisfying $R'$ and not $\alpha\beta|\gamma$}
%
%
%First observe that the only triple in $R$ including $\alpha$ or $\beta$ is $\alpha\beta | a_1$, and so any hypothetical subset $R' \subset R$ pseud o-entailing $\alpha\beta|\gamma$ must necessarily include $\alpha\beta | a_1$.  But then observe that the only other triple in $R$ including $\alpha$ or $\beta$ is $\beta a_1 | b_1$, so it must be included. Next, observe that the only other triples in $R$ including $\beta$ or $a_1$ are $a_1b_1 | x_i^1$ and $a_1b_1 | \bar x_i^1$, so at least one of them must be included. We claim that by repeated application of arguments of this kind, we obtain that the arcs corresponding to the triples of any such $R'$ must trace out a path from $\alpha\beta$ to $c_{m+1}\gamma$.
%
%Second, observe that if $P$ contained a cycle, then the triples corresponding to the hyperarcs appearing in that cycle would themselves be inconsistent, contradicting the consistency of $R'$.
\end{proof}






\begin{lemma}\label{lem:uvpairs}
Let $A'$ be acyclic, suppose there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. and let $V_{\alpha \beta}^* \subseteq V_{\alpha\beta}$ and $V_{c_{m+1}\gamma}^* \subseteq V_{c_{m+1}\gamma}$ be defined as in the proof of Lemma \ref{lem:notentailed} above. Then $|V_{\alpha \beta}^*| = |V_{c_{m+1}\gamma}^*| \in [3]$, 
%and there is bijection between $V_{\alpha \beta}^*$ and $V_{c_{m+1}\gamma}^*$, with each pair corresponding to a unique edge in $A-A'$.
%By Lemma \ref{lem:uvpairs} proved below, we can assume wlog that there are at most 3 $u^*$s and at most 3 $v^*$s, 
which together yield $w \in [3]$ pairs $\{(u_h,v_h) : h \in [w]\}$, with each pair connected by an arc $e_h \in  A - A'$.
\end{lemma}
\begin{proof}
First, we claim we can assume wlog that for no $u \in V_{\alpha\beta}$ will the path to it from $\alpha\beta$ cross a back-arc, i.e., a subpath taking an arc of the form $c_j \tilde x_i^j{\to}\{c_j\tilde y_i^j, \tilde x_i^j\tilde y_i^j\}$ to $\tilde x_i^j\tilde y_i^j$ (see Fig.\ \ref{fig:clause}). Preceding $c_j \tilde x_i^j$, the path would have had to visit $c_jd_j$, and if after crossing the back-arc the path is going to eventually reach $c_{m+1}\gamma$, then it would have to visit $c_jd_j$ again, making it cyclic and $R'$ inconsistent.

Second, we claim we can assume wlog that no $v^*$'s path to $c_{m+1}\gamma$ will contain back-arcs.
%, i.e., a subpath taking an arc of the form $c_j \tilde x_i^j{\to}\{c_j\tilde y_i^j, \tilde x_i^j\tilde y_i^j\}$ to $\tilde x_i^j\tilde y_i^j$. 
To see this, consider what node $v^*$ could possibly benefit (in terms of reaching $c_{m+1}\gamma$) from such a path. If $v^*=c_jd_j$ (or any predecessor it it), then the path from $v^*$ to $c_{m+1}\gamma$ would again have to eventually return to $c_jd_j$ again, making the path cyclic. If $v^*= c_jx_i^j$, then it is not impossible per se for there to be an acyclic path from it to $c_{m+1}\gamma$ traversing the specified subpath. The only possible arc that could be used for reaching $c_jx_i^j$, however, is the one from $c_jd_j$, in which case once again the resulting path from $\alpha\beta$ to $c_{m+1}\gamma$ would be cyclic.

Now, how far are the maximal elements $V_{\alpha\beta}$ away from the minimal elements $V_{c_{m+1}\gamma}^*$? That is, how many arcs from $A$ would have to be added to $A'$ in order to reach a node $v^* \in  V_{c_{m+1}\gamma}^*$ from a node $u^* \in V_{\alpha \beta}^*$?

Since our goal is to show that $R'$ does {\em not} entail $\alpha \beta | \gamma$, we assume wlog the most difficult case, i.e., that any $v^* \in V_{c_{m+1}\gamma}^*$ is only one hop away from some $u \in V_{\alpha \beta}$, via some arc $e \in A - A'$, the addition of which to $A'$ would complete a path from $\alpha\beta$ to $c_{m+1}\gamma$. Conversely, we can assume wlog that for every $u^* \in V_{\alpha \beta}^*$ there exists an edge $e \in A-A'$ that would connect it to some $v \in V_{c_{m+1}\gamma}$. If $A_\times$ is the set of all arcs $e$ playing this role for some $u^*$ and/or $v^*$, then observe that $(V_{\alpha \beta}^*,V_{c_{m+1}\gamma}^*)$ is a {\em directed cut} separating $\alpha\beta$ from $c_{m+1}\gamma$ in the hypergraph $(V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^*, A' \cup A_\times)$, and $A_\times$ consists of the forward cross-arcs of that cut.

Now, how many arcs could there be in $A_\times$? By inspection of the hypergraph construction, it can be seen that $|A_\times|$ will be either 2, 3, or 1, depending (respectively) on whether the cut occurs within a variable gadget, within a clause gadget, or elsewhere. 
%Note also that due to hypergraph construction there will be a bijection between $u^*$s and $v^*$s. To see this, recall that the only arcs in which both heads are non-sink nodes are those in which a clause gadget's witness node $c_j \tilde x_i^j$ points back to a variable gadget node $\tilde x_i^j \tilde y_i^j$. But we have seen that no $u^*$'s path will contain a back-arc. Therefore if $A_\times$ contains an edge of the form $c_j \tilde x_i^j{\to}\{c_j \tilde y_i^j, \tilde x_i^j \tilde y_i^j\}$, it must be due to $u^*=c_j \tilde x_i^j$ and $v^*=c_j \tilde y_i^j$.
\end{proof}















\begin{lemma}\label{lem:treeexs}
Let $A'$ be acyclic, suppose there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$, and let $V_{\alpha \beta}^* \subseteq V_{\alpha\beta}$ and $V_{c_{m+1}\gamma}^* \subseteq V_{c_{m+1}\gamma}$ be defined as in the proof of Lemma \ref{lem:notentailed} above, and let $|V_{\alpha \beta}^*| = |V_{c_{m+1}\gamma}^*| \in [3]$, 
%where is bijection between $V_{\alpha \beta}^*$ and $V_{c_{m+1}\gamma}^*$, with each pair corresponding to a unique edge in $A-A'$.
which together yield $w \in [3]$ pairs $\{(u_h,v_h) : h \in [w]\}$, with each pair connected by an arc $e_h \in  A - A'$.
Then there exists a tree displaying $R' \cup \{\alpha\gamma | \beta\}$.
\end{lemma}
\begin{proof}
%Now we will show that for such an $A''$, $R' = \text{triples}(A'')$ is compatible with $\alpha\beta | \gamma$ not holding.
%
%Let $w \in [3]$ be the number of pairs $(u_h^*,v_h^*)$. 
There must be some latest common predecessor node $u_0$ of $\{u_h : h \in [w]\}$ and some earliest common successor node $v_4$ of $\{v_h : h \in [w]\}$. Let the (possibly empty) sequence of intermediate nodes on the path from $p$ to $u_h$ be $U_h = (u_h^1,...,u_h^{\ell_h})$, and the (possibly empty) sequence of intermediate nodes on the path from $v_h$ to $v_4$ be $V_h = (v_h^{1},...,v_h^{\ell_h'})$ Observe that each node $u_w^h$'s outgoing arc introduces one more leaf appearing in the triple's LHS, and so $U_h$ corresponds to $\ell_h$ such leaves, say, $p_h^1,...,p_h^{\ell_h}$. Each node $v_h^h$'s outgoing arc similarly introduces one more leaf in the triple's LHS, except for $v_1^1$, which introduces {\em two} more, because the leaf it shares in common with $u_w$ is also appearing on the LHS of a triple for the first time, due to $u_w$'s missing outgoing cross-arc, for a total of $\ell_h'+1$ such leaves, say, $q_h^0,...,q_h^{\ell_h'}$. Let $p_0$ be the leaf introduced by node $u_0$ and $q_4$ the leaf introduced by node $v_4$.

Then observe that $\{p\} \cup \bigcup_{f \in [w]} U_h$ can be put in a linear order, and hence $S(\alpha\beta,V,R')$ can as well. Let $L_S$ be the set of all leaves appearing in tail nodes of paths between $\alpha\beta$ and members of $V_{\alpha\beta}$, i.e., the leaves appearing in nodes $V_{\alpha\beta} - \{U_h^{\ell_h} : h \in [w]\}$. Then can we construct a caterpillar tree $C_S$ having leaves $L_S$ (see root's left subtree in Fig.\ \ref{fig:nopathtree}, except ignoring the appearance of $\gamma$ for a moment).

Similarly, observe that $\{s\} \cup \bigcup_{h \in [w]} V_h$ and hence $V_{c_{m+1}\gamma}$ can also be linearly ordered, and so if we define $L_P$ as the set of all leaves appearing in tail nodes of paths between members of $V_{c_{m+1}\gamma}$ and $c_{m+1}\gamma$,  i.e., the leaves appearing in nodes $V_{c_{m+1}\gamma} - \{c_{m+1}\gamma\}$, then we can also construct a caterpillar tree $C_P$ with leaves $L_P$ (see right subtree in Fig.\ \ref{fig:nopathtree}).

Now create a root node, whose children are the roots of $C_P$ and $S_P$. This resulting tree contains every leaf but $\gamma$, and observe that it displays every triple of $R'$ except (obviously) $c_m c_{m+1} | \gamma$.

Finally, we subdivide the tree's edge to $\alpha$ and add $\gamma$ as the second child of the tree's new inner node, with the result that the tree now displays $c_j c_{j+1} | \gamma$ and the rest of the triples of $R'$, as desired, yet also displays $\alpha \gamma | \beta$.
\end{proof}



%\textbf{start quotes:}
%
%%{\em Q: how do we know that a subset entailing $\alpha\beta|\gamma$ must necessarily correspond to a path?}
%
%\begin{lemma}[Bryant and Steel,  Prop. 9(1)]\label{lem:noabctrip} If $R$ is a closed set of rooted triples containing no triple with
%the leaves $\{a,b,c\}$ then $R \cup \{ab|e\}$, $R \cup \{ae|b\}$ and $R \cup \{be|a\}$ are all compatible.
%\end{lemma}
%
%{\em Q: can we get that entailment must follow a path by repeated (inductive) application of Lemma \ref{lem:noabctrip}?}
%
%\textbf{\em Q: is the consistency and/or the closure of a path in this construction actually somehow just obvious based on the construction?}
%\textbf{end quotes}





%\begin{lemma}[$\Leftarrow$]
%If there is a consistent triple set $R'$ entailing $\alpha\beta|\gamma$, then there is an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%%
%%Or: If there is no acyclic path from $ab$ to $ac$, then there is no consistent subset entailing $\alpha\beta|\gamma$.
%\end{lemma}
%\begin{proof}
%%First observe that the only triple in $R$ including $\alpha$ is $\alpha\beta | a_1$, and so any hypothetical subset $R' \subset R$ entailing $\alpha\beta|\gamma$ must necessarily include $\alpha\beta | a_1$.  But then observe that the only other triple in $R$ including $\beta$ is $\beta a_1 | b_1$. By repeated application of similar arguments, we obtain that the hyperarcs corresponding to the triples of any such $R'$ must trace out a path from $\alpha\beta$ to $c_{m+1}\gamma$.
%
%Second, observe that if the path contained a cycle, then the triples corresponding to the hyperarcs appearing in that cycle would themselves be inconsistent, contradicting the consistency of $R'$.
%%the portion of the Ahograph induced by everything from the start of the caterpillar up to the cycle's back-arc would be a single component.
%%
%%That is, if we pluck off the sink nodes one by one, then plucking off the node just following the back-arc will reduce the number of components from 2 to 1, indicating that $R$ is inconsistent.
%%
%%Does it suffice to argue that for any path from $ab$ to $ac$, if the path is acyclic then it implies a consistent subset entailing $\alpha\beta|\gamma$?
%%
%%\textbf{That is, can we assume that entailment will imply a path?}
%\end{proof}




%\begin{lemma}[$\Rightarrow$]
%If there is an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$, then there is a satisfying truth assignment.
%\end{lemma}
%\begin{proof}
%We read off the truth assignment from the choices the path makes passing through the series of variable gadgets. Because the path is acyclic, we know that in the case of each clause gadget it passes through, the node within the variable gadget pointed to is on the side of the variable gadget that the path did {\em not} use. Since we set the variable's truth value based on which side we did not use, this implies that the corresponding literal in the clause gadget is true, thus satisfying the clause.
%\end{proof}

Combining the Lemmas \ref{lem:isentailed} and \ref{lem:notentailed} with Theorem \ref{thm:apdh}, we conclude:

\begin{theorem}
\entailprob\:is NP-Complete.
\end{theorem}

And because computing the closure reduces to deciding whether $R \vdash t$ for $O(|L|^3)$ triples $t$, we also have:

\begin{corollary}
\closureprob\:is NP-hard.
\end{corollary}


%Also:
%
%\begin{corollary}
%The complementary problem, of deciding whether a triple is entailed by {\em every} consistent subset of $R$ is co-NP-Complete.
%\end{corollary}
%\begin{proof}
%Solve the original problem for both negations of the triple.
%\end{proof}


==> rt-proof-arx_copy_2.tex <==
% !TEX root = rootedtriples-arx.tex

\section{The Proof}

Clearly \entailprob\ is in NP: if we guess the subset $R' \subset R$, then we can verify both that $R'$ is consistent and that $R' \vdash t$ by executing Aho et al.\ \cite{aho1981inferring}'s polynomial-time BUILD algorithm on $R'$ \cite{bryant1995extension}. \minapdh\:is as well: guess the path, and check that it is acyclic.

Now we prove hardness, arguing that $R$ contains a consistent subset entailing $\alpha\beta|\gamma$ iff $H$ contains an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ iff $F$ admits a satisfying assignment $\mathbf{v}(\cdot)$, in two steps.



First we argue that acyclic paths correspond to satisfying truth assignments.
%\textbf{3SAT} reduces to \apdh\:(which is therefore NP-Complete):


\subsection{Acyclic Path $\Leftrightarrow$ Satisfying Truth Assignment}

\begin{lemma}
There is an an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ iff $F$ admits a satisfying truth assignment $\mathbf{v}(\cdot)$.
%If there is a satisfying truth assignment, then there is an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$.
\end{lemma}
\begin{proof}
($\Leftarrow$)
We construct $P$ based on the satisfying truth assignment $\mathbf{v}(\cdot)$. For each $x_i$, if $\mathbf{v}(x_i) =$ true, then we have $P$ take the $x_i$ gadget's {\em negative} side (drawn lower in Fig.\ \ref{fig:var}); otherwise, we have $P$ take its {\em positive} side (drawn higher). Then within each $C_j$, among the three possible witness paths, we choose one corresponding to the appearance of a literal that is true under $\mathbf{v}(\cdot)$ (which by assumption must exist).
%, which therefore points only to sides of variable gadgets that $P$ did {\em not} take. 
For the remainder of $P$ we have it take the required connecting arcs.

Notice that any potenial cycle contained within $P$ must necessarily involve an arc $e$ whose tail lies within some clause $C_j$'s gadget and one of whose heads lies within some variable $x_i$'s gadget. But the witness path taken within $C_j$'s gadget corresponds to an appearance $\tilde x_i^j$ of a true literal $\tilde x_i$. If it a positive literal, i.e., $\tilde x_i=x_i$, then $\mathbf{v}(x_i) =$ true, and we would have had $P$ take the $x_i$ gadget's {\em negative} side---not the side $e$ is pointing to. Similarly, if $\tilde x_i=\bar x_i$, then $\mathbf{v}(x_i) =$ false, $P$ would have taken the $x_i$ gadget's {\em positive} side, which again is then not the side $e$ is pointing to. Thus $P$ must be acyclic.

($\Rightarrow$)
We read off $\mathbf{v}(\cdot)$ from the choices the path $P$ makes when passing through the series of variable gadgets, i.e., setting $\mathbf{v}(x_i) = $ true if $P$ used the $x_i$ gadget's {\em negative} side, and setting it to false otherwise. Now, consider a clause $C_j$'s gadget, whose witness node points to a node $v'$ within some variable $x_i$'s gadget. Because $P$ is acyclic, we know that $v'$ is on the side of $x_i$'s gadget that $P$ did {\em not} use. Since we chose the truth value $\mathbf{v}(x_i)$ that makes literals within nodes on the $x_i$ gadget's {\em unused} side true, this implies that literal corresponding to $C_j$'s witness node is true, thus satisfying the clause.
\end{proof}

Thus we have proven:

\begin{theorem}\label{thm:apdh}
\minapdh\:is NP-Complete.
\end{theorem}

Since an infeasible solution is defined to have infinite cost, an algorithm with {\em any} approximation factor would allow us to distinguish between positive and negative problem instances, which immediately implies:
\begin{corollary}
Approximating \minapdh\:to within {\em any} factor is NP-hard.
\end{corollary}

Even if we restrict ourselves to problem instances admitting feasible solutions, this ``promise problem" \cite{goldreich2005promise} special case is hard to approximate within any reasonable factor.

%More formally, we obtain the following hardness of approximation.

\begin{corollary}
%In the promise problem \cite{goldreich2005promise} special case in which an acyclic B-hyperpath is assumed to exist, approximating \minapdh\:to within factor $|V|^{1-\epsilon}$ for any $\epsilon>0$ is NP-hard.
\minapdhprom\:is NP-hard to approximate to within factor $|V|^{1-\epsilon}$ for all $\epsilon>0$.
\end{corollary}
\begin{proof}
Let $\epsilon \in (0,1/4)$. Let $I = \langle H,u,v \rangle$ be an instance \minapdhprom. For this proof only, let $n=|V(H)|$.
We extend $H$ to a new hypergraph $H'$ by adding polynomially many dummy edges forming an acyclic $u{\to}v$ path of length $n^{\lceil1+1/\epsilon\rceil}$, yielding a hypergraph $H'$ with $n' = n+n^{\lceil1+1/\epsilon\rceil}-1$ nodes and a new problem instance $I' = \langle H',u,v \rangle$, which is also by construction a valid problem instance of \minapdhprom. If $H$ has a path ($I$ is a positive instance), then $H'$ (like $H$) has one of some length $OPT^+ \le n-1$; if not ($I$ is a negative instance), then $H'$'s only path has length $OPT^- = n^{\lceil1+1/\epsilon\rceil}$.

Now, suppose there were a $|V|^{1-\epsilon}$-approximation algorithm.

Running it on the $I'$ resulting from a negative $I$ will yield a path of length at least $LB^- = OPT^- = n \cdot n^{\lceil1/\epsilon\rceil}$.

Running it on the $I'$ resulting from a positive $I$ will yield a path of length of at most
\begin{align*}
UB^+ &= n'^{1-\epsilon}\cdot (n-1)\\
&= (n+n^{\lceil1+1/\epsilon\rceil}-1)^{1-\epsilon}\cdot (n-1)\\
& < (n-1) \cdot n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)} + (n-1)^{2-\epsilon}\\
&< n \cdot n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)},
\end{align*}
where the last inequality follows from the fact that $(n-1)^{2-\epsilon} < n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)}$ for $\epsilon<1/4$.

Because $\lceil1+1/\epsilon\rceil\cdot(1-\epsilon) = 1+\lceil1/\epsilon\rceil - \epsilon - \epsilon \lceil 1/\epsilon \rceil < \lceil 1/\epsilon \rceil$, it follows that $UB^+ < LB^-$.

%$\lceil1/\epsilon\rceil$ vs $\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)$
%
%$\lceil1/\epsilon\rceil$ vs $\lceil1/\epsilon\rceil\cdot(1-\epsilon) + (1-\epsilon)$
%
%$\lceil1/\epsilon\rceil$ vs $\lceil1/\epsilon\rceil - \lceil1/\epsilon\rceil\cdot\epsilon + (1-\epsilon)$
%
%0 vs $- \lceil1/\epsilon\rceil\cdot\epsilon + (1-\epsilon)$
%
%$\lceil1/\epsilon\rceil\cdot\epsilon > (1-\epsilon)$

Thus by comparing the length $ALG$ of the path in $H'$ found by the hypothetical algorithm to $UB^+$ and $LB^-$, we can decide whether $I$ was positive or negative.
%
%Then any algorithm providing an $f(|V|)$-approximation would allow us to distinguish (for $|V|$ sufficiently large) between instances $H'$ with optimal solution cost $<f(|V|)\cdot|V|$ and those with optimal solution cost $\ge f(|V|) \cdot |V|^2$, thus deciding whether $H$ had a path.
\end{proof}




Second, to extend the reduction to \entailprob, we argue that $H$ is a faithful representation of $R$ in the sense that acyclic paths from $\alpha\beta$ to $c_{m+1}\gamma$ (or acyclic supersets of such paths) correspond to consistent subsets entailing $\alpha\beta|\gamma$, and vice versa.


\subsection{Consistent Entailing Subset $\Leftarrow$ Acyclic Path}

We prove this direction via two lemmas, proving that the set of triples corresponding to an acyclic path are consistent and entail $\alpha\beta|\gamma$, respectively.



\begin{lemma}\label{lem:consistR}
If $P$ is an acyclic path $P$ in the hypergraph from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \text{triples}(P)$ is consistent.
\end{lemma}
\begin{proof}
To prove $R'$ consistent, we 
%reinterpret the procedure we carried out in the proof of Lemma \ref{lem:isentailed} as implicitly executing 
step through the execution of Aho et al.\ \cite{aho1981inferring}'s BUILD algorithm on input $R'$, picturing the state of the resulting Ahograph (see Fig.\ \ref{fig:ahograph}) and the tree being constructed (see Fig.\ \ref{fig:pathtree}) as they progress over time.
%Specifically, each application of dyadic inference rule (\ref{eq:2b}), as we step through $P$ in reverse order, can be interpreted as one iteration (or recursive call) of BUILD.
Each iteration can be interpreted one application of dyadic inference rule (\ref{eq:2b}), as we step through $P$ in reverse order.

%, of stepping through $P$ in reverse, repeatedly applying dyadic inference rule (\ref{eq:2b})
%
%again step through $P$ in reverse, implicitly executing Aho et al.\ \cite{aho1981inferring}'s BUILD algorithm on input $R'$, picturing the state of the resulting Ahograph (see Fig.\ \ref{fig:ahograph}) and the tree being constructed (see Fig.\ \ref{fig:pathtree}) along the way. 

Observe that in Ahograph $[R', L(R')]$ (see Fig.\ \ref{fig:ahograph}), $\gamma$ will be an isolated A-node, since $R$ contains no triples with $\gamma$ on their LHSs,
%Just as dyadic inference rule (\ref{eq:2b}) carried us through to $\alpha\beta | \sigma$, 
%Observe also that by definition of $R'$, the A-nodes $L(R') - \{\gamma\}$ are connected in one component of Ahograph $[R', L(R')]$, 
and that the edge $\{c_m, c_{m+1}\}$ in $[R', L(R')]$ due to $P$'s last arc (representing $c_m c_{m+1} | \gamma$) is labeled (only) with $\gamma$. Isolated A-node $\gamma$ is removed for BUILD's second iteration, in which we recurse on the remaining A-nodes. The edge $\{c_m, c_{m+1}\}$ will therefore no longer appear in that iteration's Ahograph, $[R', L(R') - \{\gamma\}]$, rendering $c_{m+1}$ an isolated A-node.

We claim that this pattern will continue to obtain the rest of the way back to the start of $P$, with a new A-node becoming isolated  by the start of each iteration, causing an edge to be removed, and hence isolating another A-node for the succeeding iteration.
%
More precisely, number the iterations in reverse, counting downward from $\ell=|P|$, where iteration $\ell$ is the first iteration executed, in which because A-node $o_\ell$ is observed to be isolated, the Ahograph's edge $\{p_\ell,q_\ell\}$ due to triple $p_\ell q_\ell | o_\ell = c_m,c_{m+1} | \gamma$ is removed. 



Let $H_P$ be the subhypergraph of $H$ induced by the nodes $\{\text{t}(e) : {e \in P}\} \cup \{c_{m+1}\gamma\}$, and recall that nodes in $H$ correspond to unordered pairs of A-nodes, and thus to potential edges in the Ahograph.

Because $P$ is a path, each node in $H_P$ except $c_{m+1}\gamma$ (which has out-degree 0) will have out-degree 1. Therefore the Ahograph will have exactly $\ell$ edges, each with one label.
%
%%of $H$ induced by $P$ has out-degree at most one. Therefore no edge in the Ahograph has more than one label. Note that $\alpha$ and $\beta$ will not be labels of any edge.
%
Because $P$ is acyclic, each node in $H_P$ except $\alpha\beta$ (which has in-degree 0) will have in-degree 1. Therefore no label will appear on multiple edges in the Ahograph.
%
Thus there is a bijection between Ahograph's $\ell$ edges and the labels appearing on them.

Node $\alpha\beta$ contains two leaves, and each arc in $P$ introduces one additional leaf, for a total of $\ell+2$ leaves in $L(R')$, and hence $\ell+2$ A-nodes in the Ahograph.

Note also that the first arc in $P$ adds label $a_1$ to edge $\{\alpha,\beta\}$ in the Ahograph, and that each subsequent arc adds a label to an edge incident to the preceding edge, and so all the Ahograph's $\ell$ edges lie within a single component. Since $\gamma$ is an isolated A-node, this means that that component has exactly $\ell+1$ A-nodes, and is therefore a tree.

%To see this, suppose $c_j \tilde x_i^j{\to}\{\tilde x_i^j \tilde y_i^j, c_j \tilde y_i^j\}$ is a back-arc in $P$.
%
%there are no other edges in the Ahograph beyond those listed here.
%%
%Note also that no label appears on more than one edge. Therefore there is a one-to-one correspondence between the Ahograph's $\ell$ edge labels and $P$'s arcs. Every A-node appears (once) as a label, except for $\alpha$ and $\beta$. Thus the Ahograph has $\ell+2$ A-nodes, and its second component is a tree.

Now, we prove by induction that at the start of each iteration $k$ from $\ell$ down to $1$, the Ahograph consists of two components: some isolated A-node $o_k$ and a tree. We have already verified the base case: $o_\ell$ is isolated at the start, in iteration $\ell$, and the $\ell+1$ remaining nodes form a tree. Assume the claim is true for each iteration from $\ell$ down through some iteration $k$.

%If this is not true for every iteration, let $k$ be the first iteration at the start of which $o_k$ is not isolated. Now, we know that at the start the previous iteration (iteration $k+1$), $o_{k+1}$ (which is the right-hand side of triple $u_{k+1}|o_{k+1}$, where $o_k \in u_{k+1}$) was found to be isolated, and therefore was removed from the iteration-$k$ Ahograph. What does it mean if we find at the start of iteration $k$ that $o_k$ is still not isolated?
%
%The deletion of $o_{k+1}$ meant the removal of label $o_{k+1}$ from from the Ahograph of edge $u_{k+1}$, which contains $o_k$. If edge $u_{k+1}$ nonetheless remains in the Ahograph, this means that it still has some label.


%\begin{align}
%\nonumber(&\gamma{:}\{c_{m+1},c_m\},\\
%&c_{m+1}{:}\{\tilde y_{i_{w_m}}^m,c_m\},~\tilde y_{i_{w_m}}^m{:}\{\tilde x_{i_{w_m}}^m,c_m\},~\tilde x_{i_{w_m}}^m{:}\{d_m,c_m\},~ d_m{:}\{c_m,c_{m-1}\},~ c_m{:}\{\tilde y_{i_{w_{m-1}}}^{m-1},c_{m-1}\},\\
%& ...,\\
%&c_2{:}\{\tilde y_{i_{w_1}}^1,c_1\},~\tilde y_{i_{w_1}}^1{:}\{\tilde x_{i_{w_1}}^1,c_1\},~\tilde x_{i_{w_1}}^1{:}\{d_1,c_1\},~ d_1{:}\{c_1,b_{n+1}\},~c_1{:}\{b_{n+1},a_{n+1}\},~b_{n+1}{:}\{a_{n+1},\tilde y_n^m\},\label{eq:clauses}\\
%&a_{n+1}{:}\{\tilde y_n^m,\tilde x_n^m\},~\tilde y_n^m{:}\{\tilde x_n^m,\tilde y_n^{m-1}\},~ ...,~\tilde x_{n}^2 {:}\{\tilde y_{n}^1,\tilde x_{n}^1\},~\tilde y_n^1{:}\{\tilde x_n^1,b_n\},~\tilde x_n^1{:}\{b_n,a_n\},~b_n{:}\{a_n,\tilde y_{n-1}^m\},\label{eq:varn}\\
%\nonumber&a_n{:}\{\tilde y_{n-1}^{m},\tilde x_{n-1}^{m}\},~\tilde y_{n-1}^m{:}\{\tilde x_{n-1}^m,\tilde y_{n-1}^{m-1}\},~ ...,~\tilde x_{n-1}^2{:}\{\tilde y_{n-1}^1,\tilde x_{n-1}^1\},~\tilde y_{n-1}^1{:}\{\tilde x_{n-1}^1,b_{n-1}\},~\tilde x_{n-1}^1{:}\{b_{n-1},a_{n-1}\},\\ 
%&b_{n-1}{:}\{a_{n-1},\tilde y_{n-2}^m\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&a_2{:}\{\tilde y_1^m,\tilde x_1^m\},~\tilde y_m^1{:}\{\tilde x_1^m,\tilde y_1^{m-1}\},~ ...,~\tilde x_1^2{:}\{\tilde y_1^1,\tilde x_1^1\},~\tilde y_1^1{:}\{\tilde x_1^1,b_1\},~\tilde x_1^1{:}\{b_1,a_1\},~
%b_1{:}\{a_1,\beta\},\label{eq:var1}\\ 
%\nonumber&a_1{:}\{\beta,\alpha\})
%\end{align}



 
%Given such a path $P$, we construct the corresponding $R'=f(P)$. By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths as follows:
%\begin{eqnarray*}
%P &=& (\alpha\beta,e_1,\beta a_1, e_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (a_{n+1}b_{n+1},e_3,b_{n+1}c_1,e_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (c_{m+1}\gamma)
%\end{eqnarray*}
%Given such an arc set $P$, we construct the corresponding $R'=f(P)$. 
%We choose $A' = P$, and set $R' = \text{triples}(A')$, which is consistent by Lemma \ref{lem:consistR}.
By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths:
\begin{align*}
P &~=~ (e_1,e_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (e_3,e_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m},
\end{align*}
where $P_{x_i}$ is one of the two length-$2m{+}2$ subpaths passing through $x_i$'s gadget (from $a_ib_i$ to $a_{i+1}b_{i+1}$), $P_{C_j}$ is one of the three length-4 subpaths traversing one of the $C_j$ gadget's three witness paths (from $c_jd_j$ to $c_jc_{j+1}$) {\em plus the succeeding arc with tail $c_jc_{j+1}$}, and $e_1,...,e_4$ are shorthand names for the other four connecting arcs.





For each $C_j$, let $\hat i_j$ denote the index $i$ of the variable $x_i$ appearing in the witness path of $C_j$ (through literal appearance $\tilde x_{\hat i_j}^j$) that $P$ traverses.

Now, consider the following {\em reverse linear ordering} of the A-node-labeled edges of Ahograph $[R', L(R')]$, with each subsequence of A-node-labeled edges is tagged to indicate the corresponding subpath of $P$ (compare to Figs.\ \ref{fig:ahograph} and \ref{fig:overview}, and in particular compare each ($P_{C_j}$) to Fig.\ \ref{fig:clause} and each ($P_{x_i}$) to Fig.\ \ref{fig:var}): %, for an acyclic path $P$: 
%(which takes the positive sides of variable gadgets $x_n,\tilde x_{n-1},\tilde x_1$):
\begin{alignat}{7}
(&\gamma{:}\{c_m,c_{m+1}\}, ~~&&c_{m+1}{:}\{c_m,\tilde y_{\hat i_m}^m\}, ~~&&\tilde y_{\hat i_m}^m{:}\{c_m,\tilde x_{\hat i_m}^m\}, ~~&&\tilde x_{\hat i_m}^m{:}\{c_m,d_m\},\label{eq:clausem}\tag{$P_{C_m}$}\\
&d_m{:}\{c_m,c_{m-1}\}, ~~&&c_m{:}\{c_{m-1},\tilde y_{\hat i_{m-1}}^{m-1}\}, ~~&&\tilde y_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},\tilde x_{\hat i_{m-1}}^{m-1}\}, ~~&&\tilde x_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},d_{m-1}\},\label{eq:clausemm1}\tag{$P_{C_{m-1}}$}\\
& ...,\nonumber\\
&d_2{:}\{c_2,c_2\}, ~~&&c_2{:}\{c_1,\tilde y_{\hat i_1}^1\}, ~~&&\tilde y_{\hat i_1}^1{:}\{c_1,\tilde x_{\hat i_1}^1\}, ~~&&\tilde x_{\hat i_1}^1{:}\{c_1,d_1\},\label{eq:clause1}\tag{$P_{C_1}$}\\
&d_1{:}\{c_1,b_{n+1}\}, ~~&&c_1{:}\{b_{n+1},a_{n+1}\},\label{eq:var2clause}\tag{$e_3,e_4$}\\
&b_{n+1}{:}\{a_{n+1},\tilde y_n^m\}, ~~&&a_{n+1}{:}\{\tilde y_n^m,\tilde x_n^m\}, ~~&&\tilde y_n^m{:}\{\tilde x_n^m,\tilde y_n^{m-1}\}, ~ \quad..., ~~&&\tilde x_{n}^2 {:}\{\tilde y_{n}^1,\tilde x_{n}^1\},\nonumber\\
&\quad\tilde y_n^1{:}\{\tilde x_n^1,b_n\}, ~~&&\tilde x_n^1{:}\{b_n,a_n\},\label{eq:varn}\tag{$P_{x_n}$}\\
&b_n{:}\{a_n,\tilde y_{n-1}^m\}, ~~&&a_n{:}\{\tilde y_{n-1}^{m},\tilde x_{n-1}^{m}\}, ~~&&\tilde y_{n-1}^m{:}\{\tilde x_{n-1}^m,\tilde y_{n-1}^{m-1}\},~~ ..., ~~&&\tilde x_{n-1}^2{:}\{\tilde y_{n-1}^1,\tilde x_{n-1}^1\},\nonumber\\
&\quad\tilde y_{n-1}^1{:}\{\tilde x_{n-1}^1,b_{n-1}\}, ~~&&\tilde x_{n-1}^1{:}\{b_{n-1},a_{n-1}\},\label{eq:varnm1}\tag{$P_{x_{n-1}}$}\\
&...,\nonumber\\
&b_{2}{:}\{a_{2},\tilde y_{1}^m\}, ~~&&a_{2}{:}\{\tilde y_{1}^m,\tilde x_{1}^m\}, ~~&&\tilde y_1^m{:}\{\tilde x_1^m,\tilde y_1^{m-1}\},~ \quad..., ~~&&\tilde x_1^2{:}\{\tilde y_1^1,\tilde x_1^1\},\nonumber\\
&\tilde y_1^1{:}\{\tilde x_1^1,b_1\}, ~~&&\tilde x_1^1{:}\{b_1,a_1\},\label{eq:var1}\tag{$P_{x_1}$}\\
&b_1{:}\{a_1,\beta\}, ~~&&a_1{:}\{\beta,\alpha\})\tag{$e_3,e_4$}
\end{alignat}


%\begin{alignat}{3}
%(&\gamma{:}\{c_m,c_{m+1}\}, ~~&&c_{m+1}{:}\{c_m,\tilde y_{\hat i_m}^m\}, ~~\tilde y_{\hat i_m}^m{:}\{c_m,\tilde x_{\hat i_m}^m\}, ~~\tilde x_{\hat i_m}^m{:}\{c_m,d_m\},\label{eq:clausem}\\
%&d_m{:}\{c_m,c_{m-1}\}, ~~&&c_m{:}\{c_{m-1},\tilde y_{\hat i_{m-1}}^{m-1}\}, ~~\tilde y_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},\tilde x_{\hat i_{m-1}}^{m-1}\}, ~~\tilde x_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},d_{m-1}\},\label{eq:clausemm1}\\
%& ...,\label{eq:clauses}\\
%&d_2{:}\{c_2,c_2\}, ~~c_2{:}\{c_1,\tilde y_{\hat i_1}^1\}, ~~\tilde y_{\hat i_1}^1{:}\{c_1,\tilde x_{\hat i_1}^1\}, ~~\tilde x_{\hat i_1}^1{:}\{c_1,d_1\},\label{eq:clause1}\\
%&d_1{:}\{c_1,b_{n+1}\}, ~~c_1{:}\{b_{n+1},a_{n+1}\},\label{eq:var2clause}\\
%&b_{n+1}{:}\{a_{n+1},\tilde y_n^m\}, ~~a_{n+1}{:}\{\tilde y_n^m,\tilde x_n^m\}, ~~\tilde y_n^m{:}\{\tilde x_n^m,\tilde y_n^{m-1}\}, ~~ ..., ~~\tilde x_{n}^2 {:}\{\tilde y_{n}^1,\tilde x_{n}^1\}, ~~\tilde y_n^1{:}\{\tilde x_n^1,b_n\}, ~~\tilde x_n^1{:}\{b_n,a_n\},\label{eq:varn}\\
%&b_n{:}\{a_n,\tilde y_{n-1}^m\}, ~~a_n{:}\{\tilde y_{n-1}^{m},\tilde x_{n-1}^{m}\}, ~~\tilde y_{n-1}^m{:}\{\tilde x_{n-1}^m,\tilde y_{n-1}^{m-1}\},~~ ..., ~~\tilde x_{n-1}^2{:}\{\tilde y_{n-1}^1,\tilde x_{n-1}^1\}, ~~\tilde y_{n-1}^1{:}\{\tilde x_{n-1}^1,b_{n-1}\},\\
%&\quad\tilde x_{n-1}^1{:}\{b_{n-1},a_{n-1}\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&b_{2}{:}\{a_{2},\tilde y_{1}^m\}, ~~a_{2}{:}\{\tilde y_{1}^m,\tilde x_{1}^m\}, ~~\tilde y_1^m{:}\{\tilde x_1^m,\tilde y_1^{m-1}\},~~ ..., ~~\tilde x_1^2{:}\{\tilde y_1^1,\tilde x_1^1\}, ~~\tilde y_1^1{:}\{\tilde x_1^1,b_1\}, ~~\tilde x_1^1{:}\{b_1,a_1\},\label{eq:var1}\\
%&b_1{:}\{a_1,\beta\}, ~~a_1{:}\{\beta,\alpha\})
%\end{alignat}



%\begin{align}
%\nonumber(&\gamma{:}\{c_{m+1},c_m\},~ c_{m+1}{:}\{y_m^{i_{w_m}},c_m\},~ y_m^{i_{w_m}}{:}\{x_m^{i_{w_m}},c_m\},~ x_m^{i_{w_m}}{:}\{d_m,c_m\},~ d_m{:}\{c_m,c_{m-1}\},~ c_m{:}\{y_{m-1}^{i_{w_{m-1}}},c_{m-1}\},\\
%& ...,\\
%&c_2{:}\{y_1^{i_{w_1}},c_1\},~ y_1^{i_{w_1}}{:}\{x_1^{i_{w_1}},c_1\},~x_1^{i_{w_1}}{:}\{d_1,c_1\},~ d_1{:}\{c_1,b_{n+1}\},~c_1{:}\{b_{n+1},a_{n+1}\},~b_{n+1}{:}\{a_{n+1},y_n^m\},\label{eq:clauses}\\
%&a_{n+1}{:}\{y_n^m,x_n^m\},~ y_n^m{:}\{x_n^m,y_n^{m-1}\},~ ...,~ x_{n}^2 {:}\{y_{n}^1,x_{n}^1\},~ y_n^1{:}\{x_n^1,b_n\},~x_n^1{:}\{b_n,a_n\},~b_n{:}\{a_n,y_{n-1}^m\},\label{eq:varn}\\
%\nonumber&a_n{:}\{y_{n-1}^{m},x_{n-1}^{m}\},~ y_{n-1}^m{:}\{x_{n-1}^m,y_{n-1}^{m-1}\},~ ...,~ x_{n-1}^2{:}\{y_{n-1}^1,x_{n-1}^1\},~ y_{n-1}^1{:}\{x_{n-1}^1,b_{n-1}\},~ x_{n-1}^1{:}\{b_{n-1},a_{n-1}\},\\ 
%&b_{n-1}{:}\{a_{n-1},y_{n-2}^m\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&a_2{:}\{y_1^m,x_1^m\},~ y_m^1{:}\{x_1^m,y_1^{m-1}\},~ ...,~ x_1^2{:}\{y_1^1,x_1^1\},~ y_1^1{:}\{x_1^1,b_1\},~ x_1^1{:}\{b_1,a_1\},~
%b_1{:}\{a_1,\beta\},\label{eq:var1}\\ 
%\nonumber&a_1{:}\{\beta,\alpha\})
%\end{align}

%Here (\ref{eq:clausem}) corresponds to the portion of $P$ passing through clause $C_m$'s gadget, (\ref{eq:clausemm1}) to the portion passing through $C_{m-1}$'s gadget, (\ref{eq:clauses}) to the portion passing through the gadgets for clauses $C_{m-2},...,C_2$, (\ref{eq:clause1}) through clause $C_1$, (\ref{eq:var2clause}) to the connection from clause $C_1$'s gadget back to variable $x_n$'s gadget (\ref{eq:varn}) through variable $x_n$, (\ref{eq:varnm1}) through $x_{n-1}$, (\ref{eq:othervars}) through variables $x_{n-2},...,x_2$, and (\ref{eq:var1}) through $x_1$'s gadget.

Observe that for each {\em label$:$edge} entry number $k$ after $\gamma{:}\{c_{m+1},c_m\}$ (i.e., the one for iteration $\ell$), the entry's label is one of the two A-nodes occurring in entry $k-1$'s (i.e., the next entry's) edge.

Therefore iteration $k$'s removal of the then-isolated A-node $o_k$ removes the (only) label from entry $o_k{:}\{p_k,p_k'\}$'s edge, disconnecting that component to two, in time for iteration $k-1$. Note also that one of edge $\{p_k,p_k'\}$'s two endpoints (say, $p_k$) the {\em label} of the succeeding entry $o_{k-1}{:}\{p_{k-1},p_{k-1}'\}$ (i.e., $p_k=o_{k-1}$) and does not appear as an {\em endpoint} in any subsequent edge in the ordering. That is, at the start of the iteration $k$, $p_k$ is a leaf in the Ahograph. Therefore the removal of edge $\{p_k,p_k'\}$ means that $p_k = o_{k-1}$ is an isolated A-node at the start of iteration $k-1$. The remainder of that component within the Ahograph is of course still a tree, thus proving the inductive claim.

Since the BUILD algorithm running on $R'$ never encounters a connected Ahograph, it follows \cite{bryant1995extension} that $R'$ is consistent.
%
%%Therefore each removal of the next {\em label$:$edge} entry causes the isolation of the A-node appearing as the subsequent entry's label.
%
%%The initial Ahograph consists of two components, one of which is an isolated A-node ($\gamma$). It has $\ell$ edges, corresponding to $P$'s $\ell$ arcs. Every A-node appears (once) as a label, except for $\alpha$ and $\beta$. Thus the Ahograph has $\ell+2$ A-nodes, and its second component is a tree. Therefore each deletion of an edge from that second component increases the number of components by one.
%
%Finally, observe that in each iteration, the edge deleted is incident to a leaf, thus rendering it an isolated A-node.
%
%
%\textbf{HERE}
%
%
%If $o_k$ nonetheless is still not isolated, that means that triple $p_kq_k | o_k$ was not removed in the previous iteration. 
%
%in each iteration a new A-node $u_k$ becomes isolated
%
%encountering a new isolated A-node in each iteration, 
%
%
%as the process implicitly constructs a caterpillar tree (see Fig.\ \ref{fig:caterpillar}), thus implying that $R'$ is consistent.
\end{proof}







\begin{lemma}[$\Leftarrow$]\label{lem:isentailed}
%Let $A' \subseteq A$. 
Suppose there exists an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then there exists a subset $A' \subseteq A$ for which $R' = \text{triples}(A')$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
\end{lemma}
\begin{proof}
%Given such a path $P$, we construct the corresponding $R'=f(P)$. By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths as follows:
%\begin{eqnarray*}
%P &=& (\alpha\beta,e_1,\beta a_1, e_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (a_{n+1}b_{n+1},e_3,b_{n+1}c_1,e_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (c_{m+1}\gamma)
%\end{eqnarray*}
%Given such an arc set $P$, we construct the corresponding $R'=f(P)$. 
We choose $A' = P$, and set $R' = \text{triples}(A')$, which is consistent by Lemma \ref{lem:consistR}.
%By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths:
%\begin{eqnarray*}
%P &=& (e_1,e_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (e_3,e_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (e_5)
%\end{eqnarray*}
%where $P_{x_i}$ is one of the two length-$2m{+}2$ subpaths passing through $x_i$'s gadget (from $a_ib_i$ to $a_{i+1}b_{i+1}$), $P_{C_j}$ is one of the three length-4 subpaths passing through $C_j$'s gadget (from $c_jd_j$ to $c_jc_{j+1}$) and including the succeeding connecting arc, and $e_1,...,e_5$ are placeholder names for the other five connecting arcs. 
%More precisely, the paths $P_{x_i}$ and $P_{C_j}$ are all ``half-open'' paths, meaning that they start with a node and end with an arc: $P_{x_i}$ starting with $a_ib_i$ and ending with one of the two arcs {\em preceding} $a_{i+1}b_{i+1}$, and $P_{C_j}$ starting with $c_jd_j$ and edging with the (unique) arc {\em preceding} $c_{j+1}d_{j+1}$.
%where $P_{x_i}$ is the path passing through $x_i$'s variable gadget, $P_{C_j}$ is the path passing through $C_j$'s clause gadget, and $e_1,...,e_4$ are placeholder names for the four corresponding connecting arcs. More precisely, the paths $P_{x_i}$ and $P_{C_j}$ are all ``half-open'' paths, meaning that they start with a node and end with an arc: $P_{x_i}$ starting with $a_ib_i$ and ending with one of the two arcs {\em preceding} $a_{i+1}b_{i+1}$, and $P_{C_j}$ starting with $c_jd_j$ and edging with the (unique) arc {\em preceding} $c_{j+1}d_{j+1}$.

%Recalling that each 1-2-hyperarc represents a rooted triple in $R$, we add to $R'$ the triple corresponding to each arc appearing in $P$, i.e., $R' = \{r(e) : e \in P\}$, where $r(e)$ denotes the triple represented by $e$.

Let $\ell=|P|$, and for each $k \in [\ell]$, let $e_k = u_k{\to}\{v_k,v_k'\}$ denote the $k$th arc in $P$, with $u_k = p_kq_k$ and $\{v_k,v_k'\} = \{p_ko_k, q_ko_k \}$ (for some leaves $p_k,q_k,o_k$), representing triple $p_k q_k | o_k = u_k | o_k$. The names $v_\ell,v_\ell'$ can be assigned so that $v_\ell = c_{m+1}\gamma$ (and $v_\ell'$ is $e_\ell$'s non-destination sink node $c_m \gamma$), but we can also simply represent $e_\ell$ as $u_\ell|o_\ell = c_mc_{m+1} | \gamma$.
%so hyperarc $e_\ell = u_\ell{\to}\{v_\ell, v_\ell'\}$, representing triple $u_\ell|o_\ell = p_\ellq_\ell | o_\ell = c_mc_{m+1} | \gamma$. 
Similarly, for each $k \in [2,...,\ell]$, we can assign the names $v_{k-1},v_{k-1}'$ so that $v_{k-1}=u_k$, i.e., $\text{t}(e_k) = u_k = v_{k-1} \in \text{h}(e_{k-1})$,
%and so hyperarc $e_{k-1} = u_{k-1}{\to}\{u_k, v_{k-1}'\}$, representing triple $p_{k-1}q_{k-1} | o_{k-1} = u_{k-1}|o_{k-1}$.
and we can also simply represent $e_{k-1}$ as $u_{k-1}|o_{k-1}$.

Now consider arcs $e_{\ell-1}$ and $e_\ell$, and observe that their representations as $u_{\ell-1}|o_{\ell-1}$ and $u_\ell|o_\ell$ (respectively) are 
%$e_{\ell-1} = u_{\ell-1}{\to}\{u_\ell, v_{\ell-1}'\}$ and $e_\ell = u_\ell{\to}\{v_\ell, v_\ell'\}$, representing triples $u_{\ell-1}|o_{\ell-1}$ and $u_\ell|o_\ell$, respectively, and observe that this pair of triples is 
of exactly the form that dyadic inference rule (\ref{eq:2b}) applies to: via that inference rule---{\em assuming $R'$ is consistent}---we can infer the triple $u_{\ell-1}|o_\ell$, which have the form $c_m \tilde y_i^m | \gamma$ (for some $i$). % or $c_j \bar y_i^m | \gamma$.

%, where the names $v_k,v_k'$ are assigned so that $v_k$ is $u_k$'s successor on $P$, i.e., $v_k = u_{k+1}$ (except when $k=\ell$, in which case $v_k=c_{m+1}\gamma$), and therefore, $u_k=v_{k-1}$, i.e., $u_k = \text{t}(e_k) \in \text{h}(e_{k-1}) = \{v_{k-1},v_{k-1}'\}$
%
%That is, $\text{t}(e_k) = p_kq_k$, and $o_{k-1} \in \{p_k, q_k\}$ and $|\{p_k, q_k\} \cap \{p_{k-1}, q_{k-1}\}|=1$, and so $e_k$ represents $p_k q_k | o_k$. Then observe that by applying the second dyadic inference rule (recall Def.\ \ref{def:2ord}) to the triples represented by the path's last two arcs (i.e., $p_{\ell-1} q_{\ell-1} | o_{\ell-1}$ and $p_\ell q_\ell | o_\ell$), we can infer $p_{\ell-1} q_{\ell-1} | o_\ell$. 

Similarly, by applying this inference rule to the triple represented $P$'s third-to-last arc (i.e., $u_{\ell-2} | o_{\ell-2}$) and the derived triple  $u_{\ell-1} | o_\ell$, we can infer $u_{\ell-2} | o_\ell$. Via a total of $\ell-1$ such applications of dyadic inference rule (\ref{eq:2b}) (each corresponding to one BUILD iteration), we can derive $u_1 | o_\ell = p_1 q_1 | o_\ell$ = $\alpha \beta | \gamma$.
%
%Second, by Lemma \ref{lem:consistR} proved below, $R'$ is indeed consistent.
\end{proof}





%mpj
%\newpage


%mpj
\begin{figure}%[t!]
\centering
	\begin{subfigure}{\textwidth}
\centering
%\input{triples-fig-var-leaves}
%\captionsetup{justification=centering}
%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%\input{triples-fig-tree}
\makebox[1\textwidth][c]{ %\hskip -2cm
\includegraphics[width=1.15\textwidth]{rt-fig-ahograph-arx.pdf}
}
%\vskip .05cm
%\vskip -.05cm
\caption{The initial Ahograph $[R',L(R')]$ constructed based on an underlying {\em acyclic} path $P$. Because $P$ is acyclic, the node  $\tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j$ pointed to by each $C_j$'s witness node $c_j \tilde x_{\hat i_j}^j$ is a {\em sink node in $H$}, and thus A-nodes $\tilde y_i^j$ and $\tilde x_i^j$ are {\em leaves in the Ahograph}. As a result, at each BUILD iteration, the Ahograph has two components, a tree and an isolated node.
%, distinct from the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets.% (as occurs in Fig.\ \ref{fig:ahocycle}).
%
%Because $P$ is acyclic, 
%, where $P$ is an acyclic path in the hypergraph from $\alpha\beta$ to $c_{m+1}\gamma$,
%%(specifically, the red path shown in Fig.\ \ref{fig:overview}), 
%and $R'=\text{triples}(P)$. 
%%Here $x_2$ is false and $x_1,x_3,x_4$ are true, and the witness literals for clauses $C_1,C_2,C_3,C_4$ are $\bar x_n, \bar x_1, \bar x_n, \bar x_1$, respectively. 
%%If $P$ had contained a cycle involving some clause $C_j$, then $C_j$'s $x$ and $p$ nodes in the resulting Ahograph would have 
%Let $\tilde x_i^j \tilde y_i^j$ be the variable gadget node pointed to by the $C_j$ clause's witness node. Then, because $P$ is acyclic, A-nodes $\tilde x_i^j$ and $\tilde y_i^j$ are both leaves {\em in the Ahograph}, rather than appearing in the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets (as occurs in Fig.\ \ref{fig:ahocycle}).
}
\label{fig:ahograph}
%\end{figure}
%\begin{figure}[t!]
\end{subfigure}
\vskip .5cm
\centering
	\begin{subfigure}{\textwidth}
\centering
%\captionsetup{justification=centering}
%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%\input{triples-fig-tree}
\includegraphics[width=.75\textwidth]{rt-fig-ahocycle-arx.pdf}
%\vskip .05cm
%\vskip -.05cm
\caption{A fragment of the Ahograph resulting from the cause of a cycle in $P$, viz., a back-arc in which some clause $C_j$'s witness node $c_j \bar x_i^j$ points to a {\em non-sink} node $\bar x_i^j \bar y_i^j$ that lies earlier in the path $P$ (specifically, within $x_i$'s gadget), and thus A-nodes $\tilde y_i^j$ and $\tilde x_i^j$ are {\em non-leaves} in the Ahograph. This yields the triangle $c_j-\bar y_i^j - \bar x_i^j$. After the BUILD iteration in which A-node $c_{j+1}$ and edge $c_j\bar y_i^j$ are removed, $\bar y_i^j$ will still {\em not} be isolated, and hence the Ahograph will at that point consist of a single component, indicating $R'$ is inconsistent.
%Ahograph $[R',L(R')]$, where $P$ is an acyclic path in the hypergraph from $\alpha\beta$ to $c_{m+1}\gamma$ (specifically, the red path shown in Fig.\ \ref{fig:overview}), and $R'=\text{triples}(\text{arcs}(P))$. Here $x_2$ is false and $x_1,x_3,x_4$ are true, and the witness literals are $\bar x_n, \bar x_1, \bar x_n, \bar x_1$ for clauses $C_1,C_2,C_3,C_4$, respectively. 
%%If $P$ had contained a cycle involving some clause $C_j$, then $C_j$'s $x$ and $p$ A-nodes in the resulting Ahograph would have  
%Because $P$ is acyclic, each clause $C_j$'s $x$ and $p$ A-nodes are leaves {\em in the Ahograph}, rather than being A-nodes in the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets. 
}
\label{fig:ahocycle}
\end{subfigure}
\caption{The Ahograph $[R',L(R')]$ is constructed when Aho et al.'s BUILD algorithm is executed on the triples $R' = \text{triples}(P)$ corresponding to the path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$. The existence of any cycle within $P$ involving some clause $C_j$'s witness node $c_j \tilde x_{\hat i_j}^j$ pointing to $\tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j$ (i.e., arc $c_j \tilde x_{\hat i_j}^j \to \{c_j \tilde y_{\hat i_j}^j, \tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j\}$) will be reflected in the locations in the Ahograph of A-nodes $\tilde y_{\hat i_j}^j$ and $\tilde x_{\hat i_j}^j$.}
\end{figure}







\begin{figure}[t!]
\centering
\makebox[1\textwidth][c]{ %\hskip -2cm
  \begin{subfigure}[t]{.35\linewidth}
    \centering
%    \captionsetup{width=.9\linewidth}%
    \includegraphics[height=.5\textheight]{rt-fig-pathtree-arx.pdf}
\caption{The (unique) caterpillar tree determined by the triples corresponding to $P$, which thence satisfies $\alpha\beta|\gamma$.
\label{fig:pathtree}
}
  \end{subfigure}
\hskip .35cm
  \begin{subfigure}[t]{.79\linewidth}
    \centering
    %\captionsetup{width=1.1\linewidth}%
    \includegraphics[height=.5\textheight]{rt-fig-nopathtree-arx.pdf}
\caption{A tree consistent with $A'$, i.e., displaying all of $R'=\text{triples}(A')$, but {\em not} displaying $\alpha \beta | \gamma$.
%The tree that can be constructed displaying all triples in $R'=\text{triples}(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. 
The root's left subtree contains all leaves appearing in A-nodes before the ``directed cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
\label{fig:nopathtree}
}
  \end{subfigure}
 }
%
%
%%\captionsetup{justification=centering}
%%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%%\input{triples-fig-tree}
%\includegraphics[height=.5\textheight]{triples-fig-pathtree.pdf}
%%\vskip .05cm
%\vskip -.1cm
%\caption{The caterpillar tree resulting from the triples corresponding to $P$, which thence satisfies $\alpha\beta|\gamma$.}
%\label{fig:caterpillar}
%\vskip .1cm
%\centering
%%\captionsetup{justification=centering}
%%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%%\input{triples-fig-tree}
%\includegraphics[height=.5\textheight]{triples-fig-nopathtree.pdf}
%%\vskip .05cm
%%\vskip -.05cm
\caption{Trees resulting from triples corresponding to an acyclic arc set $A' \subseteq A$ in $H$ that (a) does or (b) does not contain a path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%The tree that can be constructed displaying all triples in $R'=\text{triples}(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. The root's left subtree contains all leaves appearing in A-nodes before the ``directed cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
}
\end{figure}




























\subsection{Consistent Entailing Subset $\Rightarrow$ Acyclic Path}

We prove the contrapositive, via a proof that will depend on two subsequent lemmas proved below.

\begin{lemma}[$\Rightarrow$]\label{lem:notentailed}
%If $R'$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$, then $A' = \text{arcs}(R')$ contains the arcs of an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%
%Let $A' \subseteq A$. 
Suppose there is no acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then for every subset $A' \subseteq A$, $R' = \text{triples}(A')$ is {\em not} a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
%If $A' \subseteq A$ is {\em not} an acyclic arc set subsuming the set $P$ of arcs appearing in some path from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \text{triples}(A')$ is not a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
\end{lemma}
\begin{proof}
%Given such a subset $R'$, we construct the corresponding $P=f^{-1}(R')$.
Let $A' \subseteq A$ be an arbitrary subset of $A$, and set $R' = \text{triples}(A')$.

First, suppose there {\em is} a path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then $P$ must be cyclic, and thus $\text{triples}(P) \subseteq R'$ will be inconsistent. Intuitively, it can be seen that any (directed) cycle in $H$ corresponds to a vicious (inconsistent) cycle of rooted triples. In particular (see Fig.\ \ref{fig:ahocycle}), any clause $C_j$'s component whose witness node points to a variable gadget node already visited on the path (causing a simple cycle in $H$) will induce a triangle {\em in the Ahograph}, resulting in a single-component Ahograph in the corresponding iteration of the BUILD algorithm (if no single-component Ahograph is encountered in an earlier iteration).

Second, suppose there is no path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ having $P \subseteq A$, cyclic or otherwise. If $A'$ is cyclic then $R' = \text{triples}(A')$ will again be inconsistent, so assume $A'$ is acyclic. Now we will show constructively that in this case, $R'$ does not entail $\alpha\beta|\gamma$.

Let $S(\alpha \beta,V,R') \subseteq V$ (written $V_{\alpha\beta}$) be the set of all nodes reachable from $\alpha \beta$ via the nodes $V$ and the arcs $A'$ and let $P(c_{m+1}\gamma,V,R') \subseteq V$ (written $V_{c_{m+1}\gamma}$) be the set of all nodes that $c_{m+1}\gamma$ is reachable {\em from} via $V$ and $A'$, and set $V' = V_{\alpha\beta} \cup .V_{c_{m+1}\gamma}$ Then by assumption $V_{\alpha\beta}$ and $V_{c_{m+1}\gamma}$ are disjoint. That is, the hypergraph $(V',A')$ has two components.

Let $V_{\alpha \beta}^* \subseteq V_{\alpha\beta}$ be the maximal elements of $V_{\alpha\beta} $ in the sense that every $u \in V_{\alpha \beta}^*$ is reachable from $\alpha\beta$ but no other node $v \in V_{\alpha\beta}$'s reachability {\em depends on} $u$. That is, $S(\alpha \beta,V-\{u\},R') = S(\alpha \beta,V,R') - \{u\}$. Similarly, let $V_{c_{m+1}\gamma}^* \subseteq V_{c_{m+1}\gamma}$ be the minimal elements of $V_{c_{m+1}\gamma}$ in the sense that for any $v \in V_{c_{m+1}\gamma}^*$, there is no other node $u \in V_{c_{m+1}\gamma}$ dependent on $v$, i.e., $P(c_{m+1}\gamma,V-\{v\},R') = P(c_{m+1}\gamma,V,R')-\{v\}$.

By Lemma \ref{lem:uvpairs} proved below, we can assume wlog that there are at most 3 $u^*$s and at most 3 $v^*$s, which together yield either 1, 2, or 3 pairs $(u_h,v_h)$, with each pair connected by an arc $e_h \in  A - A'$.

Then by Lemma \ref{lem:treeexs} proved below, we can build a tree displaying $\text{triples}(A') \cup \{\alpha\gamma | \beta\}$ (see Fig.\ \ref{fig:nopathtree}). This shows that $R' \cup \{\alpha\gamma | \beta\}$ is consistent, and thus that $R'$ does not entail $\alpha\beta | \gamma$.
%
%
%
%
%
%
%%\textbf{but then there's a tree satisfying $R'$ and not $\alpha\beta|\gamma$}
%
%
%First observe that the only triple in $R$ including $\alpha$ or $\beta$ is $\alpha\beta | a_1$, and so any hypothetical subset $R' \subset R$ pseud o-entailing $\alpha\beta|\gamma$ must necessarily include $\alpha\beta | a_1$.  But then observe that the only other triple in $R$ including $\alpha$ or $\beta$ is $\beta a_1 | b_1$, so it must be included. Next, observe that the only other triples in $R$ including $\beta$ or $a_1$ are $a_1b_1 | x_i^1$ and $a_1b_1 | \bar x_i^1$, so at least one of them must be included. We claim that by repeated application of arguments of this kind, we obtain that the arcs corresponding to the triples of any such $R'$ must trace out a path from $\alpha\beta$ to $c_{m+1}\gamma$.
%
%Second, observe that if $P$ contained a cycle, then the triples corresponding to the hyperarcs appearing in that cycle would themselves be inconsistent, contradicting the consistency of $R'$.
\end{proof}






\begin{lemma}\label{lem:uvpairs}
Let $A'$ be acyclic, suppose there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. and let $V_{\alpha \beta}^* \subseteq V_{\alpha\beta}$ and $V_{c_{m+1}\gamma}^* \subseteq V_{c_{m+1}\gamma}$ be defined as in the proof of Lemma \ref{lem:notentailed} above. Then $|V_{\alpha \beta}^*| = |V_{c_{m+1}\gamma}^*| \in [3]$, 
%and there is bijection between $V_{\alpha \beta}^*$ and $V_{c_{m+1}\gamma}^*$, with each pair corresponding to a unique edge in $A-A'$.
%By Lemma \ref{lem:uvpairs} proved below, we can assume wlog that there are at most 3 $u^*$s and at most 3 $v^*$s, 
which together yield $w \in [3]$ pairs $\{(u_h,v_h) : h \in [w]\}$, with each pair connected by an arc $e_h \in  A - A'$.
\end{lemma}
\begin{proof}
First, we claim we can assume wlog that for no $u \in V_{\alpha\beta}$ will the path to it from $\alpha\beta$ cross a back-arc, i.e., a subpath taking an arc of the form $c_j \tilde x_i^j{\to}\{c_j\tilde y_i^j, \tilde x_i^j\tilde y_i^j\}$ to $\tilde x_i^j\tilde y_i^j$ (see Fig.\ \ref{fig:clause}). Preceding $c_j \tilde x_i^j$, the path would have had to visit $c_jd_j$, and if after crossing the back-arc the path is going to eventually reach $c_{m+1}\gamma$, then it would have to visit $c_jd_j$ again, making it cyclic and $R'$ inconsistent.

Second, we claim we can assume wlog that no $v^*$'s path to $c_{m+1}\gamma$ will contain back-arcs.
%, i.e., a subpath taking an arc of the form $c_j \tilde x_i^j{\to}\{c_j\tilde y_i^j, \tilde x_i^j\tilde y_i^j\}$ to $\tilde x_i^j\tilde y_i^j$. 
To see this, consider what node $v^*$ could possibly benefit (in terms of reaching $c_{m+1}\gamma$) from such a path. If $v^*=c_jd_j$ (or any predecessor it it), then the path from $v^*$ to $c_{m+1}\gamma$ would again have to eventually return to $c_jd_j$ again, making the path cyclic. If $v^*= c_jx_i^j$, then it is not impossible per se for there to be an acyclic path from it to $c_{m+1}\gamma$ traversing the specified subpath. The only possible arc that could be used for reaching $c_jx_i^j$, however, is the one from $c_jd_j$, in which case once again the resulting path from $\alpha\beta$ to $c_{m+1}\gamma$ would be cyclic.

Now, how far are the maximal elements $V_{\alpha\beta}$ away from the minimal elements $V_{c_{m+1}\gamma}^*$? That is, how many arcs from $A$ would have to be added to $A'$ in order to reach a node $v^* \in  V_{c_{m+1}\gamma}^*$ from a node $u^* \in V_{\alpha \beta}^*$?

Since our goal is to show that $R'$ does {\em not} entail $\alpha \beta | \gamma$, we assume wlog the most difficult case, i.e., that any $v^* \in V_{c_{m+1}\gamma}^*$ is only one hop away from some $u \in V_{\alpha \beta}$, via some arc $e \in A - A'$, the addition of which to $A'$ would complete a path from $\alpha\beta$ to $c_{m+1}\gamma$. Conversely, we can assume wlog that for every $u^* \in V_{\alpha \beta}^*$ there exists an edge $e \in A-A'$ that would connect it to some $v \in V_{c_{m+1}\gamma}$. If $A_\times$ is the set of all arcs $e$ playing this role for some $u^*$ and/or $v^*$, then observe that $(V_{\alpha \beta}^*,V_{c_{m+1}\gamma}^*)$ is a {\em directed cut} separating $\alpha\beta$ from $c_{m+1}\gamma$ in the hypergraph $(V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^*, A' \cup A_\times)$, and $A_\times$ consists of the forward cross-arcs of that cut.

Now, how many arcs could there be in $A_\times$? By inspection of the hypergraph construction, it can be seen that $|A_\times|$ will be either 2, 3, or 1, depending (respectively) on whether the cut occurs within a variable gadget, within a clause gadget, or elsewhere. 
%Note also that due to hypergraph construction there will be a bijection between $u^*$s and $v^*$s. To see this, recall that the only arcs in which both heads are non-sink nodes are those in which a clause gadget's witness node $c_j \tilde x_i^j$ points back to a variable gadget node $\tilde x_i^j \tilde y_i^j$. But we have seen that no $u^*$'s path will contain a back-arc. Therefore if $A_\times$ contains an edge of the form $c_j \tilde x_i^j{\to}\{c_j \tilde y_i^j, \tilde x_i^j \tilde y_i^j\}$, it must be due to $u^*=c_j \tilde x_i^j$ and $v^*=c_j \tilde y_i^j$.
\end{proof}















\begin{lemma}\label{lem:treeexs}
Let $A'$ be acyclic, suppose there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$, and let $V_{\alpha \beta}^* \subseteq V_{\alpha\beta}$ and $V_{c_{m+1}\gamma}^* \subseteq V_{c_{m+1}\gamma}$ be defined as in the proof of Lemma \ref{lem:notentailed} above, and let $|V_{\alpha \beta}^*| = |V_{c_{m+1}\gamma}^*| \in [3]$, 
%where is bijection between $V_{\alpha \beta}^*$ and $V_{c_{m+1}\gamma}^*$, with each pair corresponding to a unique edge in $A-A'$.
which together yield $w \in [3]$ pairs $\{(u_h,v_h) : h \in [w]\}$, with each pair connected by an arc $e_h \in  A - A'$.
Then there exists a tree displaying $R' \cup \{\alpha\gamma | \beta\}$.
\end{lemma}
\begin{proof}
%Now we will show that for such an $A''$, $R' = \text{triples}(A'')$ is compatible with $\alpha\beta | \gamma$ not holding.
%
%Let $w \in [3]$ be the number of pairs $(u_h^*,v_h^*)$. 
There must be some latest common predecessor node $u_0$ of $\{u_h : h \in [w]\}$ and some earliest common successor node $v_4$ of $\{v_h : h \in [w]\}$. Let the (possibly empty) sequence of intermediate nodes on the path from $p$ to $u_h$ be $U_h = (u_h^1,...,u_h^{\ell_h})$, and the (possibly empty) sequence of intermediate nodes on the path from $v_h$ to $v_4$ be $V_h = (v_h^{1},...,v_h^{\ell_h'})$ Observe that each node $u_w^h$'s outgoing arc introduces one more leaf appearing in the triple's LHS, and so $U_h$ corresponds to $\ell_h$ such leaves, say, $p_h^1,...,p_h^{\ell_h}$. Each node $v_h^h$'s outgoing arc similarly introduces one more leaf in the triple's LHS, except for $v_1^1$, which introduces {\em two} more, because the leaf it shares in common with $u_w$ is also appearing on the LHS of a triple for the first time, due to $u_w$'s missing outgoing cross-arc, for a total of $\ell_h'+1$ such leaves, say, $q_h^0,...,q_h^{\ell_h'}$. Let $p_0$ be the leaf introduced by node $u_0$ and $q_4$ the leaf introduced by node $v_4$.

Then observe that $\{p\} \cup \bigcup_{f \in [w]} U_h$ can be put in a linear order, and hence $S(\alpha\beta,V,R')$ can as well. Let $L_S$ be the set of all leaves appearing in tail nodes of paths between $\alpha\beta$ and members of $V_{\alpha\beta}$, i.e., the leaves appearing in nodes $V_{\alpha\beta} - \{U_h^{\ell_h} : h \in [w]\}$. Then can we construct a caterpillar tree $C_S$ having leaves $L_S$ (see root's left subtree in Fig.\ \ref{fig:nopathtree}, except ignoring the appearance of $\gamma$ for a moment).

Similarly, observe that $\{s\} \cup \bigcup_{h \in [w]} V_h$ and hence $V_{c_{m+1}\gamma}$ can also be linearly ordered, and so if we define $L_P$ as the set of all leaves appearing in tail nodes of paths between members of $V_{c_{m+1}\gamma}$ and $c_{m+1}\gamma$,  i.e., the leaves appearing in nodes $V_{c_{m+1}\gamma} - \{c_{m+1}\gamma\}$, then we can also construct a caterpillar tree $C_P$ with leaves $L_P$ (see right subtree in Fig.\ \ref{fig:nopathtree}).

Now create a root node, whose children are the roots of $C_P$ and $S_P$. This resulting tree contains every leaf but $\gamma$, and observe that it displays every triple of $R'$ except (obviously) $c_m c_{m+1} | \gamma$.

Finally, we subdivide the tree's edge to $\alpha$ and add $\gamma$ as the second child of the tree's new inner node, with the result that the tree now displays $c_j c_{j+1} | \gamma$ and the rest of the triples of $R'$, as desired, yet also displays $\alpha \gamma | \beta$.
\end{proof}



%\textbf{start quotes:}
%
%%{\em Q: how do we know that a subset entailing $\alpha\beta|\gamma$ must necessarily correspond to a path?}
%
%\begin{lemma}[Bryant and Steel,  Prop. 9(1)]\label{lem:noabctrip} If $R$ is a closed set of rooted triples containing no triple with
%the leaves $\{a,b,c\}$ then $R \cup \{ab|e\}$, $R \cup \{ae|b\}$ and $R \cup \{be|a\}$ are all compatible.
%\end{lemma}
%
%{\em Q: can we get that entailment must follow a path by repeated (inductive) application of Lemma \ref{lem:noabctrip}?}
%
%\textbf{\em Q: is the consistency and/or the closure of a path in this construction actually somehow just obvious based on the construction?}
%\textbf{end quotes}





%\begin{lemma}[$\Leftarrow$]
%If there is a consistent triple set $R'$ entailing $\alpha\beta|\gamma$, then there is an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%%
%%Or: If there is no acyclic path from $ab$ to $ac$, then there is no consistent subset entailing $\alpha\beta|\gamma$.
%\end{lemma}
%\begin{proof}
%%First observe that the only triple in $R$ including $\alpha$ is $\alpha\beta | a_1$, and so any hypothetical subset $R' \subset R$ entailing $\alpha\beta|\gamma$ must necessarily include $\alpha\beta | a_1$.  But then observe that the only other triple in $R$ including $\beta$ is $\beta a_1 | b_1$. By repeated application of similar arguments, we obtain that the hyperarcs corresponding to the triples of any such $R'$ must trace out a path from $\alpha\beta$ to $c_{m+1}\gamma$.
%
%Second, observe that if the path contained a cycle, then the triples corresponding to the hyperarcs appearing in that cycle would themselves be inconsistent, contradicting the consistency of $R'$.
%%the portion of the Ahograph induced by everything from the start of the caterpillar up to the cycle's back-arc would be a single component.
%%
%%That is, if we pluck off the sink nodes one by one, then plucking off the node just following the back-arc will reduce the number of components from 2 to 1, indicating that $R$ is inconsistent.
%%
%%Does it suffice to argue that for any path from $ab$ to $ac$, if the path is acyclic then it implies a consistent subset entailing $\alpha\beta|\gamma$?
%%
%%\textbf{That is, can we assume that entailment will imply a path?}
%\end{proof}




%\begin{lemma}[$\Rightarrow$]
%If there is an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$, then there is a satisfying truth assignment.
%\end{lemma}
%\begin{proof}
%We read off the truth assignment from the choices the path makes passing through the series of variable gadgets. Because the path is acyclic, we know that in the case of each clause gadget it passes through, the node within the variable gadget pointed to is on the side of the variable gadget that the path did {\em not} use. Since we set the variable's truth value based on which side we did not use, this implies that the corresponding literal in the clause gadget is true, thus satisfying the clause.
%\end{proof}

Combining the Lemmas \ref{lem:isentailed} and \ref{lem:notentailed} with Theorem \ref{thm:apdh}, we conclude:

\begin{theorem}
\entailprob\:is NP-Complete.
\end{theorem}

And because computing the closure reduces to deciding whether $R \vdash t$ for $O(|L|^3)$ triples $t$, we also have:

\begin{corollary}
\closureprob\:is NP-hard.
\end{corollary}


%Also:
%
%\begin{corollary}
%The complementary problem, of deciding whether a triple is entailed by {\em every} consistent subset of $R$ is co-NP-Complete.
%\end{corollary}
%\begin{proof}
%Solve the original problem for both negations of the triple.
%\end{proof}


==> rt-proof-wabi.tex <==
% !TEX root = rootedtriples-wabi.tex

\section{The Proof}

\ifproofapp
\else
Clearly \entailprob\ is in NP: if we guess the subset $R' \subset R$, then we can verify both that $R'$ is consistent and that $R' \vdash t$ by executing Aho et al.\ \cite{aho1981inferring}'s polynomial-time BUILD algorithm on $R'$ \cite{bryant1995extension}. \minapdh\:is as well: guess the path, and check that it is acyclic.

Now we prove hardness, arguing that $R$ contains a consistent subset entailing $\alpha\beta|\gamma$ iff $H$ contains an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ iff $F$ admits a satisfying assignment $\mathbf{v}(\cdot)$, in two steps.
\fi

\ifrefapp
Due to lack of space, the proofs are deferred to the appendix.
\fi

%\textbf{3SAT} reduces to \apdh\:(which is therefore NP-Complete):


\subsection{Acyclic Path $\Leftrightarrow$ Satisfying Truth Assignment}

First we argue that acyclic paths correspond to satisfying truth assignments.

\ifproofapp
\noindent \textbf{Lemma \ref{lem:pathiffassign}.}
There is an an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ iff $F$ admits a satisfying truth assignment $\mathbf{v}(\cdot)$.
%If there is a satisfying truth assignment, then there is an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$.
\begin{proof}
($\Leftarrow$)
We construct $P$ based on the satisfying truth assignment $\mathbf{v}(\cdot)$. For each $x_i$, if $\mathbf{v}(x_i) =$ true, then we have $P$ take the $x_i$ gadget's {\em negative} side (drawn lower in Fig.\ \ref{fig:var}); otherwise, we have $P$ take its {\em positive} side (drawn higher). Then within each $C_j$, among the three possible witness paths, we choose one corresponding to the appearance of a literal that is true under $\mathbf{v}(\cdot)$ (which by assumption must exist).
%, which therefore points only to sides of variable gadgets that $P$ did {\em not} take. 
For the remainder of $P$ we have it take the required connecting arcs.

Notice that any potential cycle contained within $P$ must necessarily involve an arc $a$ whose tail lies within some clause $C_j$'s gadget and one of whose heads lies within some variable $x_i$'s gadget. But the witness path taken within $C_j$'s gadget corresponds to an appearance $\tilde x_i^j$ of a true literal $\tilde x_i$. If it a positive literal, i.e., $\tilde x_i=x_i$, then $\mathbf{v}(x_i) =$ true, and we would have had $P$ take the $x_i$ gadget's {\em negative} side---not the side $a$ is pointing to. Similarly, if $\tilde x_i=\bar x_i$, then $\mathbf{v}(x_i) =$ false, $P$ would have taken the $x_i$ gadget's {\em positive} side, which again is then not the side $a$ is pointing to. Thus $P$ must be acyclic.

($\Rightarrow$)
We read off $\mathbf{v}(\cdot)$ from the choices the path $P$ makes when passing through the series of variable gadgets, i.e., setting $\mathbf{v}(x_i) = $ true if $P$ used the $x_i$ gadget's {\em negative} side, and setting it to false otherwise. Now, consider a clause $C_j$'s gadget, whose witness node points to a node $v'$ within some variable $x_i$'s gadget. Because $P$ is acyclic, we know that $v'$ is on the side of $x_i$'s gadget that $P$ did {\em not} use. Since we chose the truth value $\mathbf{v}(x_i)$ that makes literals within nodes on the $x_i$ gadget's {\em unused} side true, this implies that literal corresponding to $C_j$'s witness node is true, thus satisfying the clause.
\end{proof}
Thus we have proven:

\vskip .2cm
\noindent\textbf{Theorem \ref{thm:apdh}.}
\apdh\:is NP-Complete.
\vskip .2cm
\else
\begin{lemma}\label{lem:pathiffassign}
There is an an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ iff $F$ admits a satisfying truth assignment $\mathbf{v}(\cdot)$.
%If there is a satisfying truth assignment, then there is an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$.
\end{lemma}
Thus we have proven:

\begin{theorem}\label{thm:apdh}
\apdh\:is NP-Complete.
\end{theorem}
\fi


Since an infeasible solution is defined to have infinite cost, an algorithm with {\em any} approximation factor would allow us to distinguish between positive and negative problem instances, which immediately implies:

\ifproofapp
\vskip .2cm
\noindent \textbf{Corollary \ref{cor:hardanyfactor}.} Approximating \minapdh\:to within {\em any} factor is NP-hard.
\vskip .2cm
\else
\begin{corollary}\label{cor:hardanyfactor}
Approximating \minapdh\:to within {\em any} factor is NP-hard.
\end{corollary}
\fi

Even if we restrict ourselves to problem instances admitting feasible solutions, this ``promise problem" \cite{goldreich2006promise} special case is hard to approximate within any reasonable factor.

%More formally, we obtain the following hardness of approximation.

\ifproofapp
\vskip .2cm
\noindent\textbf{Corollary \ref{cor:pathhardapx}.}
%In the promise problem \cite{goldreich2006promise} special case in which an acyclic B-hyperpath is assumed to exist, approximating \minapdh\:to within factor $|V|^{1-\epsilon}$ for any $\epsilon>0$ is NP-hard.
\minapdhprom\:is NP-hard to approximate to within factor $|V|^{1-\epsilon}$ for all $\epsilon>0$.
\begin{proof}
Let $\epsilon \in (0,1/4)$. Let $I = \langle H,u,v \rangle$ be an instance \minapdhprom. For this proof only, let $n=|V(H)|$.
We extend $H$ to a new hypergraph $H'$ by adding polynomially many dummy arcs forming an acyclic $u{\to}v$ path of length $n^{\lceil1+1/\epsilon\rceil}$, yielding a hypergraph $H'$ with $n' = n+n^{\lceil1+1/\epsilon\rceil}-1$ nodes and a new problem instance $I' = \langle H',u,v \rangle$, which is also by construction a valid problem instance of \minapdhprom. If $H$ has a path ($I$ is a positive instance), then $H'$ (like $H$) has one of some length $OPT^+ \le n-1$; if not ($I$ is a negative instance), then $H'$'s only path has length $OPT^- = n^{\lceil1+1/\epsilon\rceil}$.

Now, suppose there were a $|V|^{1-\epsilon}$-approximation algorithm.

Running it on the $I'$ resulting from a negative $I$ will yield a path of length at least $LB^- = OPT^- = n \cdot n^{\lceil1/\epsilon\rceil}$.

Running it on the $I'$ resulting from a positive $I$ will yield a path of length of at most
\begin{align*}
UB^+ &= n'^{1-\epsilon}\cdot (n-1)\\
&= (n+n^{\lceil1+1/\epsilon\rceil}-1)^{1-\epsilon}\cdot (n-1)\\
& < (n-1) \cdot n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)} + (n-1)^{2-\epsilon}\\
&< n \cdot n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)},
\end{align*}
where the last inequality follows from the fact that $(n-1)^{2-\epsilon} < n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)}$ for $\epsilon<1/4$.

Because $\lceil1+1/\epsilon\rceil\cdot(1-\epsilon) = 1+\lceil1/\epsilon\rceil - \epsilon - \epsilon \lceil 1/\epsilon \rceil < \lceil 1/\epsilon \rceil$, it follows that $UB^+ < LB^-$.

%$\lceil1/\epsilon\rceil$ vs $\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)$
%
%$\lceil1/\epsilon\rceil$ vs $\lceil1/\epsilon\rceil\cdot(1-\epsilon) + (1-\epsilon)$
%
%$\lceil1/\epsilon\rceil$ vs $\lceil1/\epsilon\rceil - \lceil1/\epsilon\rceil\cdot\epsilon + (1-\epsilon)$
%
%0 vs $- \lceil1/\epsilon\rceil\cdot\epsilon + (1-\epsilon)$
%
%$\lceil1/\epsilon\rceil\cdot\epsilon > (1-\epsilon)$

Thus by comparing the length $ALG$ of the path in $H'$ found by the hypothetical algorithm to $UB^+$ and $LB^-$, we can decide whether $I$ was positive or negative.
%
%Then any algorithm providing an $f(|V|)$-approximation would allow us to distinguish (for $|V|$ sufficiently large) between instances $H'$ with optimal solution cost $<f(|V|)\cdot|V|$ and those with optimal solution cost $\ge f(|V|) \cdot |V|^2$, thus deciding whether $H$ had a path.
\end{proof}
\else
\begin{corollary}\label{cor:pathhardapx}
%In the promise problem \cite{goldreich2006promise} special case in which an acyclic B-hyperpath is assumed to exist, approximating \minapdh\:to within factor $|V|^{1-\epsilon}$ for any $\epsilon>0$ is NP-hard.
\minapdhprom\:is NP-hard to approximate to within factor $|V|^{1-\epsilon}$ for all $\epsilon>0$.
\end{corollary}
\fi




Second, to extend the reduction to \entailprob, we argue that $H$ is a faithful representation of $R$ in the sense that acyclic paths from $\alpha\beta$ to $c_{m+1}\gamma$ (or acyclic supersets of such paths) correspond to consistent subsets entailing $\alpha\beta|\gamma$, and vice versa.


\subsection{Consistent Entailing Subset $\Leftarrow$ Acyclic Path}

We prove this direction via two lemmas, proving that the set of triples corresponding to an acyclic path are consistent and entail $\alpha\beta|\gamma$, respectively.



\ifproofapp
\vskip .2cm
\noindent\textbf{Lemma \ref{lem:consistR}.}
If there is an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(P)$ is consistent.
\begin{proof}
To prove $R'$ consistent, we 
%reinterpret the procedure we carried out in the proof of Lemma \ref{lem:isentailed} as implicitly executing 
step through the execution of Aho et al.\ \cite{aho1981inferring}'s BUILD algorithm running on input $R'$, tracking the state of the resulting Ahograph (see Fig.\ \ref{fig:ahograph}) and the tree being constructed (see Fig.\ \ref{fig:pathtree}) as they progress over time.
%Specifically, each application of dyadic inference rule (\ref{eq:2b}), as we step through $P$ in reverse order, can be interpreted as one iteration (or recursive call) of BUILD.
Each iteration can be interpreted as one application of dyadic inference rule (\ref{eq:2b}), as we step through $P$ in reverse order.

%, of stepping through $P$ in reverse, repeatedly applying dyadic inference rule (\ref{eq:2b})
%
%again step through $P$ in reverse, implicitly executing Aho et al.\ \cite{aho1981inferring}'s BUILD algorithm on input $R'$, picturing the state of the resulting Ahograph (see Fig.\ \ref{fig:ahograph}) and the tree being constructed (see Fig.\ \ref{fig:pathtree}) along the way. 

Observe that in Ahograph $[R', L(R')]$ (see Fig.\ \ref{fig:ahograph}), $\gamma$ will be an isolated A-node, since $R$ contains no triples with $\gamma$ on their LHSs,
%Just as dyadic inference rule (\ref{eq:2b}) carried us through to $\alpha\beta | \sigma$, 
%Observe also that by definition of $R'$, the A-nodes $L(R') - \{\gamma\}$ are connected in one component of Ahograph $[R', L(R')]$, 
and that the A-edge $\{c_m, c_{m+1}\}$ in $[R', L(R')]$ due to $P$'s last arc (representing $c_m c_{m+1} | \gamma$) is labeled (only) with $\gamma$. Isolated A-node $\gamma$ is removed for BUILD's second iteration, in which we recurse on the remaining A-nodes. The A-edge $\{c_m, c_{m+1}\}$ will therefore no longer appear in that iteration's Ahograph, $[R', L(R') - \{\gamma\}]$, rendering $c_{m+1}$ an isolated A-node.

We claim that this pattern will continue to obtain the rest of the way back to the start of $P$, with a new A-node becoming isolated  by the start of each iteration, causing an A-edge to be removed, and hence isolating another A-node for the succeeding iteration.
%
More precisely, number the iterations in reverse, counting downward from $\ell=|P|$, where iteration $\ell$ is the first iteration executed (the one in which A-node $o_\ell=\gamma$ is observed isolated and removed for the second iteration, thus also deleting the A-edge $\{p_\ell,q_\ell\}=\{c_m,c_{m+1}\}$).



Let $H_P$ be the subhypergraph of $H$ induced by the nodes $\{\text{t}(e) \cup \text{h}(e) : {e \in P}\}$, and recall that nodes in $H$ correspond to unordered pairs of A-nodes, and thus to potential A-edges in the Ahograph.

Because $P$ is a path (and because there are no arcs between two witness paths or between the two sides of a variable gadget), each non-sink node in $H_P$ will have out-degree 1 ($c_{m+1}\gamma$ has out-degree 0). Therefore $[R', L(R')]$ will have exactly $\ell$ A-edges, each with one label.
%
%%of $H$ induced by $P$ has out-degree at most one. Therefore no A-edge in the Ahograph has more than one label. Note that $\alpha$ and $\beta$ will not be labels of any A-edge.
%
Because $P$ is acyclic, each node in $H_P$ except $\alpha\beta$ (which has in-degree 0) will have in-degree 1. Therefore no label will appear on multiple A-edges in $[R', L(R')]$.
%
Thus there is a bijection between Ahograph $[R', L(R')]$'s $\ell$ A-edges and the labels appearing on them.

Node $\alpha\beta$ contains two leaves, and each arc in $P$ introduces one additional leaf, for a total of $\ell+2$ leaves in $L(R')$, and hence $\ell+2$ A-nodes in the Ahograph.

Note also that the first arc in $P$ adds label $b_1$ to A-edge $\{\alpha,\beta\}$ in the Ahograph, and that each subsequent arc adds a label to an A-edge incident to the preceding A-edge, and so all $\ell$ of the Ahograph's A-edges lie within a single component. Since isolated A-node $\gamma$ is one of the $\ell+2$ A-nodes, this means that the other component has exactly $\ell+1$ A-nodes, and is therefore a tree.

%To see this, suppose $c_j \tilde x_i^j{\to}\{\tilde x_i^j \tilde y_i^j, c_j \tilde y_i^j\}$ is a back-arc in $P$.
%
%there are no other A-edges in the Ahograph beyond those listed here.
%%
%Note also that no label appears on more than one A-edge. Therefore there is a one-to-one correspondence between the Ahograph's $\ell$ A-edge labels and $P$'s arcs. Every A-node appears (once) as a label, except for $\alpha$ and $\beta$. Thus the Ahograph has $\ell+2$ A-nodes, and its second component is a tree.

Now, we prove by induction that at the start of each iteration $k$ from $\ell$ down to $1$, the Ahograph consists of two components: some isolated A-node $o_k$ and a tree. We have already verified the base case: $o_\ell$ is isolated at the start, in iteration $\ell$, and the $\ell+1$ remaining nodes form a tree. Assume the claim is true for each iteration from $\ell$ down through some iteration $k$.

%If this is not true for every iteration, let $k$ be the first iteration at the start of which $o_k$ is not isolated. Now, we know that at the start the previous iteration (iteration $k+1$), $o_{k+1}$ (which is the right-hand side of triple $u_{k+1}|o_{k+1}$, where $o_k \in u_{k+1}$) was found to be isolated, and therefore was removed from the iteration-$k$ Ahograph. What does it mean if we find at the start of iteration $k$ that $o_k$ is still not isolated?
%
%The deletion of $o_{k+1}$ meant the removal of label $o_{k+1}$ from from the Ahograph of A-edge $u_{k+1}$, which contains $o_k$. If A-edge $u_{k+1}$ nonetheless remains in the Ahograph, this means that it still has some label.


%\begin{align}
%\nonumber(&\gamma{:}\{c_{m+1},c_m\},\\
%&c_{m+1}{:}\{\tilde y_{i_{w_m}}^m,c_m\},~\tilde y_{i_{w_m}}^m{:}\{\tilde x_{i_{w_m}}^m,c_m\},~\tilde x_{i_{w_m}}^m{:}\{d_m,c_m\},~ d_m{:}\{c_m,c_{m-1}\},~ c_m{:}\{\tilde y_{i_{w_{m-1}}}^{m-1},c_{m-1}\},\\
%& ...,\\
%&c_2{:}\{\tilde y_{i_{w_1}}^1,c_1\},~\tilde y_{i_{w_1}}^1{:}\{\tilde x_{i_{w_1}}^1,c_1\},~\tilde x_{i_{w_1}}^1{:}\{d_1,c_1\},~ d_1{:}\{c_1,b'_{n+1}\},~c_1{:}\{b'_{n+1},b_{n+1}\},~b'_{n+1}{:}\{b_{n+1},\tilde y_n^m\},\label{eq:clauses}\\
%&b_{n+1}{:}\{\tilde y_n^m,\tilde x_n^m\},~\tilde y_n^m{:}\{\tilde x_n^m,\tilde y_n^{m-1}\},~ ...,~\tilde x_{n}^2 {:}\{\tilde y_{n}^1,\tilde x_{n}^1\},~\tilde y_n^1{:}\{\tilde x_n^1,b'_n\},~\tilde x_n^1{:}\{b'_n,b_n\},~b'_n{:}\{b_n,\tilde y_{n-1}^m\},\label{eq:varn}\\
%\nonumber&b_n{:}\{\tilde y_{n-1}^{m},\tilde x_{n-1}^{m}\},~\tilde y_{n-1}^m{:}\{\tilde x_{n-1}^m,\tilde y_{n-1}^{m-1}\},~ ...,~\tilde x_{n-1}^2{:}\{\tilde y_{n-1}^1,\tilde x_{n-1}^1\},~\tilde y_{n-1}^1{:}\{\tilde x_{n-1}^1,b'_{n-1}\},~\tilde x_{n-1}^1{:}\{b'_{n-1},b_{n-1}\},\\ 
%&b'_{n-1}{:}\{b_{n-1},\tilde y_{n-2}^m\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&b_2{:}\{\tilde y_1^m,\tilde x_1^m\},~\tilde y_m^1{:}\{\tilde x_1^m,\tilde y_1^{m-1}\},~ ...,~\tilde x_1^2{:}\{\tilde y_1^1,\tilde x_1^1\},~\tilde y_1^1{:}\{\tilde x_1^1,b'_1\},~\tilde x_1^1{:}\{b'_1,b_1\},~
%b'_1{:}\{b_1,\beta\},\label{eq:var1}\\ 
%\nonumber&b_1{:}\{\beta,\alpha\})
%\end{align}



 
%Given such a path $P$, we construct the corresponding $R'=f(P)$. By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths as follows:
%\begin{eqnarray*}
%P &=& (\alpha\beta,a_1,\beta b_1, a_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (b_{n+1}b'_{n+1},a_3,b'_{n+1}c_1,a_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (c_{m+1}\gamma)
%\end{eqnarray*}
%Given such an arc set $P$, we construct the corresponding $R'=f(P)$. 
%We choose $A' = P$, and set $R' = \triples(A')$, which is consistent by Lemma \ref{lem:consistR}.
By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths:
\begin{align*}
P &~=~ (a_1,a_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (a_3,a_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m},
\end{align*}
where $P_{x_i}$ is one of the two length-$2m{+}2$ subpaths passing through $x_i$'s gadget (from $b_ib'_i$ to $b_{i+1}b'_{i+1}$), $P_{C_j}$ is one of the three length-4 subpaths traversing one of the $C_j$ gadget's three witness paths (from $c_jd_j$ to $c_jc_{j+1}$) {\em plus the succeeding arc with tail $c_jc_{j+1}$}, and $a_1,...,a_4$ are shorthand names for the other four connecting arcs.





For each $C_j$, let $\hat i_j$ denote the index $i$ of the variable $x_i$ appearing in the witness path of $C_j$ (through literal appearance $\tilde x_{\hat i_j}^j$) that $P$ traverses.

Now, consider the {\em reverse linear ordering} shown in Table \ref{tbl:linord} of the A-node-labeled A-edges of Ahograph $[R', L(R')]$, with each subsequence of A-node-labeled A-edges tagged to indicate the corresponding subpath of $P$ (compare to Figs.\ \ref{fig:ahograph} and \ref{fig:overview}, and in particular compare each ($P_{C_j}$) to Fig.\ \ref{fig:clause} and each ($P_{x_i}$) to Fig.\ \ref{fig:var}). %, for an acyclic path $P$: 
%(which takes the positive sides of variable gadgets $x_n,\tilde x_{n-1},\tilde x_1$):

%\begin{table}[t]
%\centering
%\begin{alignat}{7}
%(~&\gamma{:}\{c_m,c_{m+1}\}, ~~&&c_{m+1}{:}\{c_m,\tilde y_{\hat i_m}^m\}, ~~&&\tilde y_{\hat i_m}^m{:}\{c_m,\tilde x_{\hat i_m}^m\}, ~~&&\tilde x_{\hat i_m}^m{:}\{c_m,d_m\},\label{eq:clausem}\tag{$P_{C_m}$}\\
%&d_m{:}\{c_{m-1},c_m\}, ~~&&c_m{:}\{c_{m-1},\tilde y_{\hat i_{m-1}}^{m-1}\}, ~~&&\tilde y_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},\tilde x_{\hat i_{m-1}}^{m-1}\}, ~~&&\tilde x_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},d_{m-1}\},\label{eq:clausemm1}\tag{$P_{C_{m-1}}$}\\
%& ...,\nonumber\\
%&d_2{:}\{c_1,c_2\}, ~~&&c_2{:}\{c_1,\tilde y_{\hat i_1}^1\}, ~~&&\tilde y_{\hat i_1}^1{:}\{c_1,\tilde x_{\hat i_1}^1\}, ~~&&\tilde x_{\hat i_1}^1{:}\{c_1,d_1\},\label{eq:clause1}\tag{$P_{C_1}$}\\
%&d_1{:}\{b'_{n+1},c_1\}, ~~&&c_1{:}\{b_{n+1},b'_{n+1}\},\label{eq:var2clause}\tag{$a_3,a_4$}\\
%&b'_{n+1}{:}\{\tilde y_n^m,b_{n+1}\}, ~~&&b_{n+1}{:}\{\tilde x_n^m,\tilde y_n^m\}, ~~&&\tilde y_n^m{:}\{\tilde y_n^{m-1},\tilde x_n^m\}, ~ \quad..., ~~&&\tilde x_{n}^2 {:}\{\tilde x_{n}^1,\tilde y_{n}^1\},\nonumber\\
%&\quad\tilde y_n^1{:}\{b'_n,\tilde x_n^1\}, ~~&&\tilde x_n^1{:}\{b_n,b'_n\},\label{eq:varn}\tag{$P_{x_n}$}\\
%&b'_n{:}\{\tilde y_{n-1}^m,b_n\}, ~~&&b_n{:}\{\tilde x_{n-1}^{m},\tilde y_{n-1}^{m}\}, ~~&&\tilde y_{n-1}^m{:}\{\tilde y_{n-1}^{m-1},\tilde x_{n-1}^m\},~~ ..., ~~&&\tilde x_{n-1}^2{:}\{\tilde x_{n-1}^1,\tilde y_{n-1}^1\},\nonumber\\
%&\quad\tilde y_{n-1}^1{:}\{b'_{n-1},\tilde x_{n-1}^1\}, ~~&&\tilde x_{n-1}^1{:}\{b_{n-1},b'_{n-1}\},\label{eq:varnm1}\tag{$P_{x_{n-1}}$}\\
%&...,\nonumber\\
%&b'_{2}{:}\{\tilde y_{1}^m,b_{2}\}, ~~&&b_{2}{:}\{\tilde x_{1}^m,\tilde y_{1}^m\}, ~~&&\tilde y_1^m{:}\{\tilde y_1^{m-1},\tilde x_1^m\},~ \quad..., ~~&&\tilde x_1^2{:}\{\tilde x_1^1,\tilde y_1^1\},\nonumber\\
%&\tilde y_1^1{:}\{b'_1,\tilde x_1^1\}, ~~&&\tilde x_1^1{:}\{b_1,b'_1\},\label{eq:var1}\tag{$P_{x_1}$}\\
%&b'_1{:}\{\beta,b_1\}, ~~&&b_1{:}\{\alpha,\beta\})\tag{$a_3,a_4$~}
%\end{alignat}
%\vskip -.5cm
%\caption{Reverse linear ordering.}
%\label{tbl:linord}
%\end{table}



%\ifproofapp
\begin{table}[t]
\caption{Reverse linear ordering of the A-edges corresponding to arcs in path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.}
\vskip -.45cm
\centering
\begin{alignat}{7}
(~&\{c_m,c_{m+1}\}:\gamma, ~~&&\{c_m,\tilde y_{\hat i_m}^m\}:c_{m+1}, ~~&&\{c_m,\tilde x_{\hat i_m}^m\}:\tilde y_{\hat i_m}^m, ~~&&\{c_m,d_m\}:\tilde x_{\hat i_m}^m,\label{eq:clausem}\tag{$P_{C_m}$}\\
&\{c_{m-1},c_m\}:d_m, ~~&&\{c_{m-1},\tilde y_{\hat i_{m-1}}^{m-1}\}:c_m, ~~&&\{c_{m-1},\tilde x_{\hat i_{m-1}}^{m-1}\}:\tilde y_{\hat i_{m-1}}^{m-1}, ~~&&\{c_{m-1},d_{m-1}\}:\tilde x_{\hat i_{m-1}}^{m-1},\label{eq:clausemm1}\tag{$P_{C_{m-1}}$}\\
& ...,\nonumber\\
&\{c_1,c_2\}:d_2, ~~&&\{c_1,\tilde y_{\hat i_1}^1\}:c_2, ~~&&\{c_1,\tilde x_{\hat i_1}^1\}:\tilde y_{\hat i_1}^1, ~~&&\{c_1,d_1\}:\tilde x_{\hat i_1}^1,\label{eq:clause1}\tag{$P_{C_1}$}\\
&\{b'_{n+1},c_1\}:d_1, ~~&&\{b_{n+1},b'_{n+1}\}:c_1,\label{eq:var2clause}\tag{$a_3,a_4$}\\
&\{\tilde y_n^m,b_{n+1}\}:b'_{n+1}, ~~&&\{\tilde x_n^m,\tilde y_n^m\}:b_{n+1}, ~~&&\{\tilde y_n^{m-1},\tilde x_n^m\}:\tilde y_n^m, ~ \quad..., ~~&&\{\tilde x_{n}^1,\tilde y_{n}^1\}:\tilde x_{n}^2,\nonumber\\
&\quad\{b'_n,\tilde x_n^1\}:\tilde y_n^1, ~~&&\{b_n,b'_n\}:\tilde x_n^1,\label{eq:varn}\tag{$P_{x_n}$}\\
&\{\tilde y_{n-1}^m,b_n\}:b'_n, ~~&&\{\tilde x_{n-1}^{m}:b_n,\tilde y_{n-1}^{m}\}, ~~&&\{\tilde y_{n-1}^{m-1},\tilde x_{n-1}^m\}:\tilde y_{n-1}^m,~~ ..., ~~&&\{\tilde x_{n-1}^1,\tilde y_{n-1}^1\}:\tilde x_{n-1}^2,\nonumber\\
&\quad\{b'_{n-1},\tilde x_{n-1}^1\}:\tilde y_{n-1}^1, ~~&&\{b_{n-1},b'_{n-1}\}:\tilde x_{n-1}^1,\label{eq:varnm1}\tag{$P_{x_{n-1}}$}\\
&...,\nonumber\\
&\{\tilde y_{1}^m,b_{2}\}:b'_{2}, ~~&&\{\tilde x_{1}^m,\tilde y_{1}^m\}:b_{2}, ~~&&\{\tilde y_1^{m-1}:\tilde y_1^m,\tilde x_1^m\},~ \quad..., ~~&&\{\tilde x_1^1,\tilde y_1^1\}:\tilde x_1^2,\nonumber\\
&\{b'_1,\tilde x_1^1\}:\tilde y_1^1, ~~&&\{b_1,b'_1\}:\tilde x_1^1,\label{eq:var1}\tag{$P_{x_1}$}\\
&\{\beta,b_1\}:b'_1, ~~&&\{\alpha,\beta\}:b_1~)\tag{$a_3,a_4$}
\end{alignat}
\vskip -.25cm
\label{tbl:linord}
\end{table}
%\else
%\fi




%\begin{alignat}{3}
%(&\gamma{:}\{c_m,c_{m+1}\}, ~~&&c_{m+1}{:}\{c_m,\tilde y_{\hat i_m}^m\}, ~~\tilde y_{\hat i_m}^m{:}\{c_m,\tilde x_{\hat i_m}^m\}, ~~\tilde x_{\hat i_m}^m{:}\{c_m,d_m\},\label{eq:clausem}\\
%&d_m{:}\{c_m,c_{m-1}\}, ~~&&c_m{:}\{c_{m-1},\tilde y_{\hat i_{m-1}}^{m-1}\}, ~~\tilde y_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},\tilde x_{\hat i_{m-1}}^{m-1}\}, ~~\tilde x_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},d_{m-1}\},\label{eq:clausemm1}\\
%& ...,\label{eq:clauses}\\
%&d_2{:}\{c_2,c_2\}, ~~c_2{:}\{c_1,\tilde y_{\hat i_1}^1\}, ~~\tilde y_{\hat i_1}^1{:}\{c_1,\tilde x_{\hat i_1}^1\}, ~~\tilde x_{\hat i_1}^1{:}\{c_1,d_1\},\label{eq:clause1}\\
%&d_1{:}\{c_1,b'_{n+1}\}, ~~c_1{:}\{b'_{n+1},b_{n+1}\},\label{eq:var2clause}\\
%&b'_{n+1}{:}\{b_{n+1},\tilde y_n^m\}, ~~b_{n+1}{:}\{\tilde y_n^m,\tilde x_n^m\}, ~~\tilde y_n^m{:}\{\tilde x_n^m,\tilde y_n^{m-1}\}, ~~ ..., ~~\tilde x_{n}^2 {:}\{\tilde y_{n}^1,\tilde x_{n}^1\}, ~~\tilde y_n^1{:}\{\tilde x_n^1,b'_n\}, ~~\tilde x_n^1{:}\{b'_n,b_n\},\label{eq:varn}\\
%&b'_n{:}\{b_n,\tilde y_{n-1}^m\}, ~~b_n{:}\{\tilde y_{n-1}^{m},\tilde x_{n-1}^{m}\}, ~~\tilde y_{n-1}^m{:}\{\tilde x_{n-1}^m,\tilde y_{n-1}^{m-1}\},~~ ..., ~~\tilde x_{n-1}^2{:}\{\tilde y_{n-1}^1,\tilde x_{n-1}^1\}, ~~\tilde y_{n-1}^1{:}\{\tilde x_{n-1}^1,b'_{n-1}\},\\
%&\quad\tilde x_{n-1}^1{:}\{b'_{n-1},b_{n-1}\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&b'_{2}{:}\{b_{2},\tilde y_{1}^m\}, ~~b_{2}{:}\{\tilde y_{1}^m,\tilde x_{1}^m\}, ~~\tilde y_1^m{:}\{\tilde x_1^m,\tilde y_1^{m-1}\},~~ ..., ~~\tilde x_1^2{:}\{\tilde y_1^1,\tilde x_1^1\}, ~~\tilde y_1^1{:}\{\tilde x_1^1,b'_1\}, ~~\tilde x_1^1{:}\{b'_1,b_1\},\label{eq:var1}\\
%&b'_1{:}\{b_1,\beta\}, ~~b_1{:}\{\beta,\alpha\})
%\end{alignat}



%\begin{align}
%\nonumber(&\gamma{:}\{c_{m+1},c_m\},~ c_{m+1}{:}\{y_m^{i_{w_m}},c_m\},~ y_m^{i_{w_m}}{:}\{x_m^{i_{w_m}},c_m\},~ x_m^{i_{w_m}}{:}\{d_m,c_m\},~ d_m{:}\{c_m,c_{m-1}\},~ c_m{:}\{y_{m-1}^{i_{w_{m-1}}},c_{m-1}\},\\
%& ...,\\
%&c_2{:}\{y_1^{i_{w_1}},c_1\},~ y_1^{i_{w_1}}{:}\{x_1^{i_{w_1}},c_1\},~x_1^{i_{w_1}}{:}\{d_1,c_1\},~ d_1{:}\{c_1,b'_{n+1}\},~c_1{:}\{b'_{n+1},b_{n+1}\},~b'_{n+1}{:}\{b_{n+1},y_n^m\},\label{eq:clauses}\\
%&b_{n+1}{:}\{y_n^m,x_n^m\},~ y_n^m{:}\{x_n^m,y_n^{m-1}\},~ ...,~ x_{n}^2 {:}\{y_{n}^1,x_{n}^1\},~ y_n^1{:}\{x_n^1,b'_n\},~x_n^1{:}\{b'_n,b_n\},~b'_n{:}\{b_n,y_{n-1}^m\},\label{eq:varn}\\
%\nonumber&b_n{:}\{y_{n-1}^{m},x_{n-1}^{m}\},~ y_{n-1}^m{:}\{x_{n-1}^m,y_{n-1}^{m-1}\},~ ...,~ x_{n-1}^2{:}\{y_{n-1}^1,x_{n-1}^1\},~ y_{n-1}^1{:}\{x_{n-1}^1,b'_{n-1}\},~ x_{n-1}^1{:}\{b'_{n-1},b_{n-1}\},\\ 
%&b'_{n-1}{:}\{b_{n-1},y_{n-2}^m\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&b_2{:}\{y_1^m,x_1^m\},~ y_m^1{:}\{x_1^m,y_1^{m-1}\},~ ...,~ x_1^2{:}\{y_1^1,x_1^1\},~ y_1^1{:}\{x_1^1,b'_1\},~ x_1^1{:}\{b'_1,b_1\},~
%b'_1{:}\{b_1,\beta\},\label{eq:var1}\\ 
%\nonumber&b_1{:}\{\beta,\alpha\})
%\end{align}

%Here (\ref{eq:clausem}) corresponds to the portion of $P$ passing through clause $C_m$'s gadget, (\ref{eq:clausemm1}) to the portion passing through $C_{m-1}$'s gadget, (\ref{eq:clauses}) to the portion passing through the gadgets for clauses $C_{m-2},...,C_2$, (\ref{eq:clause1}) through clause $C_1$, (\ref{eq:var2clause}) to the connection from clause $C_1$'s gadget back to variable $x_n$'s gadget (\ref{eq:varn}) through variable $x_n$, (\ref{eq:varnm1}) through $x_{n-1}$, (\ref{eq:othervars}) through variables $x_{n-2},...,x_2$, and (\ref{eq:var1}) through $x_1$'s gadget.

%Observe that for each {\em label$:$edge} entry $k$ for $k < \ell$, that entry's label $o_{k}$ is one of the two A-nodes occurring in entry $k+1$'s (i.e., the preceding entry's) A-edge, say $p_{k+1}$, and crucially, $p_{k+1}$ has no further appearances in the list beyond entry $k$.

Observe the relationship between each {\em A-edge$:$label} entry in the ordering and its predecessor: for each entry $k-1$ for $k \le \ell$, its label $o_{k-1}$ is one of the two A-nodes occurring in entry $k$'s (i.e., the preceding entry's) A-edge, say $p_k$, and crucially, $p_k$ has no further appearances in the list past entry $k-1$. That is, {\em at the start of iteration $k$, $p_k$ is a leaf in the Ahograph}.

Therefore iteration $k$'s removal of the then-isolated A-node $o_k$ and of the (only) label from A-edge $\{p_k,p_k'\}$ disconnects the component that had contained that A-edge in two, thus isolating $p_k = o_{k-1}$ in time for iteration $k-1$. 
%Thus A-edge $\{p_k,p_k'\}$'s removal in iteration $k$ means that $p_k = o_{k-1}$ will be an isolated A-node at the start of iteration $k-1$. 
The remainder of that same component is of course also a tree, thus proving the inductive claim for iteration $k-1$.

%Note also that one of A-edge $\{p_k,p_k'\}$'s two endpoints (say, $p_k$) the {\em label} of the succeeding entry $o_{k-1}{:}\{p_{k-1},p_{k-1}'\}$ (i.e., $p_k=o_{k-1}$) and does not appear as an {\em endpoint} in any subsequent A-edge in the ordering. That is, at the start of the iteration $k$, $p_k$ is a leaf in the Ahograph. Therefore the removal of A-edge $\{p_k,p_k'\}$ means that $p_k = o_{k-1}$ is an isolated A-node at the start of iteration $k-1$. The remainder of that component within the Ahograph is of course still a tree, thus proving the inductive claim.

Since the BUILD algorithm running on $R'$ therefore never encounters a connected Ahograph, it follows \cite{bryant1995extension} that $R'$ is consistent.
%
%%Therefore each removal of the next {\em label$:$edge} entry causes the isolation of the A-node appearing as the subsequent entry's label.
%
%%The initial Ahograph consists of two components, one of which is an isolated A-node ($\gamma$). It has $\ell$ A-edges, corresponding to $P$'s $\ell$ arcs. Every A-node appears (once) as a label, except for $\alpha$ and $\beta$. Thus the Ahograph has $\ell+2$ A-nodes, and its second component is a tree. Therefore each deletion of an A-edge from that second component increases the number of components by one.
%
%Finally, observe that in each iteration, the A-edge deleted is incident to a leaf, thus rendering it an isolated A-node.
%
%
%\textbf{HERE}
%
%
%If $o_k$ nonetheless is still not isolated, that means that triple $p_kq_k | o_k$ was not removed in the previous iteration. 
%
%in each iteration a new A-node $u_k$ becomes isolated
%
%encountering a new isolated A-node in each iteration, 
%
%
%as the process implicitly constructs a caterpillar tree (see Fig.\ \ref{fig:caterpillar}), thus implying that $R'$ is consistent.
\end{proof}
\else
\begin{lemma}\label{lem:consistR}
If there is an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(P)$ is consistent.
\end{lemma}
\fi





\ifproofapp
\vskip .2cm
\noindent\textbf{Lemma \ref{lem:isentailed}.}
If there is an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(P)$ entails $\alpha\beta|\gamma$.
\begin{proof}
%Given such a path $P$, we construct the corresponding $R'=f(P)$. By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths as follows:
%\begin{eqnarray*}
%P &=& (\alpha\beta,a_1,\beta b_1, a_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (b_{n+1}b'_{n+1},a_3,b'_{n+1}c_1,a_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (c_{m+1}\gamma)
%\end{eqnarray*}
%Given such an arc set $P$, we construct the corresponding $R'=f(P)$. 
%We choose $A' = P$, and set $R' = \triples(A')$, which is consistent by Lemma \ref{lem:consistR}.
%By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths:
%\begin{eqnarray*}
%P &=& (a_1,a_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (a_3,a_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (a_5)
%\end{eqnarray*}
%where $P_{x_i}$ is one of the two length-$2m{+}2$ subpaths passing through $x_i$'s gadget (from $b_ib'_i$ to $b_{i+1}b'_{i+1}$), $P_{C_j}$ is one of the three length-4 subpaths passing through $C_j$'s gadget (from $c_jd_j$ to $c_jc_{j+1}$) and including the succeeding connecting arc, and $a_1,...,a_5$ are placeholder names for the other five connecting arcs. 
%More precisely, the paths $P_{x_i}$ and $P_{C_j}$ are all ``half-open'' paths, meaning that they start with a node and end with an arc: $P_{x_i}$ starting with $b_ib'_i$ and ending with one of the two arcs {\em preceding} $b_{i+1}b'_{i+1}$, and $P_{C_j}$ starting with $c_jd_j$ and edging with the (unique) arc {\em preceding} $c_{j+1}d_{j+1}$.
%where $P_{x_i}$ is the path passing through $x_i$'s variable gadget, $P_{C_j}$ is the path passing through $C_j$'s clause gadget, and $a_1,...,a_4$ are placeholder names for the four corresponding connecting arcs. More precisely, the paths $P_{x_i}$ and $P_{C_j}$ are all ``half-open'' paths, meaning that they start with a node and end with an arc: $P_{x_i}$ starting with $b_ib'_i$ and ending with one of the two arcs {\em preceding} $b_{i+1}b'_{i+1}$, and $P_{C_j}$ starting with $c_jd_j$ and edging with the (unique) arc {\em preceding} $c_{j+1}d_{j+1}$.

%Recalling that each 1-2-hyperarc represents a rooted triple in $R$, we add to $R'$ the triple corresponding to each arc appearing in $P$, i.e., $R' = \{r(a) : a \in P\}$, where $r(e)$ denotes the triple represented by $$.
%
Let $\ell=|P|$, and for each $k \in [\ell]$, let $a_k = u_k{\to}\{v_k,v_k'\}$ denote the $k$th arc in $P$, with $u_k = p_kq_k$ and $\{v_k,v_k'\} = \{p_ko_k, q_ko_k \}$ (for some leaves $p_k,q_k,o_k$), representing triple $p_k q_k | o_k = u_k | o_k$. The names $v_\ell,v_\ell'$ can be assigned so that $v_\ell = c_{m+1}\gamma$ (and $v_\ell'$ is $a_\ell$'s non-destination sink node $c_m \gamma$), but we can also simply represent $a_\ell$ as $u_\ell|o_\ell = c_mc_{m+1} | \gamma$.
%so hyperarc $a_\ell = u_\ell{\to}\{v_\ell, v_\ell'\}$, representing triple $u_\ell|o_\ell = p_\ellq_\ell | o_\ell = c_mc_{m+1} | \gamma$. 
Similarly, for each $k \in [2,...,\ell]$, we can assign the names $v_{k-1},v_{k-1}'$ so that $v_{k-1}=u_k$, i.e., $\text{t}(a_k) = u_k = v_{k-1} \in \text{h}(a_{k-1})$,
%and so hyperarc $a_{k-1} = u_{k-1}{\to}\{u_k, v_{k-1}'\}$, representing triple $p_{k-1}q_{k-1} | o_{k-1} = u_{k-1}|o_{k-1}$.
and we can also simply represent $a_{k-1}$ as $u_{k-1}|o_{k-1}$.

Now consider arcs $a_{\ell-1}$ and $a_\ell$, and observe that their representations as $u_{\ell-1}|o_{\ell-1}$ and $u_\ell|o_\ell$ (respectively) are 
%$a_{\ell-1} = u_{\ell-1}{\to}\{u_\ell, v_{\ell-1}'\}$ and $a_\ell = u_\ell{\to}\{v_\ell, v_\ell'\}$, representing triples $u_{\ell-1}|o_{\ell-1}$ and $u_\ell|o_\ell$, respectively, and observe that this pair of triples is 
of exactly the form that dyadic inference rule (\ref{eq:2b}) applies to: via that inference rule, we can derive the triple $u_{\ell-1}|o_\ell$, which have the form $c_m \tilde y_i^m | \gamma$ (for some $i$). % or $c_j \bar y_i^m | \gamma$.

%, where the names $v_k,v_k'$ are assigned so that $v_k$ is $u_k$'s successor on $P$, i.e., $v_k = u_{k+1}$ (except when $k=\ell$, in which case $v_k=c_{m+1}\gamma$), and therefore, $u_k=v_{k-1}$, i.e., $u_k = \text{t}(a_k) \in \text{h}(a_{k-1}) = \{v_{k-1},v_{k-1}'\}$
%
%That is, $\text{t}(a_k) = p_kq_k$, and $o_{k-1} \in \{p_k, q_k\}$ and $|\{p_k, q_k\} \cap \{p_{k-1}, q_{k-1}\}|=1$, and so $a_k$ represents $p_k q_k | o_k$. Then observe that by applying the second dyadic inference rule (recall Def.\ \ref{def:2ord}) to the triples represented by the path's last two arcs (i.e., $p_{\ell-1} q_{\ell-1} | o_{\ell-1}$ and $p_\ell q_\ell | o_\ell$), we can infer $p_{\ell-1} q_{\ell-1} | o_\ell$. 

Similarly, by applying this inference rule to the triple represented $P$'s third-to-last arc (i.e., $u_{\ell-2} | o_{\ell-2}$) and the derived triple  $u_{\ell-1} | o_\ell$, we can derive $u_{\ell-2} | o_\ell$. Via a total of $\ell-1$ such applications of dyadic inference rule (\ref{eq:2b}) (each corresponding to one BUILD iteration), we can derive $u_1 | o_\ell = p_1 q_1 | o_\ell$ = $\alpha \beta | \gamma$.
%
%Second, by Lemma \ref{lem:consistR} proved below, $R'$ is indeed consistent.
\end{proof}
\else
\begin{lemma}\label{lem:isentailed}
If there is an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(P)$ entails $\alpha\beta|\gamma$.
\end{lemma}
\fi

%Thus we have:
%
%\vskip .2cm
%\noindent\textbf{Corollary \ref{cor:consentails} ($\Leftarrow$).}
%%Let $A' \subseteq A$. 
%If there is an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(P)$ is consistent and entails $\alpha\beta|\gamma$.
%%there exists a subset $A' \subseteq A$ for which $R' = \triples(A')$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
%\else
Thus we have:

\ifproofapp
\vskip .2cm
\noindent\textbf{Corollary \ref{cor:consentails}.}
If there is an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(P)$ is consistent and entails $\alpha\beta|\gamma$.
\else
\begin{corollary}[$\Leftarrow$]\label{cor:consentails}
If there is an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(P)$ is consistent and entails $\alpha\beta|\gamma$.
\end{corollary}
\fi






%mpj
%\newpage


\ifproofapp
%mpj
\begin{figure}%[t!]
\centering
	\begin{subfigure}{\textwidth}
\centering
%\input{triples-fig-var-leaves}
%\captionsetup{justification=centering}
%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%\input{triples-fig-tree}
\makebox[1\textwidth][c]{ %\hskip -2cm
\includegraphics[width=1\textwidth]{rt-fig-ahopath-arx.pdf}
}
%\vskip .05cm
%\vskip -.05cm
\caption{The initial Ahograph $[R',L(R')]$ constructed based on an underlying {\em acyclic} path $P$. Because $P$ is acyclic, the node  $\tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j$ pointed to by each $C_j$'s witness node $c_j \tilde x_{\hat i_j}^j$ is a {\em sink node in $H$}, and thus A-nodes $\tilde y_i^j$ and $\tilde x_i^j$ are {\em leaves in the Ahograph}. As a result, at each BUILD iteration, the Ahograph has two components, a tree and an isolated node.
%, distinct from the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets.% (as occurs in Fig.\ \ref{fig:ahocycle}).
%
%Because $P$ is acyclic, 
%, where $P$ is an acyclic path in the hypergraph from $\alpha\beta$ to $c_{m+1}\gamma$,
%%(specifically, the red path shown in Fig.\ \ref{fig:overview}), 
%and $R'=\triples(P)$. 
%%Here $x_2$ is false and $x_1,x_3,x_4$ are true, and the witness literals for clauses $C_1,C_2,C_3,C_4$ are $\bar x_n, \bar x_1, \bar x_n, \bar x_1$, respectively. 
%%If $P$ had contained a cycle involving some clause $C_j$, then $C_j$'s $x$ and $p$ nodes in the resulting Ahograph would have 
%Let $\tilde x_i^j \tilde y_i^j$ be the variable gadget node pointed to by the $C_j$ clause's witness node. Then, because $P$ is acyclic, A-nodes $\tilde x_i^j$ and $\tilde y_i^j$ are both leaves {\em in the Ahograph}, rather than appearing in the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets (as occurs in Fig.\ \ref{fig:ahocycle}).
\label{fig:ahograph}
}
%\end{figure}
%\begin{figure}[t!]
\end{subfigure}
\vskip .5cm
\centering
	\begin{subfigure}{\textwidth}
\centering
%\captionsetup{justification=centering}
%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%\input{triples-fig-tree}
\includegraphics[width=.75\textwidth]{rt-fig-ahocycle-arx.pdf}
%\vskip .05cm
%\vskip -.05cm
\caption{A fragment of the Ahograph resulting from the cause of a cycle in $P$, viz., a back-arc in which some clause $C_j$'s witness node $c_j \tilde x_{\hat i_j}^j$ points to a {\em non-sink} node $\tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j$ that lies earlier in the path $P$ (specifically, within $x_{\hat i_j}$'s gadget), and thus A-nodes $\tilde y_{\hat i_j}^j$ and $\tilde x_{\hat i_j}^j$ are {\em non-leaves} in the Ahograph. This yields the triangle $c_j-\tilde y_{\hat i_j}^j - \tilde x_{\hat i_j}^j$. After the BUILD iteration in which A-node $c_{j+1}$ and A-edge $\{c_j, \tilde y_{\hat i_j}^j\}$ are removed, $\tilde y_{\hat i_j}^j$ will still {\em not} be isolated, and hence the Ahograph will at that point consist of a single component, indicating $R'$ is inconsistent.
%Ahograph $[R',L(R')]$, where $P$ is an acyclic path in the hypergraph from $\alpha\beta$ to $c_{m+1}\gamma$ (specifically, the red path shown in Fig.\ \ref{fig:overview}), and $R'=\triples(\arcs(P))$. Here $x_2$ is false and $x_1,x_3,x_4$ are true, and the witness literals are $\tilde x_n, \tilde x_1, \tilde x_n, \tilde x_1$ for clauses $C_1,C_2,C_3,C_4$, respectively. 
%%If $P$ had contained a cycle involving some clause $C_j$, then $C_j$'s $x$ and $p$ A-nodes in the resulting Ahograph would have  
%Because $P$ is acyclic, each clause $C_j$'s $x$ and $p$ A-nodes are leaves {\em in the Ahograph}, rather than being A-nodes in the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets. 
\label{fig:ahocycle}
}
\end{subfigure}
\caption{The Ahograph $[R',L(R')]$ is constructed when Aho et al.'s BUILD algorithm is executed on the triples $R' = \triples(P)$ corresponding to the path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$. The existence of any cycle within $P$ involving some clause $C_j$'s witness node $c_j \tilde x_{\hat i_j}^j$ pointing to $\tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j$ (i.e., arc $c_j \tilde x_{\hat i_j}^j \to \{c_j \tilde y_{\hat i_j}^j, \tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j\}$) will be reflected in the locations in the Ahograph of A-nodes $\tilde y_{\hat i_j}^j$ and $\tilde x_{\hat i_j}^j$.}
\end{figure}






\begin{figure}
\centering
\includegraphics[width=1\textwidth]{rt-fig-ahoincompgr-arx.pdf}
%\vskip -,25cm
\caption{The Ahograph $[R',L(R')]$ for $R'=\triples(A')$, where $A'$ is a maximal acyclic subset of $A$ and the three variable gadgets shown (for $x_1,x_2,x_n$) are each maximal in the sense that both sides are included and the three clause gadgets shown (for $C_1,C_2,C_m$) are each maximal in the sense that all three witness paths are included. (Hence all the appearances within clauses $C_1,C_2,C_m$ must be of variables $x_3,...,x_{n-1}$.) If there is no disconnection between either $b_2$ and $b'_n$ or $c_2$ and $c_m$, then the Ahograph is connected and $R'$ is inconsistent.\label{fig:ahoincompgr}
}
%none of $x_1,x_2,x_n$ appear in any of $C_1,C_2,C_m$.)}
%\end{figure}
%
%
\vskip .5cm
%\begin{figure}[t!]
\centering
\includegraphics[width=.95\textwidth]{rt-fig-ahodiscordvar-arx.pdf}
\vskip -,05cm
\caption{A fragment of the Ahograph corresponding to a variable $x_i$'s gadget (see Fig.\ \ref{fig:var}) if its only two arcs missing from $A'$ are $\arcs(b_ib'_i|x_i^1, ~\bar y_i^m|b_{i+1}|b'_{i+1})$, with the A-edge we consider hypothetically adding in the proof of Lemma \ref{lem:degeneratecutpath} shown dashed.\label{fig:ahodiscordvar}
}
\end{figure}
\else
\fi
























\subsection{Consistent Entailing Subset $\Rightarrow$ Acyclic Path}

Now we argue for the reverse direction, % (or rather, its contrapositive), %, that satisfying truth assignments correspond to acyclic paths, 
proving through a series of lemmas that if there is no acyclic $\alpha\beta{-}c_{m+1}\gamma$ path, then there will be no consistent triple subset entailed $\alpha\beta|\gamma$.
%via a proof that will depend on two subsequent lemmas proved below.


\ifproofapp
\vskip .2cm
\noindent\textbf{Corollary \ref{lem:cycpath}.}
Let $A' \subseteq A$. Suppose there exists a {\em cyclic} path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then $R' = \triples(A')$ is inconsistent.
\begin{proof}
Intuitively, it can be seen that any cycle in $H$ corresponds to a vicious (inconsistent) cycle of rooted triples. In particular (see Fig.\ \ref{fig:ahocycle}), any clause $C_j$'s component whose witness node points to a variable gadget node already visited on the path (causing a cycle in $H$) will induce a triangle {\em in the Ahograph}, resulting in a single-component Ahograph in the BUILD iteration following the deletion of isolated node $c_{j+1}$ (if no single-component Ahograph has yet been encountered in an earlier iteration), since at that point A-node $\tilde y_{\hat i_j}^j$ will have failed to become isolated.
\end{proof}
\else
\begin{lemma}\label{lem:cycpath}
Let $A' \subseteq A$. Suppose there exists a {\em cyclic} path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then $R' = \triples(A')$ is inconsistent.
\end{lemma}
\fi

Most of the remainder of this subsection will be dedicated to showing {\em constructively} that if $A'$ contains no path from $\alpha\beta$ to $c_{m+1}\gamma$ at all, cyclic or otherwise, then $R'$ does not entail $\alpha\beta|\gamma$. We do so by showing that in the case of such a (consistent) $R'$, there exist trees displaying $R' \cup \{\alpha\beta|\gamma\}$. Therefore assume w.l.o.g.\ that $R'$ is consistent and maximal in the sense that adding any other triple of $R$ to it would either make $R'$ inconsistent or would introduce an $\alpha\beta{-}c_{m+1}\gamma$ path in $A'=\arcs(R')$.
%The remainder of the proof in this subsection will be to show (constructively) that if there exists a consistent $R'$ entailing $\alpha\beta|\gamma$ then there exists a path from $\alpha\beta$ to $c_{m+1}\gamma$.
%$A'$ subsumes no path from $\alpha\beta$ to $c_{m+1}\gamma$ at all, cyclic or otherwise, then $R'$ will not entail $\alpha\beta|\gamma$. Therefore assume w.l.o.g.\ that $R'$ is consistent.
%
%We begin by defining some notation.

Observe that the missing arcs $A^\times = A - A'$ can be thought of as the (source side to sink side) cross arcs of a cut separating source $\alpha\beta$ and sink $c_{m+1}\gamma$.
%
In the following argument we will refer to hypergraph $H^\gamma = (V \cup \{ \gamma\alpha\}, A' \cup \arc(\gamma\alpha|\beta))$ and its corresponding Ahograph $G^\gamma$.

% mpj
%Let $S(\alpha \beta,V,A') \subseteq V$ (written $V_{\alpha\beta}$) be the set of all nodes reachable from $\alpha \beta$ via the nodes $V$ and the arcs $A'$, and let $P(c_{m+1}\gamma,V,A') \subseteq V$ (written $V_{c_{m+1}\gamma}$) be the set of all nodes that $c_{m+1}\gamma$ is reachable {\em from} via $V$ and $A'$, and set $V' = V_{\alpha\beta} \cup V_{c_{m+1}\gamma}$ Then by assumption $V_{\alpha\beta}$ and $V_{c_{m+1}\gamma}$ are disjoint. That is, the subhypergraph of $(V,A')$ induced by $V'$ has two components.
%
%Let $V_{\alpha \beta}^* \subseteq V_{\alpha\beta}$ be the maximal elements of $V_{\alpha\beta} $ in the sense that every $u \in V_{\alpha \beta}^*$ is reachable from $\alpha\beta$ but no other node $v \in V_{\alpha\beta}$'s reachability {\em depends on} $u$. That is, $S(\alpha \beta,V-\{u\},A') = S(\alpha \beta,V,A') - \{u\}$. Similarly, let $V_{c_{m+1}\gamma}^* \subseteq V_{c_{m+1}\gamma}$ be the minimal elements of $V_{c_{m+1}\gamma}$ in the sense that for any $v \in V_{c_{m+1}\gamma}^*$, there is no other node $u \in V_{c_{m+1}\gamma}$ dependent on $v$, i.e., $P(c_{m+1}\gamma,V-\{v\},A') = P(c_{m+1}\gamma,V,A')-\{v\}$.


%\begin{lemma}[$\Rightarrow$]\label{lem:notentailed}
%%If $R'$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$, then $A' = \arcs(R')$ contains the arcs of an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%%
%%Let $A' \subseteq A$. not
%Suppose there is no acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then for every subset $A' \subseteq A$, $R' = \triples(A')$ is  inconsistent or does not entail $\alpha\beta|\gamma$.
%%If $A' \subseteq A$ is {\em not} an acyclic arc set subsuming the set $P$ of arcs appearing in some path from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(A')$ is not a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
%\end{lemma}
%\begin{proof}
%%Given such a subset $R'$, we construct the corresponding $P=f^{-1}(R')$.
%%Let $A' \subseteq A$ be an arbitrary subset of $A$, and set $R' = \triples(A')$.
%
%%First, suppose there {\em is} a path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then $P$ must be cyclic, and thus $\triples(P) \subseteq R'$ will be inconsistent. 
%
%%Second, suppose there is no path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ having $P \subseteq A$, cyclic or otherwise. If $A'$ is cyclic then $R' = \triples(A')$ will again be inconsistent, so assume $A'$ is acyclic. Now we will show constructively that in this case, $R'$ does not entail $\alpha\beta|\gamma$.
%
%
%
%%By Lemma \ref{lem:uvpairs} proved below, we can assume w.l.o.g.\ that there are at most 3 $u^*$s and at most 3 $v^*$s, which together yield either 1, 2, or 3 pairs $(u_h,v_h)$, with each pair connected by an arc $a_h \in  A - A'$.
%
%%Then by Lemma \ref{lem:treeexs} proved below, we can build a tree displaying $\triples(A') \cup \{\alpha\gamma | \beta\}$ (see Fig.\ \ref{fig:nopathtree}). This shows that $R' \cup \{\alpha\gamma | \beta\}$ is consistent, and thus that $R'$ does not entail $\alpha\beta | \gamma$.
%%
%%
%%
%%
%%
%%
%%%\textbf{but then there's a tree satisfying $R'$ and not $\alpha\beta|\gamma$}
%%
%%
%%First observe that the only triple in $R$ including $\alpha$ or $\beta$ is $\alpha\beta | b_1$, and so any hypothetical subset $R' \subset R$ pseud o-entailing $\alpha\beta|\gamma$ must necessarily include $\alpha\beta | b_1$.  But then observe that the only other triple in $R$ including $\alpha$ or $\beta$ is $\beta b_1 | b'_1$, so it must be included. Next, observe that the only other triples in $R$ including $\beta$ or $b_1$ are $b_1b'_1 | x_i^1$ and $b_1b'_1 | \bar x_i^1$, so at least one of them must be included. We claim that by repeated application of arguments of this kind, we obtain that the arcs corresponding to the triples of any such $R'$ must trace out a path from $\alpha\beta$ to $c_{m+1}\gamma$.
%%
%%Second, observe that if $P$ contained a cycle, then the triples corresponding to the hyperarcs appearing in that cycle would themselves be inconsistent, contradicting the consistency of $R'$.
%\end{proof}





% mpj
%\begin{lemma}\label{lem:uvpairs}
%Suppose $A' \subseteq A$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. Let $V_{\alpha \beta}^* \subseteq V_{\alpha\beta}$ and $V_{c_{m+1}\gamma}^* \subseteq V_{c_{m+1}\gamma}$ be defined as above.
%%in the proof of Lemma \ref{lem:notentailed} above. 
%Then $|V_{\alpha \beta}^*| = |V_{c_{m+1}\gamma}^*| \in [3]$, 
%%and there is bijection between $V_{\alpha \beta}^*$ and $V_{c_{m+1}\gamma}^*$, with each pair corresponding to a unique A-edge in $A-A'$.
%%By Lemma \ref{lem:uvpairs} proved below, we can assume w.l.o.g.\ that there are at most 3 $u^*$s and at most 3 $v^*$s, 
%which (w.l.o.g.) together yield $w \in [3]$ ordered pairs $\{(u_h,v_h) : h \in [w]\}$ and a set of arcs $A^\times$, where each pair is connected by a unique arc $a_h \in A^\times \subseteq A - A'$.
%\end{lemma}
%\begin{proof}
%First, we claim we can assume w.l.o.g.\ that for no $u^* \in V_{\alpha\beta}^*$ will the path to it from $\alpha\beta$ cross a back-arc, i.e., a subpath taking an arc of the form $c_j \tilde x_i^j{\to}\{c_j\tilde y_i^j, \tilde x_i^j\tilde y_i^j\}$ to reach a node $\tilde x_i^j\tilde y_i^j$ {\em for the first time} (see Fig.\ \ref{fig:clause}). Preceding $c_j \tilde x_i^j$, the path would have had to visit $c_jd_j$, and if after crossing the back-arc the path is going (via additional A-edges from $A$ we add later) to eventually reach $c_{m+1}\gamma$, then it would have to visit $c_jd_j$ again, making it cyclic and $R'$ inconsistent.
%
%Second, we claim we can assume w.l.o.g.\ that for no $v^* \in V_{c_{m+1}\gamma}^*$ will its path to $c_{m+1}\gamma$ will contain back-arcs.
%%, i.e., a subpath taking an arc of the form $c_j \tilde x_i^j{\to}\{c_j\tilde y_i^j, \tilde x_i^j\tilde y_i^j\}$ to $\tilde x_i^j\tilde y_i^j$. 
%To see this, consider (see Fig.\ \ref{fig:clause}) what node $v^*$ could possibly benefit (in terms of reaching $c_{m+1}\gamma$) from such a path. If $v^*=c_jd_j$ (or any of its immediate predecessors) for some $j$, then the path from $v^*$ to $c_{m+1}\gamma$ would again have to eventually return to $c_jd_j$ again, making the path cyclic. If $v^*= c_j \tilde x_i^j$ for some $j,i$, then it is not impossible per se for there to be an acyclic path from it to $c_{m+1}\gamma$ traversing a back-arc. The only possible arc that could be used for reaching $c_j \tilde x_i^j$, however, is the one from $c_jd_j$, in which case once again any resulting path from $\alpha\beta$ to $c_{m+1}\gamma$ would be cyclic.
%
%Now, how far are the elements of $V_{\alpha\beta}$ away from the elements of $V_{c_{m+1}\gamma}$? That is, how many arcs from $A$ would have to be added to $A'$ in order to reach a node $v \in  V_{c_{m+1}\gamma}$ from a node $u^* \in V_{\alpha \beta}^*$ or to reach a node $v^* \in  V_{c_{m+1}\gamma}^*$ from a node $u \in V_{\alpha \beta}$?
%
%Since our eventual goal is to show that $R' = \triples(A')$ does {\em not} entail $\alpha \beta | \gamma$, we assume w.l.o.g.\ the most difficult case, i.e., that any $v^* \in V_{c_{m+1}\gamma}^*$ is only one hop away from some $u \in V_{\alpha \beta}$, via some arc $a \in A - A'$, the addition of which to $A'$ would complete a path from $\alpha\beta$ to $c_{m+1}\gamma$. Conversely, we can assume w.l.o.g.\ that for every $u^* \in V_{\alpha \beta}^*$ there exists an A-edge $a \in A-A'$ that would connect it to some $v \in V_{c_{m+1}\gamma}$. If $A^\times$ is the set of all arcs $a$ playing this role for some $u^*$ and/or $v^*$, then observe that $(V_{\alpha \beta}^*,V_{c_{m+1}\gamma}^*)$ is a {\em directed cut} separating $\alpha\beta$ from $c_{m+1}\gamma$ in the hypergraph $H^\times = (V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^*, A' \cup A^\times)$, and $A^\times$ consists of the (forward) {\em cross-arcs} of that cut.
%
%Now, how many arcs could there be in $A^\times$? By inspection of the hypergraph construction, it can be seen that $|A^\times|$ will be either 2, 3, or 1, depending (respectively) on whether the cut occurs within a variable gadget, within a clause gadget, or elsewhere.\footnote{Note that the cross-arcs can connect members of $V_{\alpha\beta}^*$ to $V_{c_{m+1}\gamma}$ and members of $V_{\alpha\beta}$ to $V_{c_{m+1}\gamma}^*$, not just members of $V_{\alpha\beta}^*$ to $V_{c_{m+1}\gamma}^*$. Consider, for example, a cut through variable $x_i$'s gadget cutting arcs $b_ib'_i{\to}\{b'_ix_i^1,b_ix_i^1\}$ and $\bar y_i^mb_{i+1}{\to}\{b_{i+1}b'_{i+1},\bar y_i^mb'_{i+1}\}$ but with all other arcs of $x_i$'s gadget present in $A'$. In this case, $b_ib'_i \in V_{\alpha\beta} - V_{\alpha\beta}^*$ and $b_{i+1}b'_{i+1} \in V_{c_{m+1}\gamma} - V_{c_{m+1}\gamma}^*$.}
%%Note also that due to hypergraph construction there will be a bijection between $u^*$s and $v^*$s. To see this, recall that the only arcs in which both heads are non-sink nodes are those in which a clause gadget's witness node $c_j \tilde x_i^j$ points back to a variable gadget node $\tilde x_i^j \tilde y_i^j$. But we have seen that no $u^*$'s path will contain a back-arc. Therefore if $A^\times$ contains an A-edge of the form $c_j \tilde x_i^j{\to}\{c_j \tilde y_i^j, \tilde x_i^j \tilde y_i^j\}$, it must be due to $u^*=c_j \tilde x_i^j$ and $v^*=c_j \tilde y_i^j$.
%\end{proof}
%







\ifproofapp
\begin{figure}
\centering
\makebox[1\textwidth][c]{ %\hskip -3.75cm
%    \captionsetup{width=.9\linewidth}%
   \centering
\ifwabi
   \begin{subfigure}[t]{.14\linewidth}
\clipbox{6.15cm .15cm 5.65cm .5cm}{      \includegraphics[height=.535\textheight,angle=33]{rt-fig-pathtree-arx.pdf}  }
\else
   \begin{subfigure}[t]{.12\linewidth}
\clipbox{6.25cm .15cm 5.75cm .5cm}{      \includegraphics[height=.535\textheight,angle=31.75]{rt-fig-pathtree-arx.pdf}  }
\fi
\caption{$A'$ is an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$.
%The caterpillar tree determined by the triples corresponding to $P$, which thence satisfies $\alpha\beta|\gamma$.
\label{fig:pathtree}
}
  \end{subfigure}
\ifwabi
\hskip .3cm
  \begin{subfigure}[t]{.26\linewidth}
\else
\hskip .35cm
  \begin{subfigure}[t]{.28\linewidth}
\fi
    \centering
    %\captionsetup{width=1.1\linewidth}%
\ifwabi
\clipbox{2.5cm .15cm 1.5cm 1.4cm}{      \includegraphics[height=.21\textheight,angle=35.6]{rt-fig-cuttreeforced-arx.pdf} }
\else
\clipbox{2.6cm .15cm 1.6cm 1.45cm}{      \includegraphics[height=.22\textheight,angle=33.6]{rt-fig-cuttreeforced-arx.pdf} }
\fi
\caption{$A^\times$ contains some forced arc $a_\times$.
%A tree consistent with $A'$, i.e., displaying all of $R'=\triples(A')$, but {\em not} displaying $\alpha \beta | \gamma$.
%The tree that can be constructed displaying all triples in $R'=\triples(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. 
%The root's left subtree contains all leaves appearing in A-nodes before the ``cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
\label{fig:cuttreeforced}
}
  \end{subfigure}
\ifwabi
\hskip .35cm
\else
\hskip .35cm
\fi  \begin{subfigure}[t]{.28\linewidth}
    \centering
    %\captionsetup{width=1.1\linewidth}%
\ifwabi
\clipbox{5.45cm .15cm 4.45cm 1.4cm}{      \includegraphics[height=.455\textheight,angle=34.6]{rt-fig-cuttreevar-arx.pdf} }
\else
\clipbox{5.75cm .15cm 4.7cm 1.25cm}{      \includegraphics[height=.47\textheight,angle=33.6]{rt-fig-cuttreevar-arx.pdf} }
\fi
\caption{$A^\times$ contains $\arcs($ $z_i^\ell z_i^{\ell+1}|z_i^{\ell+2}, ~ \bar z_i^{ell'} \bar z_i^{\ell'+1}|\bar z_i^{\ell'+2})$, where either both or neither of $z_i^\ell,\bar z_i^{\ell'}$ equal $b_i$.
%A tree consistent with $A'$, i.e., displaying all of $R'=\triples(A')$, but {\em not} displaying $\alpha \beta | \gamma$.
%The tree that can be constructed displaying all triples in $R'=\triples(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. 
%The root's left subtree contains all leaves appearing in A-nodes before the ``cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
\label{fig:cuttreevar}
}
  \end{subfigure}
\ifwabi
\hskip .45cm
  \begin{subfigure}[t]{.3\linewidth}
\else
\hskip .35cm
  \begin{subfigure}[t]{.28\linewidth}
\fi
    \centering
    %\captionsetup{width=1.1\linewidth}%
%\hskip -.35cm
\ifwabi
\clipbox{7.05cm 1.05cm 5.85cm .55cm}{   \includegraphics[height=.7\textheight,angle=32.75]{rt-fig-cuttreeclause-arx.pdf} }
\else
\clipbox{7.5cm 1.15cm 6.25cm .5cm}{   \includegraphics[height=.73\textheight,angle=31.75]{rt-fig-cuttreeclause-arx.pdf} }
\fi
%\adjincludegraphics[height=5cm,clip,bb = 0 10 612 100,angle=30]{rt-fig-cuttreeclause-arx.pdf}
%    \fbox{\tikz{
%            \clip[use as bounding box] (0,0)++(.01\textwidth,.01\textwidth) rectangle ++(.45\textwidth,.45\textwidth);
%\draw (0,0) node[inner sep=0pt,name=micrograph]{\includegraphics[angle=10,width=1.6\textwidth]{rt-fig-cuttreeclause-arx.pdf}};
%\draw[ultra thick, white] (micrograph.south west)++(0.05*0.5\textwidth,0.05*0.5\textwidth)--++(0.5*0.25806\textwidth,     0)node[above,white,midway]{}};}
%}
\caption{$A^\times$ contains three arcs lying with clause $C_j$'s gadget.
%A tree consistent with $A'$, i.e., displaying all of $R'=\triples(A')$, but {\em not} displaying $\alpha \beta | \gamma$.
%The tree that can be constructed displaying all triples in $R'=\triples(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. 
%The root's left subtree contains all leaves appearing in A-nodes before the ``cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
\label{fig:cuttreeclause}
}
  \end{subfigure}
 }
%
%
%%\captionsetup{justification=centering}
%%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%%\input{triples-fig-tree}
%\includegraphics[height=.5\textheight]{triples-fig-pathtree.pdf}
%%\vskip .05cm
%\vskip -.1cm
%\caption{The caterpillar tree resulting from the triples corresponding to $P$, which thence satisfies $\alpha\beta|\gamma$.}
%\label{fig:caterpillar}
%\vskip .1cm
%\centering
%%\captionsetup{justification=centering}
%%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%%\input{triples-fig-tree}
%\includegraphics[height=.5\textheight]{triples-fig-nopathtree.pdf}
%%\vskip .05cm
%%\vskip -.05cm
\caption{Trees resulting from triples corresponding to an acyclic arc set $A' \subseteq A$ in $H$ that (a) do or (b,c,d) do not contain a path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$, for different cases of $A'$ and $A^\times = A-A'$. Leaves corresponding to isolated A-nodes in the tree's Ahograph are shown with thick dashed borders, and the leaves corresponding to A-nodes that {\em become} isolated when those isolated A-nodes are removed are shown with thin dashed borders. In (b,c,d), leaves within the two major subtrees are also shown thus, with respect to those subtrees' Ahographs.
%The tree that can be constructed displaying all triples in $R'=\triples(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. The root's left subtree contains all leaves appearing in A-nodes before the ``directed cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
}
\end{figure}
\else
\fi



%Let $H^* = (V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^*, A')$, $H^\gamma = (V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^* \cup \{ \gamma\alpha\}, A' \cup \arc(\gamma\alpha|\beta))$, $H^\times = (V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^*, A' \cup A^\times)$, and $H^{\times\gamma} = (V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^* \cup \{ \gamma\alpha\}, A' \cup A^\times \cup \arc(\gamma\alpha|\beta))$, and let $G^*$, $G^\gamma$, $G^\times$, and $G^{\times\gamma}$ be the corresponding Ahographs (respectively).
%
%
% mpj
%$G^*$ and $G^\times$ each have (at least) two components because no triple in either of the corresponding triple sets has $\gamma$ on the LHS, whereas $G^*$ may consist of three components, due to $\gamma$ and (potentially) to the cut $A^\times$. By definition, $H^\times$ contains an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$. Running BUILD on $\triples(P)$ will produce a caterpillar tree (see Fig.\ \ref{fig:pathtree}), via an Ahograph consisting of a tree and an isolated node $\gamma$ (see Fig.\ \ref{fig:ahograph}).
%
%Since $H^{\times\gamma}$ contains $P$ as well as $\arc(\gamma\alpha|\beta)$, $\gamma$ is not an isolated A-node in $G^{\times\gamma}$, which is connected, and so BUILD will fail when run on $G^{\times\gamma}$. 

Recalling the construction of $H$, there are three types of places where the absent cross-arcs $A^\times$ could be located: within a clause gadget, within a variable gadget, or elsewhere, i.e., {\em forced arcs} (viz., connecting arcs $a_1,...,a_4$ or arcs with tail of the form $c_j c_{j+1}$ following a clause $C_j$'s gadget). There is one special subcase, which we give a name to.

\begin{definition}
We call $A^\times$ {\em degenerate} if $A^\times$ lies within a variable $x_i$'s gadget, $|A^\times|=2$, and exactly one of its members has the form $\arc(b_ib'_i|\tilde x_i^1)$. (Its other member must by definition lie within the $x_i$ gadget's opposite side.) %Otherwise, $A^\times$ is {\em non-degenerate}.
\end{definition}

We deal with all cases besides an degenerate $A^\times$ in the following lemma.


\ifproofapp
\vskip .2cm
\noindent\textbf{Lemma \ref{lem:treeexs}.}
Let $R'$ be consistent.
Suppose there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$, and that $A^\times$ is non-degenerate.
Then $R'$ does not entail $\alpha\beta|\gamma$.
\begin{proof}
%Now we will show that for such an $A''$, $R' = \triples(A'')$ is compatible with $\alpha\beta | \gamma$ not holding.
%
%Let $w \in [3]$ be the number of pairs $(u_h^*,v_h^*)$. 
%By Lemma, \ref{lem:uvpairs} there are $w \in [3]$ ordered pairs $\{(u_h,v_h) : h \in [w]\}$, with each pair connected (w.l.o.g.) by a unique arc $a_h \in A^\times \subseteq A - A'$.

First, suppose $A^\times$ contains any of the forced arcs, say $a_\times$, corresponding to a triple $p_\times q_\times|o_\times$. % and also to A-edge $\{p_\times,q_\times\}$ in $G^\times$.
%Arc $a_\times$ could be either a connecting arc, an arc in one side of a variable gadget (where none of the other side's arcs are included in $A'$, or an arc in one witness path of a clause gadget (where none of its other witness paths' arcs are included in $A'$). 
Now, consider the effect of the corresponding A-edge $\{p_\times,q_\times\}$'s absence from $G^\gamma$: $p_\times$ and $q_\times$ must lie in different components of it, since (observe) the only multi-edges in $G^\gamma$ are $\{b_i,b'_i\}$ for $i \in [n]$ and $\{c_j,d_j\}$ for $j \in [m]$, i.e., those due to nodes in $H$ with out-degree 2. Let $C^\alpha$ be the component in $G^\gamma$ containing $\alpha$ and $C^{\bar\alpha}$ the the other, and let the leaves be named so that $C^\alpha$ contains $p_\times$ and $C^{\bar\alpha}$ contains $q_\times$.

%Let the leaves be named so that $p_k$ is the leaf appearing on the RHS of the arc $a'=\arc(p'q'|o')$ in $H^\times$, i.e., $p_\times=o'$, in which case $q_\times$ does not appear in $\arc(e')$ and moreover A-node $q_\times$ does not appear in $C^\alpha$, and A-node $p_\times$ does not appear in $C^\alpha$. Therefore $G^\gamma$ will consist of two components: one before the cut (including $\gamma$) and one after, each of them containing an A-leaf whose A-edge label is an A-node lying in the {\em other} component: $q_\times=o'$ is an A-node in $C^{\bar\alpha}$, and $\gamma$ (the label of A-edge $\{c_mc_{m+1}\}$) is an A-node in $C^\alpha$.

Now, consider what happens when BUILD recurses on the triple and leaf sets corresponding to each of these components: in each case, BUILD will encounter a leaf set whose triples permit a linear ordering (similar to Table \ref{tbl:linord}), which therefore can be displayed in a (caterpillar) tree. In particular, in BUILD's recursive call for $[C^{\bar\alpha},V(C^{\bar\alpha})]$, $c_{m+1}$ will be an isolated node and the rest of the Ahograph will induce a DAG (directed acyclic graph) directed away from from $\gamma$; and in the recursive call for $[C^\alpha,V(C^\alpha)]$, $p_\times$ will be an isolated node and again the rest of the Ahograph will induce a DAG.
%therefore the Ahograph for that recursive call will consist of two components, an isolated A-node and a tree. 
In each of these two calls, therefore, BUILD's execution on its isolated-A-node-and-DAG pair will behave similarly ({\em despite the fact} that the portions of this Ahograph corresponding to clause gadgets may contain A-nodes and A-edges corresponding to all three witness paths, and the portions corresponding to variable gadgets may contain A-nodes and A-edges corresponding to both sides) to its execution on $\triples(P)$ for the acyclic $P$ in Lemmas \ref{lem:consistR} and \ref{lem:isentailed} (see Fig.\ \ref{fig:ahograph}), with each iteration isolating one additional node, thus constructing a caterpillar tree. These two caterpillars will become the root's child subtrees in the resulting tree displaying $R' \cup \{\gamma\alpha|\beta\}$ (see Fig.\ \ref{fig:cuttreeforced}).

Second, suppose there does not exist a path though the series of variable gadgets, i.e., from $b_1b'_1$ to $b_{n+1}b'_{n+1}$, meaning there does not exist a path through {\em some} variable gadget, i.e., from $b_ib'_i$ to $b_{i+1}b'_{i+1}$ for some $i \in [n]$. Then $A^\times$ must contain an arcs from both sides of $x_i$'s gadget, say $\arcs(z_i^\ell,z_{i^\ell+1}|z_i^{\ell+2},~ \bar z_i^{\ell'},\bar z_i^{\ell'+1}|\bar z_i^{\ell'+2}))$, where (because $A^\times$ is nondegenerate) either both or neither of $z_i^{\ell},\bar z_i^{\ell'}$ equals $b_i$. The absence of the two corresponding A-edges means that the Ahograph $G'$ will be disconnected. During BUILD's recursive calls for these two components, the whole process will play out similarly to how it did in the previous case (see Fig.\ \ref{fig:cuttreevar}).

%The third case is when the cut goes through some variable $x_i$'s gadget. Then $|A^\times|=2$ (if both sides of the $x_i$ gadget are including in $A'$). Since $A^\times$ is non-degenerate (i.e., either {\em both or neither} of these arcs are outgoing arcs of $b_ib'_i$), the Ahograph will be disconnected, and the whole process will play out similarly to the other two cases.


Third, suppose there does not exist a path through the series of clause gadgets, i.e., from $c_1d_1$ to $c_{m+1}d_{m+1}$. Since none of the forced arcs is missing, this means there does not exist a path through some clause gadget, i.e., from $c_jd_j$ to $c_{j+1}d_{j+1}$ for some $j \in [m]$. Then $A\times$ must contain an arc from each of the clause gadget's three witness paths (or similarly from {\em both} of them if the clause has only two literals).

%consider the case of the cut going through a clause gadget, in which case $A^\times$ consists of either two or  three arcs (since we have already dealt with the case of $|A^\times|=1$), each lying within one off that clause's witness paths. The case of two arcs is similar, so consider the most complex case of three.

Now there are several subcases to consider, but they all behave similarly. First, suppose $A^\times$ includes $c_jd_j$'s three outgoing arcs, each corresponding to a triple of the form $c_jd_j|\tilde x_{\hat w}^j$. Now, consider the effects of $c_jd_j$'s outgoing arcs' absence from $G^\gamma$: this means the three corresponding A-edges between $c_j$ and $d_j$ are absent, isolating $d_j$. Thus the initial input to BUILD consists of two components: isolated A-node $d_j$, and a DAG. In the recursive call for the DAG, the A-edge $\{c_{j-1},c_j\}$ labeled $d_j$ will no longer exist, and thus the corresponding Ahograph will consist of two components: one corresponding to the portion of the hypergraph from $\gamma$ through $C_{j-1}$'s gadget, and another corresponding top the portion from $C_j$'s gadget ({\em except for $d_j$}) though $c_{m+1}$. Now consider the recursive calls for these two components. Within the first component's recursive call, the three leaves of the form $\tilde y_{\hat w}^j$ will have been isolated, with the result that in subsequent calls the leaves of the form $\tilde x_{\hat w}^j$ will have been isolated, and so on, yielding a caterpillar tree. Similarly, $c_{m+1}$ will be isolated within the second recursive call, eventually yielding a second caterpillar tree. Then BUILD's final result will be a tree whose root's children are $d_j$ and a subtree whose two children are the roots of the two aforementioned caterpillar trees.

With three witness paths to cut, then there are  (up to isomorphism) either other subcases, which can all be verified through similar reasoning. The three cut arcs in any given case will be a subset from among the three $c_j \tilde y_{\hat w}^j$ nodes' outgoing arcs, the three $c_j \tilde x_{\hat w}^j$ nodes' outgoing arcs, and $c_jd_j$'s three outgoing arcs. Each cut arc outgoing from a $c_j \tilde y_{\hat w}^j$ node or a $c_j \tilde x_{\hat w}^j$ node will yield an isolated A-node. The initial Ahograph will therefore consist of either 1, 2, or 3 isolated A-nodes plus a DAG. Since it breaks ties arbitrarily, suppose BUILD always places isolated A-nodes as right children in the binary tree being constructed. Any time an A-node $\tilde y_{\hat w}^j$ is isolated (for some $w \in [3]$), in the following recursive call with $\tilde y_{\hat w}^j$ removed, $\tilde x_{\hat w}^j$ will be isolated. And in the recursive call following the isolation and removal of $\tilde x_{\hat w}^j$ for all $w=1,2,3$, $d_j$ will be isolated and removed.

At that point, the remaining Ahograph will consist of two DAGs $C^\alpha$ and $C^{\bar\alpha}$, where $C^\alpha$ contains $\alpha$ and $C^{\bar\alpha}$ does not. $C^{\bar\alpha}$ will also contain $c_j$ and any other A-nodes corresponding to $C_j$'s gadget that have not already been isolated and removed. In particular, $A^\times$ containing a cut arc outgoing from a $c_j \tilde x_{\hat w}^j$ node will mean $C^\alpha$ contains $y_{\hat w}^j$, and $A^\times$ containing a cut arc incoming to a $c_j \tilde x_{\hat w}^j$ will mean $C^\alpha$ contains $x_{\hat w}^j$ and $y_{\hat w}^j$.

The resulting binary tree (see Fig.\ \ref{fig:cuttreeclause}) will consist of a caterpillar region beginning at the root containing the 1-7 A-nodes isolated before the disconnection of the Ahograph into $C^\alpha$ and $C^{\bar\alpha}$, followed by a node whose two child subtrees are caterpillar trees resulting from $C^\alpha$ and $C^{\bar\alpha}$.
%
%The pattern is that the isolation of any A-node $y_{\hat w}^j$ will, in subsequent recursive calls, isolate the corresponding $x_{\hat w}^j$, the isolation of all three of which will in turn isolate $d_j$, after which the process continues as in the previous case, eventually yielding a tree (albeit a slightly differently shaped one).
\end{proof}
\else
\begin{lemma}\label{lem:treeexs}
Let $R'$ be consistent.
Suppose there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$, and that $A^\times$ is non-degenerate.
Then $R'$ does not entail $\alpha\beta|\gamma$.
\end{lemma}
\fi


The problematic situation is when exactly {\em one} of the two arcs is outgoing from $b_ib'_i$. In this case, their absence deletes only one of the Ahograph's two A-edges between the pair $\{b_i,b'_i\}$, which does {\em not} disconnect the graph, meaning BUILD will fail.

We have been arguing that if a consistent $R'$ entails $\alpha\beta|\gamma$ then $\arcs(R')$ must contain an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$. Now we refine this to a slightly weaker (yet strong enough) implication: if a consistent $R'$ entails $\alpha\beta|\gamma$, then a slightly different consistent $R^+$ will too, and an acyclic path must exist within $\arcs(R^+)$.
%(even if it does not within $\arcs(R')$).

%We handle this case via the following argument.

\ifproofapp
Taking the contrapositive, we rewrite the previous lemma as:
\begin{corollary}
Let $R'$ be consistent.
Suppose $R' \vdash \alpha\beta|\gamma$ and that $A'$ contains no path from $\alpha\beta$ to $c_{m+1}\gamma$.
Then $A^\times$ is degenerate.
%Then $|A^\times|=2$ and $A^\times$ contains exactly one arc $a_\times$ of the form $\arc(b_ib'_i|\tilde x_i^1)$.
\end{corollary}


\begin{lemma}\label{lem:degeneratecutpath}
Let $R'$ be consistent.
Suppose $R' \vdash \alpha\beta|\gamma$ and that $A'$ contains no path from $\alpha\beta$ to $c_{m+1}\gamma$.
%Assume $|A^\times|=2$ and $A^\times$ contains exactly one arc $a_\times$ of the form $\arc(b_ib'_i|\tilde x_i^1)$, and that $R'$ is consistent.
%
%Suppose a consistent $R'$ entails $\alpha\beta|\gamma$, $|A^\times|=2$, and $A^\times$ contains exactly one arc $a_\times$ of the form $\arc(b_ib'_i|\tilde x_i^1)$.
Then there exists an acyclic path $P \subseteq A' \cup \{a_\times\}$.
%
\end{lemma}
\begin{proof}
%
%In this scenario, the two members of $A^\times$ (which are absent from $A'$) are one of the two possible arcs with tail $b_ibi_i$ (say, $\arc(b_ib'_i|x_i^1)$), and an arc within the $x_i$ gadget's other side (whose tail is not $b_ib'_i$). 
%
The corollary implies that $A^\times$ is degenerate.
%$|A^\times|=2$ and $A^\times$ contains exactly one arc $a_\times$ of the form $\arc(b_ib'_i|\tilde x_i^1)$.

Let $H^+$ be the hypergraph obtained by adding $a_\times$ to $H^*$, which by construction contains a path (say, $P^+$) from $\alpha\beta$ to $c_{m+1}\gamma$.
%
Let $R^+ = \triples(A^+)$, where $A^+ = A' \cup \{a_\times\}$ is $H^+$'s arc set.

We claim that $R^+$ is consistent. We know that the point at which BUILD would potentially fail when executed on a subset of $R$ is in a call when an A-edge of the form $\{c_j,\tilde y_{\hat i_j}^j\}{:}c_{j+1}$ has been removed and the Ahograph is not disconnected, because $\tilde y_{\hat i_j}^j$ is not isolated (see Fig.\ \ref{fig:ahocycle}). But if this occurs when BUILD is executed on $R^+$, it would also have occurred when BUILD is executed on $R^*$ because $\tilde y_{\hat i_j}^j$ would still be connected in that scenario as well (see Fig.\ \ref{fig:ahodiscordvar}).
%
Therefore $A^+$, and in particular $P^+$, is acyclic.
%
%This proves in the variable gadget case as well that if a consistent $R'$ entails $\alpha\beta|\gamma$, then there exists an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$, concluding the proof.
%
%
%We want to show that if $\triples(A' \cup A^\times)$ entails $\alpha\beta|\gamma$, then $\triples(A' \cup A^\times) \cup \{b_ib'_i|x_i^1\}$ does too.
%
%We claim that $H^{*\prime}$ is acyclic.
\end{proof}
\else
\fi


%\vskip 2cm
%
%There must be some latest common predecessor node $u^0$ of $\{u_h : h \in [w]\}$ and some earliest common successor node $v^\omega$ of $\{v_h : h \in [w]\}$. Let the (possibly empty) sequence of {\em intermediate} nodes lying on the path strictly between $u^0$ and $u_h$ be $U_h = (u_h^1,...,u_h^{\ell_h})$, and the (possibly empty) sequence of {\em intermediate} nodes lying on the path strictly between $v_h$ and $v^\omega$ be $V_h = (v_h^{1},...,v_h^{\ell_h'})$. Observe that for each node in $U_h$, its incoming arc introduces one more leaf appearing in the corresponding triple's RHS, and so $U_h$ corresponds to $\ell_h$ such leaves, say, $p_h^1,...,p_h^{\ell_h}$. The first member of $V_h$ has no incoming arc, but for each subsequent member of $V_h$, the triple corresponding to its incoming arc similarly introduces one new leaf in its RHS; in addition, $V_h$'s first member's outgoing arc introduces one more new leaf. Thus $V_h$ corresponds to $\ell_h'$ leaves, say, $q_h^1,...,q_h^{\ell_h'}$.
%%
%%Similarly, for each node in $V_h$ after the first, its incoming arc introduces one more leaf in the triple's LHS, except for $v_1^1$, which introduces {\em two} more, because the leaf it shares in common with $u_w$ is also appearing on the LHS of a triple for the first time, due to $u_w$'s missing outgoing cross-arc, for a total of $\ell_h'+1$ such leaves, say, $q_h^0,...,q_h^{\ell_h'}$. 
%Let $p_0$ be the leaf introduced by node $u^0$, and $q^\omega$ the leaf introduced by node $v^\omega$.
%
%Then observe that $\{p^0\} \cup \bigcup_{h \in [w]} U_h$ can be put in a linear order, and hence $S(\alpha\beta,V,R')$ can be as well. Let $L_S$ be the set of all leaves appearing in tail nodes of paths between $\alpha\beta$ and members of $V_{\alpha\beta}$, i.e., the leaves appearing in nodes $V_{\alpha\beta} - \{U_h^{\ell_h} : h \in [w]\}$. Then can we construct a caterpillar tree $C_S$ having leaves $L_S$ (see root's left subtree in Fig.\ \ref{fig:nopathtree}, except ignoring the appearance of $\gamma$ for a moment).
%
%Similarly, observe that $\{q^\omega\} \cup \bigcup_{h \in [w]} V_h$ and hence $V_{c_{m+1}\gamma}$ can also be linearly ordered, and so if we define $L_P$ as the set of all leaves appearing in tail nodes of paths between members of $V_{c_{m+1}\gamma}$ and $c_{m+1}\gamma$,  i.e., the leaves appearing in nodes $V_{c_{m+1}\gamma} - \{c_{m+1}\gamma\}$, then we can also construct a caterpillar tree $C_P$ with leaves $L_P$ (see right subtree in Fig.\ \ref{fig:nopathtree}).
%
%Now create a root node, whose children are the roots of $C_P$ and $S_P$. This resulting tree contains every leaf but $\gamma$, and observe that it displays every triple of $R'$ except (obviously) $c_m c_{m+1} | \gamma$.
%
%Finally, we subdivide the tree's A-edge to $\alpha$ and add $\gamma$ as the second child of the tree's new inner node, with the result that the tree now displays $c_j c_{j+1} | \gamma$ and the rest of the triples of $R'$, as desired, yet also displays $\alpha \gamma | \beta$.
%
%\vskip 2cm


This implies:

\ifproofapp
\vskip .2cm
\noindent\textbf{Corollary \ref{cor:ispath}.}
If there is a consistent $R'$ entailing $\alpha\beta|\gamma$ then there exists an acyclic path $P$.
\else
\begin{corollary}[$\Rightarrow$]\label{cor:ispath}
If there is a consistent $R'$ entailing $\alpha\beta|\gamma$ then there exists an acyclic path $P$.
\end{corollary}
\fi



%Combining Lemmas \ref{lem:cycpath} and \ref{lem:treeexs}, we obtain:
%
%\begin{lemma}[$\Rightarrow$]\label{lem:notentailed}
%%If $R'$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$, then $A' = \arcs(R')$ contains the arcs of an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%%
%%Let $A' \subseteq A$. not
%Suppose there is no acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then for every subset $A' \subseteq A$, $R' = \triples(A')$ is  inconsistent or does not entail $\alpha\beta|\gamma$.
%%If $A' \subseteq A$ is {\em not} an acyclic arc set subsuming the set $P$ of arcs appearing in some path from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(A')$ is not a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
%\end{lemma}


%\textbf{start quotes:}
%
%%{\em Q: how do we know that a subset entailing $\alpha\beta|\gamma$ must necessarily correspond to a path?}
%
%\begin{lemma}[Bryant and Steel,  Prop. 9(1)]\label{lem:noabctrip} If $R$ is a closed set of rooted triples containing no triple with
%the leaves $\{a,b,c\}$ then $R \cup \{ab|e\}$, $R \cup \{ae|b\}$ and $R \cup \{be|a\}$ are all compatible.
%\end{lemma}
%
%{\em Q: can we get that entailment must follow a path by repeated (inductive) application of Lemma \ref{lem:noabctrip}?}
%
%\textbf{\em Q: is the consistency and/or the closure of a path in this construction actually somehow just obvious based on the construction?}
%\textbf{end quotes}





%\begin{lemma}[$\Leftarrow$]
%If there is a consistent triple set $R'$ entailing $\alpha\beta|\gamma$, then there is an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%%
%%Or: If there is no acyclic path from $ab$ to $ac$, then there is no consistent subset entailing $\alpha\beta|\gamma$.
%\end{lemma}
%\begin{proof}
%%First observe that the only triple in $R$ including $\alpha$ is $\alpha\beta | b_1$, and so any hypothetical subset $R' \subset R$ entailing $\alpha\beta|\gamma$ must necessarily include $\alpha\beta | b_1$.  But then observe that the only other triple in $R$ including $\beta$ is $\beta b_1 | b'_1$. By repeated application of similar arguments, we obtain that the hyperarcs corresponding to the triples of any such $R'$ must trace out a path from $\alpha\beta$ to $c_{m+1}\gamma$.
%
%Second, observe that if the path contained a cycle, then the triples corresponding to the hyperarcs appearing in that cycle would themselves be inconsistent, contradicting the consistency of $R'$.
%%the portion of the Ahograph induced by everything from the start of the caterpillar up to the cycle's back-arc would be a single component.
%%
%%That is, if we pluck off the sink nodes one by one, then plucking off the node just following the back-arc will reduce the number of components from 2 to 1, indicating that $R$ is inconsistent.
%%
%%Does it suffice to argue that for any path from $ab$ to $ac$, if the path is acyclic then it implies a consistent subset entailing $\alpha\beta|\gamma$?
%%
%%\textbf{That is, can we assume that entailment will imply a path?}
%\end{proof}




%\begin{lemma}[$\Rightarrow$]
%If there is an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$, then there is a satisfying truth assignment.
%\end{lemma}
%\begin{proof}
%We read off the truth assignment from the choices the path makes passing through the series of variable gadgets. Because the path is acyclic, we know that in the case of each clause gadget it passes through, the node within the variable gadget pointed to is on the side of the variable gadget that the path did {\em not} use. Since we set the variable's truth value based on which side we did not use, this implies that the corresponding literal in the clause gadget is true, thus satisfying the clause.
%\end{proof}

\ifproofapp
Combining the Corollary \ref{cor:consentails} and \ref{cor:ispath} with Theorem \ref{thm:apdh}, we conclude:
\vskip .2cm
\noindent\textbf{Theorem \ref{thm:entailnpc}.}
\entailprob\:is NP-Complete.
\vskip .2cm
\else
%This leads to the result:
Combining the Corollary \ref{cor:consentails} and \ref{cor:ispath} with Theorem \ref{thm:apdh}, we conclude:
\begin{theorem}\label{thm:entailnpc}
\entailprob\:is NP-Complete.
\end{theorem}
\fi



And because computing the closure reduces to deciding whether $R \vdash t$ for $O(|L|^3)$ triples $t$, we also have:

\ifproofapp
\vskip .2cm
\noindent\textbf{Corollary \ref{cor:closurenph}.}
\closureprob\:is NP-hard.
\else
\begin{corollary}\label{cor:closurenph}
\closureprob\:is NP-hard.
\end{corollary}
\fi


%Also:
%
%\begin{corollary}
%The complementary problem, of deciding whether a triple is entailed by {\em every} consistent subset of $R$ is co-NP-Complete.
%\end{corollary}
%\begin{proof}
%Solve the original problem for both negations of the triple.
%\end{proof}


==> rt-proofoutline-wabi.tex <==
% !TEX root = rootedtriples-arx.tex

\section{The Proof}

Clearly \entailprob\ is in NP: if we guess the subset $R' \subset R$, then we can verify both that $R'$ is consistent and that $R' \vdash t$ by executing Aho et al.\ \cite{aho1981inferring}'s polynomial-time BUILD algorithm on $R'$ \cite{bryant1995extension}. \minapdh\:is as well: guess the path, and check that it is acyclic.

Now we prove hardness, arguing that $R$ contains a consistent subset entailing $\alpha\beta|\gamma$ iff $H$ contains an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ iff $F$ admits a satisfying assignment $\mathbf{v}(\cdot)$, in two steps.

Due to lack of space, most of the proofs are deferred to the appendix.


%\textbf{3SAT} reduces to \apdh\:(which is therefore NP-Complete):


\subsection{Acyclic Path $\Leftrightarrow$ Satisfying Truth Assignment}

First we argue that acyclic paths correspond to satisfying truth assignments.

\begin{lemma}
There is an an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ iff $F$ admits a satisfying truth assignment $\mathbf{v}(\cdot)$.
%If there is a satisfying truth assignment, then there is an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$.
\end{lemma}

Thus we have proven:

\begin{theorem}\label{thm:apdh}
\apdh\:is NP-Complete.
\end{theorem}

Since an infeasible solution is defined to have infinite cost, an algorithm with {\em any} approximation factor would allow us to distinguish between positive and negative problem instances, which immediately implies:
\begin{corollary}
Approximating \minapdh\:to within {\em any} factor is NP-hard.
\end{corollary}

Even if we restrict ourselves to problem instances admitting feasible solutions, this ``promise problem" \cite{goldreich2006promise} special case is hard to approximate within any reasonable factor.

%More formally, we obtain the following hardness of approximation.

\begin{corollary}
%In the promise problem \cite{goldreich2006promise} special case in which an acyclic B-hyperpath is assumed to exist, approximating \minapdh\:to within factor $|V|^{1-\epsilon}$ for any $\epsilon>0$ is NP-hard.
\minapdhprom\:is NP-hard to approximate to within factor $|V|^{1-\epsilon}$ for all $\epsilon>0$.
\end{corollary}
\begin{proof}
Let $\epsilon \in (0,1/4)$. Let $I = \langle H,u,v \rangle$ be an instance \minapdhprom. For this proof only, let $n=|V(H)|$.
We extend $H$ to a new hypergraph $H'$ by adding polynomially many dummy arcs forming an acyclic $u{\to}v$ path of length $n^{\lceil1+1/\epsilon\rceil}$, yielding a hypergraph $H'$ with $n' = n+n^{\lceil1+1/\epsilon\rceil}-1$ nodes and a new problem instance $I' = \langle H',u,v \rangle$, which is also by construction a valid problem instance of \minapdhprom. If $H$ has a path ($I$ is a positive instance), then $H'$ (like $H$) has one of some length $OPT^+ \le n-1$; if not ($I$ is a negative instance), then $H'$'s only path has length $OPT^- = n^{\lceil1+1/\epsilon\rceil}$.

Now, suppose there were a $|V|^{1-\epsilon}$-approximation algorithm.

Running it on the $I'$ resulting from a negative $I$ will yield a path of length at least $LB^- = OPT^- = n \cdot n^{\lceil1/\epsilon\rceil}$.

Running it on the $I'$ resulting from a positive $I$ will yield a path of length of at most
\begin{align*}
UB^+ &= n'^{1-\epsilon}\cdot (n-1)\\
&= (n+n^{\lceil1+1/\epsilon\rceil}-1)^{1-\epsilon}\cdot (n-1)\\
& < (n-1) \cdot n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)} + (n-1)^{2-\epsilon}\\
&< n \cdot n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)},
\end{align*}
where the last inequality follows from the fact that $(n-1)^{2-\epsilon} < n^{\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)}$ for $\epsilon<1/4$.

Because $\lceil1+1/\epsilon\rceil\cdot(1-\epsilon) = 1+\lceil1/\epsilon\rceil - \epsilon - \epsilon \lceil 1/\epsilon \rceil < \lceil 1/\epsilon \rceil$, it follows that $UB^+ < LB^-$.

%$\lceil1/\epsilon\rceil$ vs $\lceil1+1/\epsilon\rceil\cdot(1-\epsilon)$
%
%$\lceil1/\epsilon\rceil$ vs $\lceil1/\epsilon\rceil\cdot(1-\epsilon) + (1-\epsilon)$
%
%$\lceil1/\epsilon\rceil$ vs $\lceil1/\epsilon\rceil - \lceil1/\epsilon\rceil\cdot\epsilon + (1-\epsilon)$
%
%0 vs $- \lceil1/\epsilon\rceil\cdot\epsilon + (1-\epsilon)$
%
%$\lceil1/\epsilon\rceil\cdot\epsilon > (1-\epsilon)$

Thus by comparing the length $ALG$ of the path in $H'$ found by the hypothetical algorithm to $UB^+$ and $LB^-$, we can decide whether $I$ was positive or negative.
%
%Then any algorithm providing an $f(|V|)$-approximation would allow us to distinguish (for $|V|$ sufficiently large) between instances $H'$ with optimal solution cost $<f(|V|)\cdot|V|$ and those with optimal solution cost $\ge f(|V|) \cdot |V|^2$, thus deciding whether $H$ had a path.
\end{proof}




Second, to extend the reduction to \entailprob, we argue that $H$ is a faithful representation of $R$ in the sense that acyclic paths from $\alpha\beta$ to $c_{m+1}\gamma$ (or acyclic supersets of such paths) correspond to consistent subsets entailing $\alpha\beta|\gamma$, and vice versa.


\subsection{Consistent Entailing Subset $\Leftarrow$ Acyclic Path}

We prove this direction via two lemmas, proving that the set of triples corresponding to an acyclic path are consistent and entail $\alpha\beta|\gamma$, respectively.



\begin{lemma}\label{lem:consistR}
If there is an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(P)$ is consistent.
\end{lemma}
\begin{proof}
To prove $R'$ consistent, we 
%reinterpret the procedure we carried out in the proof of Lemma \ref{lem:isentailed} as implicitly executing 
step through the execution of Aho et al.\ \cite{aho1981inferring}'s BUILD algorithm running on input $R'$, tracking the state of the resulting Ahograph (see Fig.\ \ref{fig:ahograph}) and the tree being constructed (see Fig.\ \ref{fig:pathtree}) as they progress over time.
%Specifically, each application of dyadic inference rule (\ref{eq:2b}), as we step through $P$ in reverse order, can be interpreted as one iteration (or recursive call) of BUILD.
Each iteration can be interpreted as one application of dyadic inference rule (\ref{eq:2b}), as we step through $P$ in reverse order.

%, of stepping through $P$ in reverse, repeatedly applying dyadic inference rule (\ref{eq:2b})
%
%again step through $P$ in reverse, implicitly executing Aho et al.\ \cite{aho1981inferring}'s BUILD algorithm on input $R'$, picturing the state of the resulting Ahograph (see Fig.\ \ref{fig:ahograph}) and the tree being constructed (see Fig.\ \ref{fig:pathtree}) along the way. 

Observe that in Ahograph $[R', L(R')]$ (see Fig.\ \ref{fig:ahograph}), $\gamma$ will be an isolated A-node, since $R$ contains no triples with $\gamma$ on their LHSs,
%Just as dyadic inference rule (\ref{eq:2b}) carried us through to $\alpha\beta | \sigma$, 
%Observe also that by definition of $R'$, the A-nodes $L(R') - \{\gamma\}$ are connected in one component of Ahograph $[R', L(R')]$, 
and that the A-edge $\{c_m, c_{m+1}\}$ in $[R', L(R')]$ due to $P$'s last arc (representing $c_m c_{m+1} | \gamma$) is labeled (only) with $\gamma$. Isolated A-node $\gamma$ is removed for BUILD's second iteration, in which we recurse on the remaining A-nodes. The A-edge $\{c_m, c_{m+1}\}$ will therefore no longer appear in that iteration's Ahograph, $[R', L(R') - \{\gamma\}]$, rendering $c_{m+1}$ an isolated A-node.

We claim that this pattern will continue to obtain the rest of the way back to the start of $P$, with a new A-node becoming isolated  by the start of each iteration, causing an A-edge to be removed, and hence isolating another A-node for the succeeding iteration.
%
More precisely, number the iterations in reverse, counting downward from $\ell=|P|$, where iteration $\ell$ is the first iteration executed (the one in which A-node $o_\ell=\gamma$ is observed isolated and removed for the second iteration, thus also deleting the A-edge $\{p_\ell,q_\ell\}=\{c_m,c_{m+1}\}$).



Let $H_P$ be the subhypergraph of $H$ induced by the nodes $\{\text{t}(e) \cup \text{h}(e) : {e \in P}\}$, and recall that nodes in $H$ correspond to unordered pairs of A-nodes, and thus to potential A-edges in the Ahograph.

Because $P$ is a path (and because there are no arcs between two witness paths or between the two sides of a variable gadget), each non-sink node in $H_P$ will have out-degree 1 ($c_{m+1}\gamma$ has out-degree 0). Therefore $[R', L(R')]$ will have exactly $\ell$ A-edges, each with one label.
%
%%of $H$ induced by $P$ has out-degree at most one. Therefore no A-edge in the Ahograph has more than one label. Note that $\alpha$ and $\beta$ will not be labels of any A-edge.
%
Because $P$ is acyclic, each node in $H_P$ except $\alpha\beta$ (which has in-degree 0) will have in-degree 1. Therefore no label will appear on multiple A-edges in $[R', L(R')]$.
%
Thus there is a bijection between Ahograph $[R', L(R')]$'s $\ell$ A-edges and the labels appearing on them.

Node $\alpha\beta$ contains two leaves, and each arc in $P$ introduces one additional leaf, for a total of $\ell+2$ leaves in $L(R')$, and hence $\ell+2$ A-nodes in the Ahograph.

Note also that the first arc in $P$ adds label $b_1$ to A-edge $\{\alpha,\beta\}$ in the Ahograph, and that each subsequent arc adds a label to an A-edge incident to the preceding A-edge, and so all $\ell$ of the Ahograph's A-edges lie within a single component. Since isolated A-node $\gamma$ is one of the $\ell+2$ A-nodes, this means that the other component has exactly $\ell+1$ A-nodes, and is therefore a tree.

%To see this, suppose $c_j \tilde x_i^j{\to}\{\tilde x_i^j \tilde y_i^j, c_j \tilde y_i^j\}$ is a back-arc in $P$.
%
%there are no other A-edges in the Ahograph beyond those listed here.
%%
%Note also that no label appears on more than one A-edge. Therefore there is a one-to-one correspondence between the Ahograph's $\ell$ A-edge labels and $P$'s arcs. Every A-node appears (once) as a label, except for $\alpha$ and $\beta$. Thus the Ahograph has $\ell+2$ A-nodes, and its second component is a tree.

Now, we prove by induction that at the start of each iteration $k$ from $\ell$ down to $1$, the Ahograph consists of two components: some isolated A-node $o_k$ and a tree. We have already verified the base case: $o_\ell$ is isolated at the start, in iteration $\ell$, and the $\ell+1$ remaining nodes form a tree. Assume the claim is true for each iteration from $\ell$ down through some iteration $k$.

%If this is not true for every iteration, let $k$ be the first iteration at the start of which $o_k$ is not isolated. Now, we know that at the start the previous iteration (iteration $k+1$), $o_{k+1}$ (which is the right-hand side of triple $u_{k+1}|o_{k+1}$, where $o_k \in u_{k+1}$) was found to be isolated, and therefore was removed from the iteration-$k$ Ahograph. What does it mean if we find at the start of iteration $k$ that $o_k$ is still not isolated?
%
%The deletion of $o_{k+1}$ meant the removal of label $o_{k+1}$ from from the Ahograph of A-edge $u_{k+1}$, which contains $o_k$. If A-edge $u_{k+1}$ nonetheless remains in the Ahograph, this means that it still has some label.


%\begin{align}
%\nonumber(&\gamma{:}\{c_{m+1},c_m\},\\
%&c_{m+1}{:}\{\tilde y_{i_{w_m}}^m,c_m\},~\tilde y_{i_{w_m}}^m{:}\{\tilde x_{i_{w_m}}^m,c_m\},~\tilde x_{i_{w_m}}^m{:}\{d_m,c_m\},~ d_m{:}\{c_m,c_{m-1}\},~ c_m{:}\{\tilde y_{i_{w_{m-1}}}^{m-1},c_{m-1}\},\\
%& ...,\\
%&c_2{:}\{\tilde y_{i_{w_1}}^1,c_1\},~\tilde y_{i_{w_1}}^1{:}\{\tilde x_{i_{w_1}}^1,c_1\},~\tilde x_{i_{w_1}}^1{:}\{d_1,c_1\},~ d_1{:}\{c_1,b'_{n+1}\},~c_1{:}\{b'_{n+1},b_{n+1}\},~b'_{n+1}{:}\{b_{n+1},\tilde y_n^m\},\label{eq:clauses}\\
%&b_{n+1}{:}\{\tilde y_n^m,\tilde x_n^m\},~\tilde y_n^m{:}\{\tilde x_n^m,\tilde y_n^{m-1}\},~ ...,~\tilde x_{n}^2 {:}\{\tilde y_{n}^1,\tilde x_{n}^1\},~\tilde y_n^1{:}\{\tilde x_n^1,b'_n\},~\tilde x_n^1{:}\{b'_n,b_n\},~b'_n{:}\{b_n,\tilde y_{n-1}^m\},\label{eq:varn}\\
%\nonumber&b_n{:}\{\tilde y_{n-1}^{m},\tilde x_{n-1}^{m}\},~\tilde y_{n-1}^m{:}\{\tilde x_{n-1}^m,\tilde y_{n-1}^{m-1}\},~ ...,~\tilde x_{n-1}^2{:}\{\tilde y_{n-1}^1,\tilde x_{n-1}^1\},~\tilde y_{n-1}^1{:}\{\tilde x_{n-1}^1,b'_{n-1}\},~\tilde x_{n-1}^1{:}\{b'_{n-1},b_{n-1}\},\\ 
%&b'_{n-1}{:}\{b_{n-1},\tilde y_{n-2}^m\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&b_2{:}\{\tilde y_1^m,\tilde x_1^m\},~\tilde y_m^1{:}\{\tilde x_1^m,\tilde y_1^{m-1}\},~ ...,~\tilde x_1^2{:}\{\tilde y_1^1,\tilde x_1^1\},~\tilde y_1^1{:}\{\tilde x_1^1,b'_1\},~\tilde x_1^1{:}\{b'_1,b_1\},~
%b'_1{:}\{b_1,\beta\},\label{eq:var1}\\ 
%\nonumber&b_1{:}\{\beta,\alpha\})
%\end{align}



 
%Given such a path $P$, we construct the corresponding $R'=f(P)$. By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths as follows:
%\begin{eqnarray*}
%P &=& (\alpha\beta,a_1,\beta b_1, a_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (b_{n+1}b'_{n+1},a_3,b'_{n+1}c_1,a_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (c_{m+1}\gamma)
%\end{eqnarray*}
%Given such an arc set $P$, we construct the corresponding $R'=f(P)$. 
%We choose $A' = P$, and set $R' = \triples(A')$, which is consistent by Lemma \ref{lem:consistR}.
By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths:
\begin{align*}
P &~=~ (a_1,a_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (a_3,a_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m},
\end{align*}
where $P_{x_i}$ is one of the two length-$2m{+}2$ subpaths passing through $x_i$'s gadget (from $b_ib'_i$ to $b_{i+1}b'_{i+1}$), $P_{C_j}$ is one of the three length-4 subpaths traversing one of the $C_j$ gadget's three witness paths (from $c_jd_j$ to $c_jc_{j+1}$) {\em plus the succeeding arc with tail $c_jc_{j+1}$}, and $a_1,...,a_4$ are shorthand names for the other four connecting arcs.





For each $C_j$, let $\hat i_j$ denote the index $i$ of the variable $x_i$ appearing in the witness path of $C_j$ (through literal appearance $\tilde x_{\hat i_j}^j$) that $P$ traverses.

Now, consider the {\em reverse linear ordering} shown in Table \ref{tbl:linord} of the A-node-labeled A-edges of Ahograph $[R', L(R')]$, with each subsequence of A-node-labeled A-edges tagged to indicate the corresponding subpath of $P$ (compare to Figs.\ \ref{fig:ahograph} and \ref{fig:overview}, and in particular compare each ($P_{C_j}$) to Fig.\ \ref{fig:clause} and each ($P_{x_i}$) to Fig.\ \ref{fig:var}). %, for an acyclic path $P$: 
%(which takes the positive sides of variable gadgets $x_n,\tilde x_{n-1},\tilde x_1$):

%\begin{table}[t]
%\centering
%\begin{alignat}{7}
%(~&\gamma{:}\{c_m,c_{m+1}\}, ~~&&c_{m+1}{:}\{c_m,\tilde y_{\hat i_m}^m\}, ~~&&\tilde y_{\hat i_m}^m{:}\{c_m,\tilde x_{\hat i_m}^m\}, ~~&&\tilde x_{\hat i_m}^m{:}\{c_m,d_m\},\label{eq:clausem}\tag{$P_{C_m}$}\\
%&d_m{:}\{c_{m-1},c_m\}, ~~&&c_m{:}\{c_{m-1},\tilde y_{\hat i_{m-1}}^{m-1}\}, ~~&&\tilde y_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},\tilde x_{\hat i_{m-1}}^{m-1}\}, ~~&&\tilde x_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},d_{m-1}\},\label{eq:clausemm1}\tag{$P_{C_{m-1}}$}\\
%& ...,\nonumber\\
%&d_2{:}\{c_1,c_2\}, ~~&&c_2{:}\{c_1,\tilde y_{\hat i_1}^1\}, ~~&&\tilde y_{\hat i_1}^1{:}\{c_1,\tilde x_{\hat i_1}^1\}, ~~&&\tilde x_{\hat i_1}^1{:}\{c_1,d_1\},\label{eq:clause1}\tag{$P_{C_1}$}\\
%&d_1{:}\{b'_{n+1},c_1\}, ~~&&c_1{:}\{b_{n+1},b'_{n+1}\},\label{eq:var2clause}\tag{$a_3,a_4$}\\
%&b'_{n+1}{:}\{\tilde y_n^m,b_{n+1}\}, ~~&&b_{n+1}{:}\{\tilde x_n^m,\tilde y_n^m\}, ~~&&\tilde y_n^m{:}\{\tilde y_n^{m-1},\tilde x_n^m\}, ~ \quad..., ~~&&\tilde x_{n}^2 {:}\{\tilde x_{n}^1,\tilde y_{n}^1\},\nonumber\\
%&\quad\tilde y_n^1{:}\{b'_n,\tilde x_n^1\}, ~~&&\tilde x_n^1{:}\{b_n,b'_n\},\label{eq:varn}\tag{$P_{x_n}$}\\
%&b'_n{:}\{\tilde y_{n-1}^m,b_n\}, ~~&&b_n{:}\{\tilde x_{n-1}^{m},\tilde y_{n-1}^{m}\}, ~~&&\tilde y_{n-1}^m{:}\{\tilde y_{n-1}^{m-1},\tilde x_{n-1}^m\},~~ ..., ~~&&\tilde x_{n-1}^2{:}\{\tilde x_{n-1}^1,\tilde y_{n-1}^1\},\nonumber\\
%&\quad\tilde y_{n-1}^1{:}\{b'_{n-1},\tilde x_{n-1}^1\}, ~~&&\tilde x_{n-1}^1{:}\{b_{n-1},b'_{n-1}\},\label{eq:varnm1}\tag{$P_{x_{n-1}}$}\\
%&...,\nonumber\\
%&b'_{2}{:}\{\tilde y_{1}^m,b_{2}\}, ~~&&b_{2}{:}\{\tilde x_{1}^m,\tilde y_{1}^m\}, ~~&&\tilde y_1^m{:}\{\tilde y_1^{m-1},\tilde x_1^m\},~ \quad..., ~~&&\tilde x_1^2{:}\{\tilde x_1^1,\tilde y_1^1\},\nonumber\\
%&\tilde y_1^1{:}\{b'_1,\tilde x_1^1\}, ~~&&\tilde x_1^1{:}\{b_1,b'_1\},\label{eq:var1}\tag{$P_{x_1}$}\\
%&b'_1{:}\{\beta,b_1\}, ~~&&b_1{:}\{\alpha,\beta\})\tag{$a_3,a_4$~}
%\end{alignat}
%\vskip -.5cm
%\caption{Reverse linear ordering.}
%\label{tbl:linord}
%\end{table}



\begin{table}[t]
\caption{Reverse linear ordering of the A-edges corresponding to arcs in path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.}
\vskip -.45cm
\centering
\begin{alignat}{7}
(~&\{c_m,c_{m+1}\}:\gamma, ~~&&\{c_m,\tilde y_{\hat i_m}^m\}:c_{m+1}, ~~&&\{c_m,\tilde x_{\hat i_m}^m\}:\tilde y_{\hat i_m}^m, ~~&&\{c_m,d_m\}:\tilde x_{\hat i_m}^m,\label{eq:clausem}\tag{$P_{C_m}$}\\
&\{c_{m-1},c_m\}:d_m, ~~&&\{c_{m-1},\tilde y_{\hat i_{m-1}}^{m-1}\}:c_m, ~~&&\{c_{m-1},\tilde x_{\hat i_{m-1}}^{m-1}\}:\tilde y_{\hat i_{m-1}}^{m-1}, ~~&&\{c_{m-1},d_{m-1}\}:\tilde x_{\hat i_{m-1}}^{m-1},\label{eq:clausemm1}\tag{$P_{C_{m-1}}$}\\
& ...,\nonumber\\
&\{c_1,c_2\}:d_2, ~~&&\{c_1,\tilde y_{\hat i_1}^1\}:c_2, ~~&&\{c_1,\tilde x_{\hat i_1}^1\}:\tilde y_{\hat i_1}^1, ~~&&\{c_1,d_1\}:\tilde x_{\hat i_1}^1,\label{eq:clause1}\tag{$P_{C_1}$}\\
&\{b'_{n+1},c_1\}:d_1, ~~&&\{b_{n+1},b'_{n+1}\}:c_1,\label{eq:var2clause}\tag{$a_3,a_4$}\\
&\{\tilde y_n^m,b_{n+1}\}:b'_{n+1}, ~~&&\{\tilde x_n^m,\tilde y_n^m\}:b_{n+1}, ~~&&\{\tilde y_n^{m-1},\tilde x_n^m\}:\tilde y_n^m, ~ \quad..., ~~&&\{\tilde x_{n}^1,\tilde y_{n}^1\}:\tilde x_{n}^2,\nonumber\\
&\quad\{b'_n,\tilde x_n^1\}:\tilde y_n^1, ~~&&\{b_n,b'_n\}:\tilde x_n^1,\label{eq:varn}\tag{$P_{x_n}$}\\
&\{\tilde y_{n-1}^m,b_n\}:b'_n, ~~&&\{\tilde x_{n-1}^{m}:b_n,\tilde y_{n-1}^{m}\}, ~~&&\{\tilde y_{n-1}^{m-1},\tilde x_{n-1}^m\}:\tilde y_{n-1}^m,~~ ..., ~~&&\{\tilde x_{n-1}^1,\tilde y_{n-1}^1\}:\tilde x_{n-1}^2,\nonumber\\
&\quad\{b'_{n-1},\tilde x_{n-1}^1\}:\tilde y_{n-1}^1, ~~&&\{b_{n-1},b'_{n-1}\}:\tilde x_{n-1}^1,\label{eq:varnm1}\tag{$P_{x_{n-1}}$}\\
&...,\nonumber\\
&\{\tilde y_{1}^m,b_{2}\}:b'_{2}, ~~&&\{\tilde x_{1}^m,\tilde y_{1}^m\}:b_{2}, ~~&&\{\tilde y_1^{m-1}:\tilde y_1^m,\tilde x_1^m\},~ \quad..., ~~&&\{\tilde x_1^1,\tilde y_1^1\}:\tilde x_1^2,\nonumber\\
&\{b'_1,\tilde x_1^1\}:\tilde y_1^1, ~~&&\{b_1,b'_1\}:\tilde x_1^1,\label{eq:var1}\tag{$P_{x_1}$}\\
&\{\beta,b_1\}:b'_1, ~~&&\{\alpha,\beta\}:b_1~)\tag{$a_3,a_4$}
\end{alignat}
\vskip -.25cm
\label{tbl:linord}
\end{table}




%\begin{alignat}{3}
%(&\gamma{:}\{c_m,c_{m+1}\}, ~~&&c_{m+1}{:}\{c_m,\tilde y_{\hat i_m}^m\}, ~~\tilde y_{\hat i_m}^m{:}\{c_m,\tilde x_{\hat i_m}^m\}, ~~\tilde x_{\hat i_m}^m{:}\{c_m,d_m\},\label{eq:clausem}\\
%&d_m{:}\{c_m,c_{m-1}\}, ~~&&c_m{:}\{c_{m-1},\tilde y_{\hat i_{m-1}}^{m-1}\}, ~~\tilde y_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},\tilde x_{\hat i_{m-1}}^{m-1}\}, ~~\tilde x_{\hat i_{m-1}}^{m-1}{:}\{c_{m-1},d_{m-1}\},\label{eq:clausemm1}\\
%& ...,\label{eq:clauses}\\
%&d_2{:}\{c_2,c_2\}, ~~c_2{:}\{c_1,\tilde y_{\hat i_1}^1\}, ~~\tilde y_{\hat i_1}^1{:}\{c_1,\tilde x_{\hat i_1}^1\}, ~~\tilde x_{\hat i_1}^1{:}\{c_1,d_1\},\label{eq:clause1}\\
%&d_1{:}\{c_1,b'_{n+1}\}, ~~c_1{:}\{b'_{n+1},b_{n+1}\},\label{eq:var2clause}\\
%&b'_{n+1}{:}\{b_{n+1},\tilde y_n^m\}, ~~b_{n+1}{:}\{\tilde y_n^m,\tilde x_n^m\}, ~~\tilde y_n^m{:}\{\tilde x_n^m,\tilde y_n^{m-1}\}, ~~ ..., ~~\tilde x_{n}^2 {:}\{\tilde y_{n}^1,\tilde x_{n}^1\}, ~~\tilde y_n^1{:}\{\tilde x_n^1,b'_n\}, ~~\tilde x_n^1{:}\{b'_n,b_n\},\label{eq:varn}\\
%&b'_n{:}\{b_n,\tilde y_{n-1}^m\}, ~~b_n{:}\{\tilde y_{n-1}^{m},\tilde x_{n-1}^{m}\}, ~~\tilde y_{n-1}^m{:}\{\tilde x_{n-1}^m,\tilde y_{n-1}^{m-1}\},~~ ..., ~~\tilde x_{n-1}^2{:}\{\tilde y_{n-1}^1,\tilde x_{n-1}^1\}, ~~\tilde y_{n-1}^1{:}\{\tilde x_{n-1}^1,b'_{n-1}\},\\
%&\quad\tilde x_{n-1}^1{:}\{b'_{n-1},b_{n-1}\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&b'_{2}{:}\{b_{2},\tilde y_{1}^m\}, ~~b_{2}{:}\{\tilde y_{1}^m,\tilde x_{1}^m\}, ~~\tilde y_1^m{:}\{\tilde x_1^m,\tilde y_1^{m-1}\},~~ ..., ~~\tilde x_1^2{:}\{\tilde y_1^1,\tilde x_1^1\}, ~~\tilde y_1^1{:}\{\tilde x_1^1,b'_1\}, ~~\tilde x_1^1{:}\{b'_1,b_1\},\label{eq:var1}\\
%&b'_1{:}\{b_1,\beta\}, ~~b_1{:}\{\beta,\alpha\})
%\end{alignat}



%\begin{align}
%\nonumber(&\gamma{:}\{c_{m+1},c_m\},~ c_{m+1}{:}\{y_m^{i_{w_m}},c_m\},~ y_m^{i_{w_m}}{:}\{x_m^{i_{w_m}},c_m\},~ x_m^{i_{w_m}}{:}\{d_m,c_m\},~ d_m{:}\{c_m,c_{m-1}\},~ c_m{:}\{y_{m-1}^{i_{w_{m-1}}},c_{m-1}\},\\
%& ...,\\
%&c_2{:}\{y_1^{i_{w_1}},c_1\},~ y_1^{i_{w_1}}{:}\{x_1^{i_{w_1}},c_1\},~x_1^{i_{w_1}}{:}\{d_1,c_1\},~ d_1{:}\{c_1,b'_{n+1}\},~c_1{:}\{b'_{n+1},b_{n+1}\},~b'_{n+1}{:}\{b_{n+1},y_n^m\},\label{eq:clauses}\\
%&b_{n+1}{:}\{y_n^m,x_n^m\},~ y_n^m{:}\{x_n^m,y_n^{m-1}\},~ ...,~ x_{n}^2 {:}\{y_{n}^1,x_{n}^1\},~ y_n^1{:}\{x_n^1,b'_n\},~x_n^1{:}\{b'_n,b_n\},~b'_n{:}\{b_n,y_{n-1}^m\},\label{eq:varn}\\
%\nonumber&b_n{:}\{y_{n-1}^{m},x_{n-1}^{m}\},~ y_{n-1}^m{:}\{x_{n-1}^m,y_{n-1}^{m-1}\},~ ...,~ x_{n-1}^2{:}\{y_{n-1}^1,x_{n-1}^1\},~ y_{n-1}^1{:}\{x_{n-1}^1,b'_{n-1}\},~ x_{n-1}^1{:}\{b'_{n-1},b_{n-1}\},\\ 
%&b'_{n-1}{:}\{b_{n-1},y_{n-2}^m\},\label{eq:varnm1}\\ 
%&...,\label{eq:othervars}\\
%&b_2{:}\{y_1^m,x_1^m\},~ y_m^1{:}\{x_1^m,y_1^{m-1}\},~ ...,~ x_1^2{:}\{y_1^1,x_1^1\},~ y_1^1{:}\{x_1^1,b'_1\},~ x_1^1{:}\{b'_1,b_1\},~
%b'_1{:}\{b_1,\beta\},\label{eq:var1}\\ 
%\nonumber&b_1{:}\{\beta,\alpha\})
%\end{align}

%Here (\ref{eq:clausem}) corresponds to the portion of $P$ passing through clause $C_m$'s gadget, (\ref{eq:clausemm1}) to the portion passing through $C_{m-1}$'s gadget, (\ref{eq:clauses}) to the portion passing through the gadgets for clauses $C_{m-2},...,C_2$, (\ref{eq:clause1}) through clause $C_1$, (\ref{eq:var2clause}) to the connection from clause $C_1$'s gadget back to variable $x_n$'s gadget (\ref{eq:varn}) through variable $x_n$, (\ref{eq:varnm1}) through $x_{n-1}$, (\ref{eq:othervars}) through variables $x_{n-2},...,x_2$, and (\ref{eq:var1}) through $x_1$'s gadget.

%Observe that for each {\em label$:$edge} entry $k$ for $k < \ell$, that entry's label $o_{k}$ is one of the two A-nodes occurring in entry $k+1$'s (i.e., the preceding entry's) A-edge, say $p_{k+1}$, and crucially, $p_{k+1}$ has no further appearances in the list beyond entry $k$.

Observe the relationship between each {\em A-edge$:$label} entry in the ordering and its predecessor: for each entry $k-1$ for $k \le \ell$, its label $o_{k-1}$ is one of the two A-nodes occurring in entry $k$'s (i.e., the preceding entry's) A-edge, say $p_k$, and crucially, $p_k$ has no further appearances in the list past entry $k-1$. That is, {\em at the start of iteration $k$, $p_k$ is a leaf in the Ahograph}.

Therefore iteration $k$'s removal of the then-isolated A-node $o_k$ and of the (only) label from A-edge $\{p_k,p_k'\}$ disconnects the component that had contained that A-edge in two, thus isolating $p_k = o_{k-1}$ in time for iteration $k-1$. 
%Thus A-edge $\{p_k,p_k'\}$'s removal in iteration $k$ means that $p_k = o_{k-1}$ will be an isolated A-node at the start of iteration $k-1$. 
The remainder of that same component is of course also a tree, thus proving the inductive claim for iteration $k-1$.

%Note also that one of A-edge $\{p_k,p_k'\}$'s two endpoints (say, $p_k$) the {\em label} of the succeeding entry $o_{k-1}{:}\{p_{k-1},p_{k-1}'\}$ (i.e., $p_k=o_{k-1}$) and does not appear as an {\em endpoint} in any subsequent A-edge in the ordering. That is, at the start of the iteration $k$, $p_k$ is a leaf in the Ahograph. Therefore the removal of A-edge $\{p_k,p_k'\}$ means that $p_k = o_{k-1}$ is an isolated A-node at the start of iteration $k-1$. The remainder of that component within the Ahograph is of course still a tree, thus proving the inductive claim.

Since the BUILD algorithm running on $R'$ therefore never encounters a connected Ahograph, it follows \cite{bryant1995extension} that $R'$ is consistent.
%
%%Therefore each removal of the next {\em label$:$edge} entry causes the isolation of the A-node appearing as the subsequent entry's label.
%
%%The initial Ahograph consists of two components, one of which is an isolated A-node ($\gamma$). It has $\ell$ A-edges, corresponding to $P$'s $\ell$ arcs. Every A-node appears (once) as a label, except for $\alpha$ and $\beta$. Thus the Ahograph has $\ell+2$ A-nodes, and its second component is a tree. Therefore each deletion of an A-edge from that second component increases the number of components by one.
%
%Finally, observe that in each iteration, the A-edge deleted is incident to a leaf, thus rendering it an isolated A-node.
%
%
%\textbf{HERE}
%
%
%If $o_k$ nonetheless is still not isolated, that means that triple $p_kq_k | o_k$ was not removed in the previous iteration. 
%
%in each iteration a new A-node $u_k$ becomes isolated
%
%encountering a new isolated A-node in each iteration, 
%
%
%as the process implicitly constructs a caterpillar tree (see Fig.\ \ref{fig:caterpillar}), thus implying that $R'$ is consistent.
\end{proof}







\begin{lemma}\label{lem:isentailed}
%Let $A' \subseteq A$. 
If there is an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(P)$ entails $\alpha\beta|\gamma$.
%there exists a subset $A' \subseteq A$ for which $R' = \triples(A')$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
\end{lemma}
\begin{proof}
%Given such a path $P$, we construct the corresponding $R'=f(P)$. By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths as follows:
%\begin{eqnarray*}
%P &=& (\alpha\beta,a_1,\beta b_1, a_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (b_{n+1}b'_{n+1},a_3,b'_{n+1}c_1,a_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (c_{m+1}\gamma)
%\end{eqnarray*}
%Given such an arc set $P$, we construct the corresponding $R'=f(P)$. 
%We choose $A' = P$, and set $R' = \triples(A')$, which is consistent by Lemma \ref{lem:consistR}.
%By inspection of $H$, observe that $P$ can be decomposed into a sequence of subpaths:
%\begin{eqnarray*}
%P &=& (a_1,a_2) \circ P_{x_1} \circ P_{x_2} \circ \cdots \circ P_{x_n} \circ  (a_3,a_4) \circ P_{C_1} \circ P_{C_2} \circ \cdots \circ P_{C_m} \circ (a_5)
%\end{eqnarray*}
%where $P_{x_i}$ is one of the two length-$2m{+}2$ subpaths passing through $x_i$'s gadget (from $b_ib'_i$ to $b_{i+1}b'_{i+1}$), $P_{C_j}$ is one of the three length-4 subpaths passing through $C_j$'s gadget (from $c_jd_j$ to $c_jc_{j+1}$) and including the succeeding connecting arc, and $a_1,...,a_5$ are placeholder names for the other five connecting arcs. 
%More precisely, the paths $P_{x_i}$ and $P_{C_j}$ are all ``half-open'' paths, meaning that they start with a node and end with an arc: $P_{x_i}$ starting with $b_ib'_i$ and ending with one of the two arcs {\em preceding} $b_{i+1}b'_{i+1}$, and $P_{C_j}$ starting with $c_jd_j$ and edging with the (unique) arc {\em preceding} $c_{j+1}d_{j+1}$.
%where $P_{x_i}$ is the path passing through $x_i$'s variable gadget, $P_{C_j}$ is the path passing through $C_j$'s clause gadget, and $a_1,...,a_4$ are placeholder names for the four corresponding connecting arcs. More precisely, the paths $P_{x_i}$ and $P_{C_j}$ are all ``half-open'' paths, meaning that they start with a node and end with an arc: $P_{x_i}$ starting with $b_ib'_i$ and ending with one of the two arcs {\em preceding} $b_{i+1}b'_{i+1}$, and $P_{C_j}$ starting with $c_jd_j$ and edging with the (unique) arc {\em preceding} $c_{j+1}d_{j+1}$.

%Recalling that each 1-2-hyperarc represents a rooted triple in $R$, we add to $R'$ the triple corresponding to each arc appearing in $P$, i.e., $R' = \{r(a) : a \in P\}$, where $r(e)$ denotes the triple represented by $$.
%
Let $\ell=|P|$, and for each $k \in [\ell]$, let $a_k = u_k{\to}\{v_k,v_k'\}$ denote the $k$th arc in $P$, with $u_k = p_kq_k$ and $\{v_k,v_k'\} = \{p_ko_k, q_ko_k \}$ (for some leaves $p_k,q_k,o_k$), representing triple $p_k q_k | o_k = u_k | o_k$. The names $v_\ell,v_\ell'$ can be assigned so that $v_\ell = c_{m+1}\gamma$ (and $v_\ell'$ is $a_\ell$'s non-destination sink node $c_m \gamma$), but we can also simply represent $a_\ell$ as $u_\ell|o_\ell = c_mc_{m+1} | \gamma$.
%so hyperarc $a_\ell = u_\ell{\to}\{v_\ell, v_\ell'\}$, representing triple $u_\ell|o_\ell = p_\ellq_\ell | o_\ell = c_mc_{m+1} | \gamma$. 
Similarly, for each $k \in [2,...,\ell]$, we can assign the names $v_{k-1},v_{k-1}'$ so that $v_{k-1}=u_k$, i.e., $\text{t}(a_k) = u_k = v_{k-1} \in \text{h}(a_{k-1})$,
%and so hyperarc $a_{k-1} = u_{k-1}{\to}\{u_k, v_{k-1}'\}$, representing triple $p_{k-1}q_{k-1} | o_{k-1} = u_{k-1}|o_{k-1}$.
and we can also simply represent $a_{k-1}$ as $u_{k-1}|o_{k-1}$.

Now consider arcs $a_{\ell-1}$ and $a_\ell$, and observe that their representations as $u_{\ell-1}|o_{\ell-1}$ and $u_\ell|o_\ell$ (respectively) are 
%$a_{\ell-1} = u_{\ell-1}{\to}\{u_\ell, v_{\ell-1}'\}$ and $a_\ell = u_\ell{\to}\{v_\ell, v_\ell'\}$, representing triples $u_{\ell-1}|o_{\ell-1}$ and $u_\ell|o_\ell$, respectively, and observe that this pair of triples is 
of exactly the form that dyadic inference rule (\ref{eq:2b}) applies to: via that inference rule, we can derive the triple $u_{\ell-1}|o_\ell$, which have the form $c_m \tilde y_i^m | \gamma$ (for some $i$). % or $c_j \bar y_i^m | \gamma$.

%, where the names $v_k,v_k'$ are assigned so that $v_k$ is $u_k$'s successor on $P$, i.e., $v_k = u_{k+1}$ (except when $k=\ell$, in which case $v_k=c_{m+1}\gamma$), and therefore, $u_k=v_{k-1}$, i.e., $u_k = \text{t}(a_k) \in \text{h}(a_{k-1}) = \{v_{k-1},v_{k-1}'\}$
%
%That is, $\text{t}(a_k) = p_kq_k$, and $o_{k-1} \in \{p_k, q_k\}$ and $|\{p_k, q_k\} \cap \{p_{k-1}, q_{k-1}\}|=1$, and so $a_k$ represents $p_k q_k | o_k$. Then observe that by applying the second dyadic inference rule (recall Def.\ \ref{def:2ord}) to the triples represented by the path's last two arcs (i.e., $p_{\ell-1} q_{\ell-1} | o_{\ell-1}$ and $p_\ell q_\ell | o_\ell$), we can infer $p_{\ell-1} q_{\ell-1} | o_\ell$. 

Similarly, by applying this inference rule to the triple represented $P$'s third-to-last arc (i.e., $u_{\ell-2} | o_{\ell-2}$) and the derived triple  $u_{\ell-1} | o_\ell$, we can derive $u_{\ell-2} | o_\ell$. Via a total of $\ell-1$ such applications of dyadic inference rule (\ref{eq:2b}) (each corresponding to one BUILD iteration), we can derive $u_1 | o_\ell = p_1 q_1 | o_\ell$ = $\alpha \beta | \gamma$.
%
%Second, by Lemma \ref{lem:consistR} proved below, $R'$ is indeed consistent.
\end{proof}

Thus we have:
\begin{corollary}[$\Leftarrow$]\label{cor:consentails}
%Let $A' \subseteq A$. 
If there is an acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(P)$ is consistent and entails $\alpha\beta|\gamma$.
%there exists a subset $A' \subseteq A$ for which $R' = \triples(A')$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
\end{corollary}



%mpj
%\newpage


%mpj
\begin{figure}%[t!]
\centering
	\begin{subfigure}{\textwidth}
\centering
%\input{triples-fig-var-leaves}
%\captionsetup{justification=centering}
%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%\input{triples-fig-tree}
\makebox[1\textwidth][c]{ %\hskip -2cm
\includegraphics[width=1\textwidth]{rt-fig-ahopath-arx.pdf}
}
%\vskip .05cm
%\vskip -.05cm
\caption{The initial Ahograph $[R',L(R')]$ constructed based on an underlying {\em acyclic} path $P$. Because $P$ is acyclic, the node  $\tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j$ pointed to by each $C_j$'s witness node $c_j \tilde x_{\hat i_j}^j$ is a {\em sink node in $H$}, and thus A-nodes $\tilde y_i^j$ and $\tilde x_i^j$ are {\em leaves in the Ahograph}. As a result, at each BUILD iteration, the Ahograph has two components, a tree and an isolated node.
%, distinct from the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets.% (as occurs in Fig.\ \ref{fig:ahocycle}).
%
%Because $P$ is acyclic, 
%, where $P$ is an acyclic path in the hypergraph from $\alpha\beta$ to $c_{m+1}\gamma$,
%%(specifically, the red path shown in Fig.\ \ref{fig:overview}), 
%and $R'=\triples(P)$. 
%%Here $x_2$ is false and $x_1,x_3,x_4$ are true, and the witness literals for clauses $C_1,C_2,C_3,C_4$ are $\bar x_n, \bar x_1, \bar x_n, \bar x_1$, respectively. 
%%If $P$ had contained a cycle involving some clause $C_j$, then $C_j$'s $x$ and $p$ nodes in the resulting Ahograph would have 
%Let $\tilde x_i^j \tilde y_i^j$ be the variable gadget node pointed to by the $C_j$ clause's witness node. Then, because $P$ is acyclic, A-nodes $\tilde x_i^j$ and $\tilde y_i^j$ are both leaves {\em in the Ahograph}, rather than appearing in the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets (as occurs in Fig.\ \ref{fig:ahocycle}).
\label{fig:ahograph}
}
%\end{figure}
%\begin{figure}[t!]
\end{subfigure}
\vskip .35cm
\centering
	\begin{subfigure}{\textwidth}
\centering
%\captionsetup{justification=centering}
%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%\input{triples-fig-tree}
\includegraphics[width=.75\textwidth]{rt-fig-ahocycle-arx.pdf}
%\vskip .05cm
%\vskip -.05cm
\caption{A fragment of the Ahograph resulting from the cause of a cycle in $P$, viz., a back-arc in which some clause $C_j$'s witness node $c_j \tilde x_{\hat i_j}^j$ points to a {\em non-sink} node $\tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j$ that lies earlier in the path $P$ (specifically, within $x_{\hat i_j}$'s gadget), and thus A-nodes $\tilde y_{\hat i_j}^j$ and $\tilde x_{\hat i_j}^j$ are {\em non-leaves} in the Ahograph. This yields the triangle $c_j-\tilde y_{\hat i_j}^j - \tilde x_{\hat i_j}^j$. After the BUILD iteration in which A-node $c_{j+1}$ and A-edge $\{c_j, \tilde y_{\hat i_j}^j\}$ are removed, $\tilde y_{\hat i_j}^j$ will still {\em not} be isolated, and hence the Ahograph will at that point consist of a single component, indicating $R'$ is inconsistent.
%Ahograph $[R',L(R')]$, where $P$ is an acyclic path in the hypergraph from $\alpha\beta$ to $c_{m+1}\gamma$ (specifically, the red path shown in Fig.\ \ref{fig:overview}), and $R'=\triples(\arcs(P))$. Here $x_2$ is false and $x_1,x_3,x_4$ are true, and the witness literals are $\tilde x_n, \tilde x_1, \tilde x_n, \tilde x_1$ for clauses $C_1,C_2,C_3,C_4$, respectively. 
%%If $P$ had contained a cycle involving some clause $C_j$, then $C_j$'s $x$ and $p$ A-nodes in the resulting Ahograph would have  
%Because $P$ is acyclic, each clause $C_j$'s $x$ and $p$ A-nodes are leaves {\em in the Ahograph}, rather than being A-nodes in the portion of the Ahograph corresponding to $P$'s traversal of the variable gadgets. 
\label{fig:ahocycle}
}
\end{subfigure}
\caption{The Ahograph $[R',L(R')]$ is constructed when Aho et al.'s BUILD algorithm is executed on the triples $R' = \triples(P)$ corresponding to the path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$. The existence of any cycle within $P$ involving some clause $C_j$'s witness node $c_j \tilde x_{\hat i_j}^j$ pointing to $\tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j$ (i.e., arc $c_j \tilde x_{\hat i_j}^j \to \{c_j \tilde y_{\hat i_j}^j, \tilde x_{\hat i_j}^j \tilde y_{\hat i_j}^j\}$) will be reflected in the locations in the Ahograph of A-nodes $\tilde y_{\hat i_j}^j$ and $\tilde x_{\hat i_j}^j$.}
\end{figure}






\begin{figure}
\centering
\includegraphics[width=1\textwidth]{rt-fig-ahoincompgr-arx.pdf}
\vskip -,25cm
\caption{The Ahograph $[R',L(R')]$ for $R'=\triples(A')$, where $A'$ is a maximal acyclic subset of $A$ and the three variable gadgets shown (for $x_1,x_2,x_n$) are each maximal in the sense that both sides are included and the three clause gadgets shown (for $C_1,C_2,C_m$) are each maximal in the sense that all three witness paths are included. (Hence all the appearances within clauses $C_1,C_2,C_m$ must be of variables $x_3,...,x_{n-1}$.) If there is no disconnection between either $b_2$ and $b'_n$ or $c_2$ and $c_m$, then the Ahograph is connected and $R'$ is inconsistent.\label{fig:ahoincompgr}
}
%none of $x_1,x_2,x_n$ appear in any of $C_1,C_2,C_m$.)}
%\end{figure}
%
%
\vskip .2cm
%\begin{figure}[t!]
\centering
\includegraphics[width=.95\textwidth]{rt-fig-ahodiscordvar-arx.pdf}
\vskip -,05cm
\caption{A fragment of the Ahograph corresponding to a variable $x_i$'s gadget (see Fig.\ \ref{fig:var}) if its only two arcs missing from $A'$ are $\arcs(b_ib'_i|x_i^1, ~\bar y_i^m|b_{i+1}|b'_{i+1})$, with the A-edge we consider hypothetically adding in the proof of Lemma \ref{lem:degeneratecutpath} shown dashed.\label{fig:ahodiscordvar}
}
\end{figure}
























\subsection{Consistent Entailing Subset $\Rightarrow$ Acyclic Path}

Now we argue for the reverse direction, % (or rather, its contrapositive), %, that satisfying truth assignments correspond to acyclic paths, 
proving through a series of lemmas that if there is no acyclic $\alpha\beta{-}c_{m+1}\gamma$ path, then there will be no consistent triple subset entailed $\alpha\beta|\gamma$.
%via a proof that will depend on two subsequent lemmas proved below.


\begin{lemma}\label{lem:cycpath}
%If $R'$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$, then $A' = \arcs(R')$ contains the arcs of an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%
%Let $A' \subseteq A$. not
Let $A' \subseteq A$. Suppose there exists a {\em cyclic} path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then $R' = \triples(A')$ is inconsistent.
%Suppose there is no acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then for every subset $A' \subseteq A$, $R' = \triples(A')$ is  inconsistent or does not entail $\alpha\beta|\gamma$.
%If $A' \subseteq A$ is {\em not} an acyclic arc set subsuming the set $P$ of arcs appearing in some path from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(A')$ is not a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
\end{lemma}
\begin{proof}
Intuitively, it can be seen that any cycle in $H$ corresponds to a vicious (inconsistent) cycle of rooted triples. In particular (see Fig.\ \ref{fig:ahocycle}), any clause $C_j$'s component whose witness node points to a variable gadget node already visited on the path (causing a cycle in $H$) will induce a triangle {\em in the Ahograph}, resulting in a single-component Ahograph in the BUILD iteration following the deletion of isolated node $c_{j+1}$ (if no single-component Ahograph has yet been encountered in an earlier iteration), since at that point A-node $\tilde y_{\hat i_j}^j$ will have failed to become isolated.
\end{proof}

Most of the remainder of this subsection will be dedicated to showing {\em constructively} that if $A'$ contains no path from $\alpha\beta$ to $c_{m+1}\gamma$ at all, cyclic or otherwise, then $R'$ does not entail $\alpha\beta|\gamma$. We do so by showing that in the case of such a (consistent) $R'$, there exist trees displaying $R' \cup \{\alpha\beta|\gamma\}$. Therefore assume w.l.o.g.\ that $R'$ is consistent and maximal in the sense that adding any other triple of $R$ to it would either make $R'$ inconsistent or would introduce an $\alpha\beta{-}c_{m+1}\gamma$ path in $A'=\arcs(R')$.
%The remainder of the proof in this subsection will be to show (constructively) that if there exists a consistent $R'$ entailing $\alpha\beta|\gamma$ then there exists a path from $\alpha\beta$ to $c_{m+1}\gamma$.
%$A'$ subsumes no path from $\alpha\beta$ to $c_{m+1}\gamma$ at all, cyclic or otherwise, then $R'$ will not entail $\alpha\beta|\gamma$. Therefore assume w.l.o.g.\ that $R'$ is consistent.
%
%We begin by defining some notation.

Observe that the missing arcs $A^\times = A - A'$ can be thought of as the (source side to sink side) cross arcs of a cut separating source $\alpha\beta$ and sink $c_{m+1}\gamma$.
%
In the following argument we will refer to hypergraph $H^\gamma = (V \cup \{ \gamma\alpha\}, A' \cup \arc(\gamma\alpha|\beta))$ and its corresponding Ahograph $G^\gamma$.

% mpj
%Let $S(\alpha \beta,V,A') \subseteq V$ (written $V_{\alpha\beta}$) be the set of all nodes reachable from $\alpha \beta$ via the nodes $V$ and the arcs $A'$, and let $P(c_{m+1}\gamma,V,A') \subseteq V$ (written $V_{c_{m+1}\gamma}$) be the set of all nodes that $c_{m+1}\gamma$ is reachable {\em from} via $V$ and $A'$, and set $V' = V_{\alpha\beta} \cup V_{c_{m+1}\gamma}$ Then by assumption $V_{\alpha\beta}$ and $V_{c_{m+1}\gamma}$ are disjoint. That is, the subhypergraph of $(V,A')$ induced by $V'$ has two components.
%
%Let $V_{\alpha \beta}^* \subseteq V_{\alpha\beta}$ be the maximal elements of $V_{\alpha\beta} $ in the sense that every $u \in V_{\alpha \beta}^*$ is reachable from $\alpha\beta$ but no other node $v \in V_{\alpha\beta}$'s reachability {\em depends on} $u$. That is, $S(\alpha \beta,V-\{u\},A') = S(\alpha \beta,V,A') - \{u\}$. Similarly, let $V_{c_{m+1}\gamma}^* \subseteq V_{c_{m+1}\gamma}$ be the minimal elements of $V_{c_{m+1}\gamma}$ in the sense that for any $v \in V_{c_{m+1}\gamma}^*$, there is no other node $u \in V_{c_{m+1}\gamma}$ dependent on $v$, i.e., $P(c_{m+1}\gamma,V-\{v\},A') = P(c_{m+1}\gamma,V,A')-\{v\}$.


%\begin{lemma}[$\Rightarrow$]\label{lem:notentailed}
%%If $R'$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$, then $A' = \arcs(R')$ contains the arcs of an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%%
%%Let $A' \subseteq A$. not
%Suppose there is no acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then for every subset $A' \subseteq A$, $R' = \triples(A')$ is  inconsistent or does not entail $\alpha\beta|\gamma$.
%%If $A' \subseteq A$ is {\em not} an acyclic arc set subsuming the set $P$ of arcs appearing in some path from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(A')$ is not a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
%\end{lemma}
%\begin{proof}
%%Given such a subset $R'$, we construct the corresponding $P=f^{-1}(R')$.
%%Let $A' \subseteq A$ be an arbitrary subset of $A$, and set $R' = \triples(A')$.
%
%%First, suppose there {\em is} a path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then $P$ must be cyclic, and thus $\triples(P) \subseteq R'$ will be inconsistent. 
%
%%Second, suppose there is no path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$ having $P \subseteq A$, cyclic or otherwise. If $A'$ is cyclic then $R' = \triples(A')$ will again be inconsistent, so assume $A'$ is acyclic. Now we will show constructively that in this case, $R'$ does not entail $\alpha\beta|\gamma$.
%
%
%
%%By Lemma \ref{lem:uvpairs} proved below, we can assume w.l.o.g.\ that there are at most 3 $u^*$s and at most 3 $v^*$s, which together yield either 1, 2, or 3 pairs $(u_h,v_h)$, with each pair connected by an arc $a_h \in  A - A'$.
%
%%Then by Lemma \ref{lem:treeexs} proved below, we can build a tree displaying $\triples(A') \cup \{\alpha\gamma | \beta\}$ (see Fig.\ \ref{fig:nopathtree}). This shows that $R' \cup \{\alpha\gamma | \beta\}$ is consistent, and thus that $R'$ does not entail $\alpha\beta | \gamma$.
%%
%%
%%
%%
%%
%%
%%%\textbf{but then there's a tree satisfying $R'$ and not $\alpha\beta|\gamma$}
%%
%%
%%First observe that the only triple in $R$ including $\alpha$ or $\beta$ is $\alpha\beta | b_1$, and so any hypothetical subset $R' \subset R$ pseud o-entailing $\alpha\beta|\gamma$ must necessarily include $\alpha\beta | b_1$.  But then observe that the only other triple in $R$ including $\alpha$ or $\beta$ is $\beta b_1 | b'_1$, so it must be included. Next, observe that the only other triples in $R$ including $\beta$ or $b_1$ are $b_1b'_1 | x_i^1$ and $b_1b'_1 | \bar x_i^1$, so at least one of them must be included. We claim that by repeated application of arguments of this kind, we obtain that the arcs corresponding to the triples of any such $R'$ must trace out a path from $\alpha\beta$ to $c_{m+1}\gamma$.
%%
%%Second, observe that if $P$ contained a cycle, then the triples corresponding to the hyperarcs appearing in that cycle would themselves be inconsistent, contradicting the consistency of $R'$.
%\end{proof}





% mpj
%\begin{lemma}\label{lem:uvpairs}
%Suppose $A' \subseteq A$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. Let $V_{\alpha \beta}^* \subseteq V_{\alpha\beta}$ and $V_{c_{m+1}\gamma}^* \subseteq V_{c_{m+1}\gamma}$ be defined as above.
%%in the proof of Lemma \ref{lem:notentailed} above. 
%Then $|V_{\alpha \beta}^*| = |V_{c_{m+1}\gamma}^*| \in [3]$, 
%%and there is bijection between $V_{\alpha \beta}^*$ and $V_{c_{m+1}\gamma}^*$, with each pair corresponding to a unique A-edge in $A-A'$.
%%By Lemma \ref{lem:uvpairs} proved below, we can assume w.l.o.g.\ that there are at most 3 $u^*$s and at most 3 $v^*$s, 
%which (w.l.o.g.) together yield $w \in [3]$ ordered pairs $\{(u_h,v_h) : h \in [w]\}$ and a set of arcs $A^\times$, where each pair is connected by a unique arc $a_h \in A^\times \subseteq A - A'$.
%\end{lemma}
%\begin{proof}
%First, we claim we can assume w.l.o.g.\ that for no $u^* \in V_{\alpha\beta}^*$ will the path to it from $\alpha\beta$ cross a back-arc, i.e., a subpath taking an arc of the form $c_j \tilde x_i^j{\to}\{c_j\tilde y_i^j, \tilde x_i^j\tilde y_i^j\}$ to reach a node $\tilde x_i^j\tilde y_i^j$ {\em for the first time} (see Fig.\ \ref{fig:clause}). Preceding $c_j \tilde x_i^j$, the path would have had to visit $c_jd_j$, and if after crossing the back-arc the path is going (via additional A-edges from $A$ we add later) to eventually reach $c_{m+1}\gamma$, then it would have to visit $c_jd_j$ again, making it cyclic and $R'$ inconsistent.
%
%Second, we claim we can assume w.l.o.g.\ that for no $v^* \in V_{c_{m+1}\gamma}^*$ will its path to $c_{m+1}\gamma$ will contain back-arcs.
%%, i.e., a subpath taking an arc of the form $c_j \tilde x_i^j{\to}\{c_j\tilde y_i^j, \tilde x_i^j\tilde y_i^j\}$ to $\tilde x_i^j\tilde y_i^j$. 
%To see this, consider (see Fig.\ \ref{fig:clause}) what node $v^*$ could possibly benefit (in terms of reaching $c_{m+1}\gamma$) from such a path. If $v^*=c_jd_j$ (or any of its immediate predecessors) for some $j$, then the path from $v^*$ to $c_{m+1}\gamma$ would again have to eventually return to $c_jd_j$ again, making the path cyclic. If $v^*= c_j \tilde x_i^j$ for some $j,i$, then it is not impossible per se for there to be an acyclic path from it to $c_{m+1}\gamma$ traversing a back-arc. The only possible arc that could be used for reaching $c_j \tilde x_i^j$, however, is the one from $c_jd_j$, in which case once again any resulting path from $\alpha\beta$ to $c_{m+1}\gamma$ would be cyclic.
%
%Now, how far are the elements of $V_{\alpha\beta}$ away from the elements of $V_{c_{m+1}\gamma}$? That is, how many arcs from $A$ would have to be added to $A'$ in order to reach a node $v \in  V_{c_{m+1}\gamma}$ from a node $u^* \in V_{\alpha \beta}^*$ or to reach a node $v^* \in  V_{c_{m+1}\gamma}^*$ from a node $u \in V_{\alpha \beta}$?
%
%Since our eventual goal is to show that $R' = \triples(A')$ does {\em not} entail $\alpha \beta | \gamma$, we assume w.l.o.g.\ the most difficult case, i.e., that any $v^* \in V_{c_{m+1}\gamma}^*$ is only one hop away from some $u \in V_{\alpha \beta}$, via some arc $a \in A - A'$, the addition of which to $A'$ would complete a path from $\alpha\beta$ to $c_{m+1}\gamma$. Conversely, we can assume w.l.o.g.\ that for every $u^* \in V_{\alpha \beta}^*$ there exists an A-edge $a \in A-A'$ that would connect it to some $v \in V_{c_{m+1}\gamma}$. If $A^\times$ is the set of all arcs $a$ playing this role for some $u^*$ and/or $v^*$, then observe that $(V_{\alpha \beta}^*,V_{c_{m+1}\gamma}^*)$ is a {\em directed cut} separating $\alpha\beta$ from $c_{m+1}\gamma$ in the hypergraph $H^\times = (V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^*, A' \cup A^\times)$, and $A^\times$ consists of the (forward) {\em cross-arcs} of that cut.
%
%Now, how many arcs could there be in $A^\times$? By inspection of the hypergraph construction, it can be seen that $|A^\times|$ will be either 2, 3, or 1, depending (respectively) on whether the cut occurs within a variable gadget, within a clause gadget, or elsewhere.\footnote{Note that the cross-arcs can connect members of $V_{\alpha\beta}^*$ to $V_{c_{m+1}\gamma}$ and members of $V_{\alpha\beta}$ to $V_{c_{m+1}\gamma}^*$, not just members of $V_{\alpha\beta}^*$ to $V_{c_{m+1}\gamma}^*$. Consider, for example, a cut through variable $x_i$'s gadget cutting arcs $b_ib'_i{\to}\{b'_ix_i^1,b_ix_i^1\}$ and $\bar y_i^mb_{i+1}{\to}\{b_{i+1}b'_{i+1},\bar y_i^mb'_{i+1}\}$ but with all other arcs of $x_i$'s gadget present in $A'$. In this case, $b_ib'_i \in V_{\alpha\beta} - V_{\alpha\beta}^*$ and $b_{i+1}b'_{i+1} \in V_{c_{m+1}\gamma} - V_{c_{m+1}\gamma}^*$.}
%%Note also that due to hypergraph construction there will be a bijection between $u^*$s and $v^*$s. To see this, recall that the only arcs in which both heads are non-sink nodes are those in which a clause gadget's witness node $c_j \tilde x_i^j$ points back to a variable gadget node $\tilde x_i^j \tilde y_i^j$. But we have seen that no $u^*$'s path will contain a back-arc. Therefore if $A^\times$ contains an A-edge of the form $c_j \tilde x_i^j{\to}\{c_j \tilde y_i^j, \tilde x_i^j \tilde y_i^j\}$, it must be due to $u^*=c_j \tilde x_i^j$ and $v^*=c_j \tilde y_i^j$.
%\end{proof}
%







\begin{figure}
\centering
\makebox[1\textwidth][c]{ %\hskip -3.75cm
%    \captionsetup{width=.9\linewidth}%
   \centering
\ifwabi
   \begin{subfigure}[t]{.14\linewidth}
\clipbox{6.15cm .15cm 5.65cm .5cm}{      \includegraphics[height=.535\textheight,angle=33]{rt-fig-pathtree-arx.pdf}  }
\else
   \begin{subfigure}[t]{.12\linewidth}
\clipbox{6.25cm .15cm 5.75cm .5cm}{      \includegraphics[height=.535\textheight,angle=31.75]{rt-fig-pathtree-arx.pdf}  }
\fi
\caption{$A'$ is an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$.
%The caterpillar tree determined by the triples corresponding to $P$, which thence satisfies $\alpha\beta|\gamma$.
\label{fig:pathtree}
}
  \end{subfigure}
\ifwabi
\hskip .3cm
  \begin{subfigure}[t]{.26\linewidth}
\else
\hskip .35cm
  \begin{subfigure}[t]{.28\linewidth}
\fi
    \centering
    %\captionsetup{width=1.1\linewidth}%
\ifwabi
\clipbox{2.5cm .15cm 1.5cm 1.4cm}{      \includegraphics[height=.21\textheight,angle=35.6]{rt-fig-cuttreeforced-arx.pdf} }
\else
\clipbox{2.6cm .15cm 1.6cm 1.45cm}{      \includegraphics[height=.22\textheight,angle=33.6]{rt-fig-cuttreeforced-arx.pdf} }
\fi
\caption{$A^\times$ contains some forced arc $a_\times$.
%A tree consistent with $A'$, i.e., displaying all of $R'=\triples(A')$, but {\em not} displaying $\alpha \beta | \gamma$.
%The tree that can be constructed displaying all triples in $R'=\triples(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. 
%The root's left subtree contains all leaves appearing in A-nodes before the ``cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
\label{fig:cuttreeforced}
}
  \end{subfigure}
\ifwabi
\hskip .35cm
\else
\hskip .35cm
\fi  \begin{subfigure}[t]{.28\linewidth}
    \centering
    %\captionsetup{width=1.1\linewidth}%
\ifwabi
\clipbox{5.45cm .15cm 4.45cm 1.4cm}{      \includegraphics[height=.455\textheight,angle=34.6]{rt-fig-cuttreevar-arx.pdf} }
\else
\clipbox{5.75cm .15cm 4.7cm 1.25cm}{      \includegraphics[height=.47\textheight,angle=33.6]{rt-fig-cuttreevar-arx.pdf} }
\fi
\caption{$A^\times$ contains $\arcs($ $z_i^\ell z_i^{\ell+1}|z_i^{\ell+2}, ~ \bar z_i^{ell'} \bar z_i^{\ell'+1}|\bar z_i^{\ell'+2})$, where either both or neither of $z_i^\ell,\bar z_i^{\ell'}$ equal $b_i$.
%A tree consistent with $A'$, i.e., displaying all of $R'=\triples(A')$, but {\em not} displaying $\alpha \beta | \gamma$.
%The tree that can be constructed displaying all triples in $R'=\triples(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. 
%The root's left subtree contains all leaves appearing in A-nodes before the ``cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
\label{fig:cuttreevar}
}
  \end{subfigure}
\ifwabi
\hskip .45cm
  \begin{subfigure}[t]{.3\linewidth}
\else
\hskip .35cm
  \begin{subfigure}[t]{.28\linewidth}
\fi
    \centering
    %\captionsetup{width=1.1\linewidth}%
%\hskip -.35cm
\ifwabi
\clipbox{7.05cm 1.05cm 5.85cm .55cm}{   \includegraphics[height=.7\textheight,angle=32.75]{rt-fig-cuttreeclause-arx.pdf} }
\else
\clipbox{7.5cm 1.15cm 6.25cm .5cm}{   \includegraphics[height=.73\textheight,angle=31.75]{rt-fig-cuttreeclause-arx.pdf} }
\fi
%\adjincludegraphics[height=5cm,clip,bb = 0 10 612 100,angle=30]{rt-fig-cuttreeclause-arx.pdf}
%    \fbox{\tikz{
%            \clip[use as bounding box] (0,0)++(.01\textwidth,.01\textwidth) rectangle ++(.45\textwidth,.45\textwidth);
%\draw (0,0) node[inner sep=0pt,name=micrograph]{\includegraphics[angle=10,width=1.6\textwidth]{rt-fig-cuttreeclause-arx.pdf}};
%\draw[ultra thick, white] (micrograph.south west)++(0.05*0.5\textwidth,0.05*0.5\textwidth)--++(0.5*0.25806\textwidth,     0)node[above,white,midway]{}};}
%}
\caption{$A^\times$ contains three arcs lying with clause $C_j$'s gadget.
%A tree consistent with $A'$, i.e., displaying all of $R'=\triples(A')$, but {\em not} displaying $\alpha \beta | \gamma$.
%The tree that can be constructed displaying all triples in $R'=\triples(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. 
%The root's left subtree contains all leaves appearing in A-nodes before the ``cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
\label{fig:cuttreeclause}
}
  \end{subfigure}
 }
%
%
%%\captionsetup{justification=centering}
%%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%%\input{triples-fig-tree}
%\includegraphics[height=.5\textheight]{triples-fig-pathtree.pdf}
%%\vskip .05cm
%\vskip -.1cm
%\caption{The caterpillar tree resulting from the triples corresponding to $P$, which thence satisfies $\alpha\beta|\gamma$.}
%\label{fig:caterpillar}
%\vskip .1cm
%\centering
%%\captionsetup{justification=centering}
%%\includegraphics[width=\linewidth, clip=true, trim={0cm 10cm 3cm 5cm}]{triplescaterpillar.jpg}
%%\input{triples-fig-tree}
%\includegraphics[height=.5\textheight]{triples-fig-nopathtree.pdf}
%%\vskip .05cm
%%\vskip -.05cm
\caption{Trees resulting from triples corresponding to an acyclic arc set $A' \subseteq A$ in $H$ that (a) do or (b,c,d) do not contain a path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$, for different cases of $A'$ and $A^\times = A-A'$. Leaves corresponding to isolated A-nodes in the tree's Ahograph are shown with thick dashed borders, and the leaves corresponding to A-nodes that {\em become} isolated when those isolated A-nodes are removed are shown with thin dashed borders. In (b,c,d), leaves within the two major subtrees are also shown thus, with respect to those subtrees' Ahographs.
%The tree that can be constructed displaying all triples in $R'=\triples(A')$ but {\em not} $\alpha \beta | \gamma$, if $A'$ is acyclic and there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$. The root's left subtree contains all leaves appearing in A-nodes before the ``directed cut'' (plus $\gamma$), and its right subtree contains all leaves appearing after the ``cut'' (except $\gamma$).
}
\end{figure}



%Let $H^* = (V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^*, A')$, $H^\gamma = (V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^* \cup \{ \gamma\alpha\}, A' \cup \arc(\gamma\alpha|\beta))$, $H^\times = (V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^*, A' \cup A^\times)$, and $H^{\times\gamma} = (V_{\alpha \beta}^* \cup V_{c_{m+1}\gamma}^* \cup \{ \gamma\alpha\}, A' \cup A^\times \cup \arc(\gamma\alpha|\beta))$, and let $G^*$, $G^\gamma$, $G^\times$, and $G^{\times\gamma}$ be the corresponding Ahographs (respectively).
%
%
% mpj
%$G^*$ and $G^\times$ each have (at least) two components because no triple in either of the corresponding triple sets has $\gamma$ on the LHS, whereas $G^*$ may consist of three components, due to $\gamma$ and (potentially) to the cut $A^\times$. By definition, $H^\times$ contains an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$. Running BUILD on $\triples(P)$ will produce a caterpillar tree (see Fig.\ \ref{fig:pathtree}), via an Ahograph consisting of a tree and an isolated node $\gamma$ (see Fig.\ \ref{fig:ahograph}).
%
%Since $H^{\times\gamma}$ contains $P$ as well as $\arc(\gamma\alpha|\beta)$, $\gamma$ is not an isolated A-node in $G^{\times\gamma}$, which is connected, and so BUILD will fail when run on $G^{\times\gamma}$. 

Recalling the construction of $H$, there are three types of places where the absent cross-arcs $A^\times$ could be located: within a clause gadget, within a variable gadget, or elsewhere, i.e., {\em forced arcs} (viz., connecting arcs $a_1,...,a_4$ or arcs with tail of the form $c_j c_{j+1}$ following a clause $C_j$'s gadget). There is one special subcase, which we give a name to.

\begin{definition}
We call $A^\times$ {\em degenerate} if $A^\times$ lies within a variable $x_i$'s gadget, $|A^\times|=2$, and exactly one of its members has the form $\arc(b_ib'_i|\tilde x_i^1)$. (Its other member must by definition lie within the $x_i$ gadget's opposite side.) %Otherwise, $A^\times$ is {\em non-degenerate}.
\end{definition}

We deal with all cases besides an degenerate $A^\times$ in the following lemma.


\begin{lemma}\label{lem:treeexs}
%Let $A'$ be acyclic, suppose there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$, and let $V_{\alpha \beta}^* \subseteq V_{\alpha\beta}$ and $V_{c_{m+1}\gamma}^* \subseteq V_{c_{m+1}\gamma}$ be defined as above,
%%in the proof of Lemma \ref{lem:notentailed} above, 
%and let $|V_{\alpha \beta}^*| = |V_{c_{m+1}\gamma}^*| \in [3]$, 
%%where is bijection between $V_{\alpha \beta}^*$ and $V_{c_{m+1}\gamma}^*$, with each pair corresponding to a unique A-edge in $A-A'$.
%which together yield $w \in [3]$ pairs $\{(u_h,v_h) : h \in [w]\}$, with each pair connected by an arc $a_h \in  A - A'$.
%
Let $R'$ be consistent.
%Assume that either $|A^\times|=1$ or $A^\times \cap \arcs(\{b_ib'_i|x_i^1,b_ib'_i\bar x_i^1\}) \ne 1$ for all $i \in [n]$, and that $R'$ is consistent.
%Suppose $A' \subseteq A$ is acyclic and 
Suppose there is no path $P \subseteq A'$ from $\alpha\beta$ to $c_{m+1}\gamma$, and that $A^\times$ is non-degenerate.
%either $|A^\times|=1$ or $A^\times \cap \arcs(\{b_ib'_i|x_i^1,b_ib'_i\bar x_i^1\}) \ne 1$ for all $i \in [n]$.
%
%Let the conditions of Lemma \ref{lem:uvpairs} hold, and suppose that either $|A^\times|=1$ or $A^\times \cap \arcs(\{b_ib'_i|x_i^1,b_ib'_i\bar x_i^1\}) \ne 1$ for all $i \in [n]$.
%do not lie within a variable gadget.
Then $R'$ does not entail $\alpha\beta|\gamma$.
%$R' \cup \{\alpha\gamma | \beta\}$ is consistent.
%there exists a tree displaying $R' \cup \{\alpha\gamma | \beta\}$.
\end{lemma}
\begin{proof}
%Now we will show that for such an $A''$, $R' = \triples(A'')$ is compatible with $\alpha\beta | \gamma$ not holding.
%
%Let $w \in [3]$ be the number of pairs $(u_h^*,v_h^*)$. 
%By Lemma, \ref{lem:uvpairs} there are $w \in [3]$ ordered pairs $\{(u_h,v_h) : h \in [w]\}$, with each pair connected (w.l.o.g.) by a unique arc $a_h \in A^\times \subseteq A - A'$.

First, suppose $A^\times$ contains any of the forced arcs, say $a_\times$, corresponding to a triple $p_\times q_\times|o_\times$. % and also to A-edge $\{p_\times,q_\times\}$ in $G^\times$.
%Arc $a_\times$ could be either a connecting arc, an arc in one side of a variable gadget (where none of the other side's arcs are included in $A'$, or an arc in one witness path of a clause gadget (where none of its other witness paths' arcs are included in $A'$). 
Now, consider the effect of the corresponding A-edge $\{p_\times,q_\times\}$'s absence from $G^\gamma$: $p_\times$ and $q_\times$ must lie in different components of it, since (observe) the only multi-edges in $G^\gamma$ are $\{b_i,b'_i\}$ for $i \in [n]$ and $\{c_j,d_j\}$ for $j \in [m]$, i.e., those due to nodes in $H$ with out-degree 2. Let $C^\alpha$ be the component in $G^\gamma$ containing $\alpha$ and $C^{\bar\alpha}$ the the other, and let the leaves be named so that $C^\alpha$ contains $p_\times$ and $C^{\bar\alpha}$ contains $q_\times$.

%Let the leaves be named so that $p_k$ is the leaf appearing on the RHS of the arc $a'=\arc(p'q'|o')$ in $H^\times$, i.e., $p_\times=o'$, in which case $q_\times$ does not appear in $\arc(e')$ and moreover A-node $q_\times$ does not appear in $C^\alpha$, and A-node $p_\times$ does not appear in $C^\alpha$. Therefore $G^\gamma$ will consist of two components: one before the cut (including $\gamma$) and one after, each of them containing an A-leaf whose A-edge label is an A-node lying in the {\em other} component: $q_\times=o'$ is an A-node in $C^{\bar\alpha}$, and $\gamma$ (the label of A-edge $\{c_mc_{m+1}\}$) is an A-node in $C^\alpha$.

Now, consider what happens when BUILD recurses on the triple and leaf sets corresponding to each of these components: in each case, BUILD will encounter a leaf set whose triples permit a linear ordering (similar to Table \ref{tbl:linord}), which therefore can be displayed in a (caterpillar) tree. In particular, in BUILD's recursive call for $[C^{\bar\alpha},V(C^{\bar\alpha})]$, $c_{m+1}$ will be an isolated node and the rest of the Ahograph will induce a DAG (directed acyclic graph) directed away from from $\gamma$; and in the recursive call for $[C^\alpha,V(C^\alpha)]$, $p_\times$ will be an isolated node and again the rest of the Ahograph will induce a DAG.
%therefore the Ahograph for that recursive call will consist of two components, an isolated A-node and a tree. 
In each of these two calls, therefore, BUILD's execution on its isolated-A-node-and-DAG pair will behave similarly ({\em despite the fact} that the portions of this Ahograph corresponding to clause gadgets may contain A-nodes and A-edges corresponding to all three witness paths, and the portions corresponding to variable gadgets may contain A-nodes and A-edges corresponding to both sides) to its execution on $\triples(P)$ for the acyclic $P$ in Lemmas \ref{lem:consistR} and \ref{lem:isentailed} (see Fig.\ \ref{fig:ahograph}), with each iteration isolating one additional node, thus constructing a caterpillar tree. These two caterpillars will become the root's child subtrees in the resulting tree displaying $R' \cup \{\gamma\alpha|\beta\}$ (see Fig.\ \ref{fig:cuttreeforced}).

Second, suppose there does not exist a path though the series of variable gadgets, i.e., from $b_1b'_1$ to $b_{n+1}b'_{n+1}$, meaning there does not exist a path through {\em some} variable gadget, i.e., from $b_ib'_i$ to $b_{i+1}b'_{i+1}$ for some $i \in [n]$. Then $A^\times$ must contain an arcs from both sides of $x_i$'s gadget, say $\arcs(z_i^\ell,z_{i^\ell+1}|z_i^{\ell+2},~ \bar z_i^{\ell'},\bar z_i^{\ell'+1}|\bar z_i^{\ell'+2}))$, where (because $A^\times$ is nondegenerate) either both or neither of $z_i^{\ell},\bar z_i^{\ell'}$ equals $b_i$. The absence of the two corresponding A-edges means that the Ahograph $G'$ will be disconnected. During BUILD's recursive calls for these two components, the whole process will play out similarly to how it did in the previous case (see Fig.\ \ref{fig:cuttreevar}).

%The third case is when the cut goes through some variable $x_i$'s gadget. Then $|A^\times|=2$ (if both sides of the $x_i$ gadget are including in $A'$). Since $A^\times$ is non-degenerate (i.e., either {\em both or neither} of these arcs are outgoing arcs of $b_ib'_i$), the Ahograph will be disconnected, and the whole process will play out similarly to the other two cases.


Third, suppose there does not exist a path through the series of clause gadgets, i.e., from $c_1d_1$ to $c_{m+1}d_{m+1}$. Since none of the forced arcs is missing, this means there does not exist a path through some clause gadget, i.e., from $c_jd_j$ to $c_{j+1}d_{j+1}$ for some $j \in [m]$. Then $A\times$ must contain an arc from each of the clause gadget's three witness paths (or similarly from {\em both} of them if the clause has only two literals).

%consider the case of the cut going through a clause gadget, in which case $A^\times$ consists of either two or  three arcs (since we have already dealt with the case of $|A^\times|=1$), each lying within one off that clause's witness paths. The case of two arcs is similar, so consider the most complex case of three.

Now there are several subcases to consider, but they all behave similarly. First, suppose $A^\times$ includes $c_jd_j$'s three outgoing arcs, each corresponding to a triple of the form $c_jd_j|\tilde x_{\hat w}^j$. Now, consider the effects of $c_jd_j$'s outgoing arcs' absence from $G^\gamma$: this means the three corresponding A-edges between $c_j$ and $d_j$ are absent, isolating $d_j$. Thus the initial input to BUILD consists of two components: isolated A-node $d_j$, and a DAG. In the recursive call for the DAG, the A-edge $\{c_{j-1},c_j\}$ labeled $d_j$ will no longer exist, and thus the corresponding Ahograph will consist of two components: one corresponding to the portion of the hypergraph from $\gamma$ through $C_{j-1}$'s gadget, and another corresponding top the portion from $C_j$'s gadget ({\em except for $d_j$}) though $c_{m+1}$. Now consider the recursive calls for these two components. Within the first component's recursive call, the three leaves of the form $\tilde y_{\hat w}^j$ will have been isolated, with the result that in subsequent calls the leaves of the form $\tilde x_{\hat w}^j$ will have been isolated, and so on, yielding a caterpillar tree. Similarly, $c_{m+1}$ will be isolated within the second recursive call, eventually yielding a second caterpillar tree. Then BUILD's final result will be a tree whose root's children are $d_j$ and a subtree whose two children are the roots of the two aforementioned caterpillar trees.

With three witness paths to cut, then there are  (up to isomorphism) either other subcases, which can all be verified through similar reasoning. The three cut arcs in any given case will be a subset from among the three $c_j \tilde y_{\hat w}^j$ nodes' outgoing arcs, the three $c_j \tilde x_{\hat w}^j$ nodes' outgoing arcs, and $c_jd_j$'s three outgoing arcs. Each cut arc outgoing from a $c_j \tilde y_{\hat w}^j$ node or a $c_j \tilde x_{\hat w}^j$ node will yield an isolated A-node. The initial Ahograph will therefore consist of either 1, 2, or 3 isolated A-nodes plus a DAG. Since it breaks ties arbitrarily, suppose BUILD always places isolated A-nodes as right children in the binary tree being constructed. Any time an A-node $\tilde y_{\hat w}^j$ is isolated (for some $w \in [3]$), in the following recursive call with $\tilde y_{\hat w}^j$ removed, $\tilde x_{\hat w}^j$ will be isolated. And in the recursive call following the isolation and removal of $\tilde x_{\hat w}^j$ for all $w=1,2,3$, $d_j$ will be isolated and removed.

At that point, the remaining Ahograph will consist of two DAGs $C^\alpha$ and $C^{\bar\alpha}$, where $C^\alpha$ contains $\alpha$ and $C^{\bar\alpha}$ does not. $C^{\bar\alpha}$ will also contain $c_j$ and any other A-nodes corresponding to $C_j$'s gadget that have not already been isolated and removed. In particular, $A^\times$ containing a cut arc outgoing from a $c_j \tilde x_{\hat w}^j$ node will mean $C^\alpha$ contains $y_{\hat w}^j$, and $A^\times$ containing a cut arc incoming to a $c_j \tilde x_{\hat w}^j$ will mean $C^\alpha$ contains $x_{\hat w}^j$ and $y_{\hat w}^j$.

The resulting binary tree (see Fig.\ \ref{fig:cuttreeclause}) will consist of a caterpillar region beginning at the root containing the 1-7 A-nodes isolated before the disconnection of the Ahograph into $C^\alpha$ and $C^{\bar\alpha}$, followed by a node whose two child subtrees are caterpillar trees resulting from $C^\alpha$ and $C^{\bar\alpha}$.
%
%The pattern is that the isolation of any A-node $y_{\hat w}^j$ will, in subsequent recursive calls, isolate the corresponding $x_{\hat w}^j$, the isolation of all three of which will in turn isolate $d_j$, after which the process continues as in the previous case, eventually yielding a tree (albeit a slightly differently shaped one).
\end{proof}


The problematic situation is when exactly {\em one} of the two arcs is outgoing from $b_ib'_i$. In this case, their absence deletes only one of the Ahograph's two A-edges between the pair $\{b_i,b'_i\}$, which does {\em not} disconnect the graph, meaning BUILD will fail.

We have been arguing that if a consistent $R'$ entails $\alpha\beta|\gamma$ then $\arcs(R')$ must contain an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$. Now we refine this to a slightly weaker (yet strong enough) implication: if a consistent $R'$ entails $\alpha\beta|\gamma$, then a slightly different consistent $R^+$ will too, and an acyclic path must exist within $\arcs(R^+)$.
%(even if it does not within $\arcs(R')$).

%We handle this case via the following argument.

Taking the contrapositive, we rewrite the previous lemma as:
\begin{corollary}
Let $R'$ be consistent.
Suppose $R' \vdash \alpha\beta|\gamma$ and that $A'$ contains no path from $\alpha\beta$ to $c_{m+1}\gamma$.
Then $A^\times$ is degenerate.
%Then $|A^\times|=2$ and $A^\times$ contains exactly one arc $a_\times$ of the form $\arc(b_ib'_i|\tilde x_i^1)$.
\end{corollary}


\begin{lemma}\label{lem:degeneratecutpath}
Let $R'$ be consistent.
Suppose $R' \vdash \alpha\beta|\gamma$ and that $A'$ contains no path from $\alpha\beta$ to $c_{m+1}\gamma$.
%Assume $|A^\times|=2$ and $A^\times$ contains exactly one arc $a_\times$ of the form $\arc(b_ib'_i|\tilde x_i^1)$, and that $R'$ is consistent.
%
%Suppose a consistent $R'$ entails $\alpha\beta|\gamma$, $|A^\times|=2$, and $A^\times$ contains exactly one arc $a_\times$ of the form $\arc(b_ib'_i|\tilde x_i^1)$.
Then there exists an acyclic path $P \subseteq A' \cup \{a_\times\}$.
%
\end{lemma}
\begin{proof}
%
%In this scenario, the two members of $A^\times$ (which are absent from $A'$) are one of the two possible arcs with tail $b_ibi_i$ (say, $\arc(b_ib'_i|x_i^1)$), and an arc within the $x_i$ gadget's other side (whose tail is not $b_ib'_i$). 
%
The corollary implies that $A^\times$ is degenerate.
%$|A^\times|=2$ and $A^\times$ contains exactly one arc $a_\times$ of the form $\arc(b_ib'_i|\tilde x_i^1)$.

Let $H^+$ be the hypergraph obtained by adding $a_\times$ to $H^*$, which by construction contains a path (say, $P^+$) from $\alpha\beta$ to $c_{m+1}\gamma$.
%
Let $R^+ = \triples(A^+)$, where $A^+ = A' \cup \{a_\times\}$ is $H^+$'s arc set.

We claim that $R^+$ is consistent. We know that the point at which BUILD would potentially fail when executed on a subset of $R$ is in a call when an A-edge of the form $\{c_j,\tilde y_{\hat i_j}^j\}{:}c_{j+1}$ has been removed and the Ahograph is not disconnected, because $\tilde y_{\hat i_j}^j$ is not isolated (see Fig.\ \ref{fig:ahocycle}). But if this occurs when BUILD is executed on $R^+$, it would also have occurred when BUILD is executed on $R^*$ because $\tilde y_{\hat i_j}^j$ would still be connected in that scenario as well (see Fig.\ \ref{fig:ahodiscordvar}).
%
Therefore $A^+$, and in particular $P^+$, is acyclic.
%
%This proves in the variable gadget case as well that if a consistent $R'$ entails $\alpha\beta|\gamma$, then there exists an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$, concluding the proof.
%
%
%We want to show that if $\triples(A' \cup A^\times)$ entails $\alpha\beta|\gamma$, then $\triples(A' \cup A^\times) \cup \{b_ib'_i|x_i^1\}$ does too.
%
%We claim that $H^{*\prime}$ is acyclic.
\end{proof}


%\vskip 2cm
%
%There must be some latest common predecessor node $u^0$ of $\{u_h : h \in [w]\}$ and some earliest common successor node $v^\omega$ of $\{v_h : h \in [w]\}$. Let the (possibly empty) sequence of {\em intermediate} nodes lying on the path strictly between $u^0$ and $u_h$ be $U_h = (u_h^1,...,u_h^{\ell_h})$, and the (possibly empty) sequence of {\em intermediate} nodes lying on the path strictly between $v_h$ and $v^\omega$ be $V_h = (v_h^{1},...,v_h^{\ell_h'})$. Observe that for each node in $U_h$, its incoming arc introduces one more leaf appearing in the corresponding triple's RHS, and so $U_h$ corresponds to $\ell_h$ such leaves, say, $p_h^1,...,p_h^{\ell_h}$. The first member of $V_h$ has no incoming arc, but for each subsequent member of $V_h$, the triple corresponding to its incoming arc similarly introduces one new leaf in its RHS; in addition, $V_h$'s first member's outgoing arc introduces one more new leaf. Thus $V_h$ corresponds to $\ell_h'$ leaves, say, $q_h^1,...,q_h^{\ell_h'}$.
%%
%%Similarly, for each node in $V_h$ after the first, its incoming arc introduces one more leaf in the triple's LHS, except for $v_1^1$, which introduces {\em two} more, because the leaf it shares in common with $u_w$ is also appearing on the LHS of a triple for the first time, due to $u_w$'s missing outgoing cross-arc, for a total of $\ell_h'+1$ such leaves, say, $q_h^0,...,q_h^{\ell_h'}$. 
%Let $p_0$ be the leaf introduced by node $u^0$, and $q^\omega$ the leaf introduced by node $v^\omega$.
%
%Then observe that $\{p^0\} \cup \bigcup_{h \in [w]} U_h$ can be put in a linear order, and hence $S(\alpha\beta,V,R')$ can be as well. Let $L_S$ be the set of all leaves appearing in tail nodes of paths between $\alpha\beta$ and members of $V_{\alpha\beta}$, i.e., the leaves appearing in nodes $V_{\alpha\beta} - \{U_h^{\ell_h} : h \in [w]\}$. Then can we construct a caterpillar tree $C_S$ having leaves $L_S$ (see root's left subtree in Fig.\ \ref{fig:nopathtree}, except ignoring the appearance of $\gamma$ for a moment).
%
%Similarly, observe that $\{q^\omega\} \cup \bigcup_{h \in [w]} V_h$ and hence $V_{c_{m+1}\gamma}$ can also be linearly ordered, and so if we define $L_P$ as the set of all leaves appearing in tail nodes of paths between members of $V_{c_{m+1}\gamma}$ and $c_{m+1}\gamma$,  i.e., the leaves appearing in nodes $V_{c_{m+1}\gamma} - \{c_{m+1}\gamma\}$, then we can also construct a caterpillar tree $C_P$ with leaves $L_P$ (see right subtree in Fig.\ \ref{fig:nopathtree}).
%
%Now create a root node, whose children are the roots of $C_P$ and $S_P$. This resulting tree contains every leaf but $\gamma$, and observe that it displays every triple of $R'$ except (obviously) $c_m c_{m+1} | \gamma$.
%
%Finally, we subdivide the tree's A-edge to $\alpha$ and add $\gamma$ as the second child of the tree's new inner node, with the result that the tree now displays $c_j c_{j+1} | \gamma$ and the rest of the triples of $R'$, as desired, yet also displays $\alpha \gamma | \beta$.
%
%\vskip 2cm


This implies:

\begin{corollary}[$\Rightarrow$]\label{cor:ispath}
If there is a consistent $R'$ entailing $\alpha\beta|\gamma$ then there exists an acyclic path $P$.
\end{corollary}

%Combining Lemmas \ref{lem:cycpath} and \ref{lem:treeexs}, we obtain:
%
%\begin{lemma}[$\Rightarrow$]\label{lem:notentailed}
%%If $R'$ is a consistent subset of $R$ entailing $\alpha\beta|\gamma$, then $A' = \arcs(R')$ contains the arcs of an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%%
%%Let $A' \subseteq A$. not
%Suppose there is no acyclic path $P \subseteq A$ from $\alpha\beta$ to $c_{m+1}\gamma$. Then for every subset $A' \subseteq A$, $R' = \triples(A')$ is  inconsistent or does not entail $\alpha\beta|\gamma$.
%%If $A' \subseteq A$ is {\em not} an acyclic arc set subsuming the set $P$ of arcs appearing in some path from $\alpha\beta$ to $c_{m+1}\gamma$, then $R' = \triples(A')$ is not a consistent subset of $R$ entailing $\alpha\beta|\gamma$.
%\end{lemma}


%\textbf{start quotes:}
%
%%{\em Q: how do we know that a subset entailing $\alpha\beta|\gamma$ must necessarily correspond to a path?}
%
%\begin{lemma}[Bryant and Steel,  Prop. 9(1)]\label{lem:noabctrip} If $R$ is a closed set of rooted triples containing no triple with
%the leaves $\{a,b,c\}$ then $R \cup \{ab|e\}$, $R \cup \{ae|b\}$ and $R \cup \{be|a\}$ are all compatible.
%\end{lemma}
%
%{\em Q: can we get that entailment must follow a path by repeated (inductive) application of Lemma \ref{lem:noabctrip}?}
%
%\textbf{\em Q: is the consistency and/or the closure of a path in this construction actually somehow just obvious based on the construction?}
%\textbf{end quotes}





%\begin{lemma}[$\Leftarrow$]
%If there is a consistent triple set $R'$ entailing $\alpha\beta|\gamma$, then there is an acyclic path $P$ from $\alpha\beta$ to $c_{m+1}\gamma$.
%%
%%Or: If there is no acyclic path from $ab$ to $ac$, then there is no consistent subset entailing $\alpha\beta|\gamma$.
%\end{lemma}
%\begin{proof}
%%First observe that the only triple in $R$ including $\alpha$ is $\alpha\beta | b_1$, and so any hypothetical subset $R' \subset R$ entailing $\alpha\beta|\gamma$ must necessarily include $\alpha\beta | b_1$.  But then observe that the only other triple in $R$ including $\beta$ is $\beta b_1 | b'_1$. By repeated application of similar arguments, we obtain that the hyperarcs corresponding to the triples of any such $R'$ must trace out a path from $\alpha\beta$ to $c_{m+1}\gamma$.
%
%Second, observe that if the path contained a cycle, then the triples corresponding to the hyperarcs appearing in that cycle would themselves be inconsistent, contradicting the consistency of $R'$.
%%the portion of the Ahograph induced by everything from the start of the caterpillar up to the cycle's back-arc would be a single component.
%%
%%That is, if we pluck off the sink nodes one by one, then plucking off the node just following the back-arc will reduce the number of components from 2 to 1, indicating that $R$ is inconsistent.
%%
%%Does it suffice to argue that for any path from $ab$ to $ac$, if the path is acyclic then it implies a consistent subset entailing $\alpha\beta|\gamma$?
%%
%%\textbf{That is, can we assume that entailment will imply a path?}
%\end{proof}




%\begin{lemma}[$\Rightarrow$]
%If there is an acyclic path from $\alpha\beta$ to $c_{m+1}\gamma$, then there is a satisfying truth assignment.
%\end{lemma}
%\begin{proof}
%We read off the truth assignment from the choices the path makes passing through the series of variable gadgets. Because the path is acyclic, we know that in the case of each clause gadget it passes through, the node within the variable gadget pointed to is on the side of the variable gadget that the path did {\em not} use. Since we set the variable's truth value based on which side we did not use, this implies that the corresponding literal in the clause gadget is true, thus satisfying the clause.
%\end{proof}

Combining the Corollary \ref{cor:consentails} and \ref{cor:ispath} with Theorem \ref{thm:apdh}, we conclude:

\begin{theorem}
\entailprob\:is NP-Complete.
\end{theorem}

And because computing the closure reduces to deciding whether $R \vdash t$ for $O(|L|^3)$ triples $t$, we also have:

\begin{corollary}
\closureprob\:is NP-hard.
\end{corollary}


%Also:
%
%\begin{corollary}
%The complementary problem, of deciding whether a triple is entailed by {\em every} consistent subset of $R$ is co-NP-Complete.
%\end{corollary}
%\begin{proof}
%Solve the original problem for both negations of the triple.
%\end{proof}

